Planet formation: key mechanisms and global models

Models of planet formation are built on underlying physical processes. In order to make sense of the origin of the planets we must first understand the origin of their building blocks. This review comes in two parts. The first part presents a detailed description of six key mechanisms of planet formation: 1) The structure and evolution of protoplanetary disks 2) The formation of planetesimals 3) Accretion of protoplanets 4) Orbital migration of growing planets 5) Gas accretion and giant planet migration 6) Resonance trapping during planet migration. While this is not a comprehensive list, it includes processes for which our understanding has changed in recent years or for which key uncertainties remain. The second part of this review shows how global models are built out of planet formation processes. We present global models to explain different populations of known planetary systems, including close-in small/low-mass planets (i.e., super-Earths), giant exoplanets, and the Solar System's planets. We discuss the different sources of water on rocky exoplanets, and use cosmochemical measurements to constrain the origin of Earth's water. We point out the successes and failings of different models and how they may be falsified. Finally, we lay out a path for the future trajectory of planet formation studies.

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> refs_bbl.include.tex <==
\begin{thebibliography}{100}
\providecommand{\url}[1]{{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{DOI~\discretionary{}{}{}#1}\else
  \providecommand{\doi}{DOI~\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi

\bibitem{abod19}
{Abod}, C.P., {Simon}, J.B., {Li}, R., {Armitage}, P.J., {Youdin}, A.N.,
  {Kretke}, K.A.: {The Mass and Size Distribution of Planetesimals Formed by
  the Streaming Instability. II. The Effect of the Radial Gas Pressure
  Gradient}.
\newblock \apj \textbf{883}(2), 192 (2019).
\newblock \doi{10.3847/1538-4357/ab40a3}

\bibitem{absil13}
{Absil}, O., {Defr{\`e}re}, D., {Coud{\'e} du Foresto}, V., {Di Folco}, E.,
  {M{\'e}rand}, A., {Augereau}, J.C., {Ertel}, S., {Hanot}, C., {Kervella}, P.,
  {Mollier}, B., {Scott}, N., {Che}, X., {Monnier}, J.D., {Thureau}, N.,
  {Tuthill}, P.G., {ten Brummelaar}, T.A., {McAlister}, H.A., {Sturmann}, J.,
  {Sturmann}, L., {Turner}, N.: {A near-infrared interferometric survey of
  debris-disc stars. III. First statistics based on 42 stars observed with
  CHARA/FLUOR}.
\newblock \aap \textbf{555}, A104 (2013).
\newblock \doi{10.1051/0004-6361/201321673}

\bibitem{adams08}
{Adams}, E.R., {Seager}, S., {Elkins-Tanton}, L.: {Ocean Planet or Thick
  Atmosphere: On the Mass-Radius Relationship for Solid Exoplanets with Massive
  Atmospheres}.
\newblock \apj \textbf{673}, 1160--1164 (2008).
\newblock \doi{10.1086/524925}

\bibitem{adams04}
{Adams}, F.C., {Hollenbach}, D., {Laughlin}, G., {Gorti}, U.: {Photoevaporation
  of Circumstellar Disks Due to External Far-Ultraviolet Radiation in Stellar
  Aggregates}.
\newblock \apj \textbf{611}, 360--379 (2004).
\newblock \doi{10.1086/421989}

\bibitem{adams03}
{Adams}, F.C., {Laughlin}, G.: {Migration and dynamical relaxation in crowded
  systems of giant planets}.
\newblock Icarus \textbf{163}, 290--306 (2003).
\newblock \doi{10.1016/S0019-1035(03)00081-2}

\bibitem{agnor99}
{Agnor}, C.B., {Canup}, R.M., {Levison}, H.F.: {On the Character and
  Consequences of Large Impacts in the Late Stage of Terrestrial Planet
  Formation}.
\newblock Icarus \textbf{142}, 219--237 (1999).
\newblock \doi{10.1006/icar.1999.6201}

\bibitem{alexander19a}
{Alexander}, C.M.O.: {Quantitative models for the elemental and isotopic
  fractionations in chondrites: The carbonaceous chondrites}.
\newblock \gca \textbf{254}, 277--309 (2019).
\newblock \doi{10.1016/j.gca.2019.02.008}

\bibitem{alexander19b}
{Alexander}, C.M.O.: {Quantitative models for the elemental and isotopic
  fractionations in the chondrites: The non-carbonaceous chondrites}.
\newblock \gca \textbf{254}, 246--276 (2019).
\newblock \doi{10.1016/j.gca.2019.01.026}

\bibitem{alexander12}
{Alexander}, C.M.O.., {Bowden}, R., {Fogel}, M.L., {Howard}, K.T., {Herd},
  C.D.K., {Nittler}, L.R.: {The Provenances of Asteroids, and Their
  Contributions to the Volatile Inventories of the Terrestrial Planets}.
\newblock Science \textbf{337}, 721 (2012).
\newblock \doi{10.1126/science.1223474}

\bibitem{alexander18}
{Alexander}, C.M.O., {McKeegan}, K.D., {Altwegg}, K.: {Water Reservoirs in
  Small Planetary Bodies: Meteorites, Asteroids, and Comets}.
\newblock \ssr \textbf{214}, 36 (2018).
\newblock \doi{10.1007/s11214-018-0474-9}

\bibitem{alexander14}
{Alexander}, R., {Pascucci}, I., {Andrews}, S., {Armitage}, P., {Cieza}, L.:
  {The Dispersal of Protoplanetary Disks}.
\newblock Protostars and Planets VI pp. 475--496 (2014)

\bibitem{alexander06}
{Alexander}, R.D., {Armitage}, P.J.: {The Stellar Mass-Accretion Rate Relation
  in T Tauri Stars and Brown Dwarfs}.
\newblock \apjl \textbf{639}, L83--L86 (2006).
\newblock \doi{10.1086/503030}

\bibitem{alexander12b}
{Alexander}, R.D., {Pascucci}, I.: {Deserts and pile-ups in the distribution of
  exoplanets due to photoevaporative disc clearing}.
\newblock \mnras \textbf{422}, L82--L86 (2012).
\newblock \doi{10.1111/j.1745-3933.2012.01243.x}

\bibitem{alma15}
{ALMA Partnership}, {Brogan}, C.L., {P{\'e}rez}, L.M., {Hunter}, T.R., {Dent},
  W.R.F., {Hales}, A.S., {Hills}, R.E., {Corder}, S., {Fomalont}, E.B.,
  {Vlahakis}, C., {Asaki}, Y., {Barkats}, D., {Hirota}, A., {Hodge}, J.A.,
  {Impellizzeri}, C.M.V., {Kneissl}, R., {Liuzzo}, E., {Lucas}, R.,
  {Marcelino}, N., {Matsushita}, S., {Nakanishi}, K., {Phillips}, N.,
  {Richards}, A.M.S., {Toledo}, I., {Aladro}, R., {Broguiere}, D., {Cortes},
  J.R., {Cortes}, P.C., {Espada}, D., {Galarza}, F., {Garcia-Appadoo}, D.,
  {Guzman-Ramirez}, L., {Humphreys}, E.M., {Jung}, T., {Kameno}, S., {Laing},
  R.A., {Leon}, S., {Marconi}, G., {Mignano}, A., {Nikolic}, B., {Nyman}, L.A.,
  {Radiszcz}, M., {Remijan}, A., {Rod{\'o}n}, J.A., {Sawada}, T., {Takahashi},
  S., {Tilanus}, R.P.J., {Vila Vilaro}, B., {Watson}, L.C., {Wiklind}, T.,
  {Akiyama}, E., {Chapillon}, E., {de Gregorio-Monsalvo}, I., {Di Francesco},
  J., {Gueth}, F., {Kawamura}, A., {Lee}, C.F., {Nguyen Luong}, Q., {Mangum},
  J., {Pietu}, V., {Sanhueza}, P., {Saigo}, K., {Takakuwa}, S., {Ubach}, C.,
  {van Kempen}, T., {Wootten}, A., {Castro-Carrizo}, A., {Francke}, H.,
  {Gallardo}, J., {Garcia}, J., {Gonzalez}, S., {Hill}, T., {Kaminski}, T.,
  {Kurono}, Y., {Liu}, H.Y., {Lopez}, C., {Morales}, F., {Plarre}, K.,
  {Schieven}, G., {Testi}, L., {Videla}, L., {Villard}, E., {Andreani}, P.,
  {Hibbard}, J.E., {Tatematsu}, K.: {The 2014 ALMA Long Baseline Campaign:
  First Results from High Angular Resolution Observations toward the HL Tau
  Region}.
\newblock \apjl \textbf{808}, L3 (2015).
\newblock \doi{10.1088/2041-8205/808/1/L3}

\bibitem{amelin02}
{Amelin}, Y., {Krot}, A.N., {Hutcheon}, I.D., {Ulyanov}, A.A.: {Lead Isotopic
  Ages of Chondrules and Calcium-Aluminum-Rich Inclusions}.
\newblock Science \textbf{297}(5587), 1678--1683 (2002).
\newblock \doi{10.1126/science.1073950}

\bibitem{andrews18}
{Andrews}, S.M., {Huang}, J., {P{\'e}rez}, L.M., {Isella}, A., {Dullemond},
  C.P., {Kurtovic}, N.T., {Guzm{\'a}n}, V.V., {Carpenter}, J.M., {Wilner},
  D.J., {Zhang}, S., {Zhu}, Z., {Birnstiel}, T., {Bai}, X.N., {Benisty}, M.,
  {Hughes}, A.M., {{\"O}berg}, K.I., {Ricci}, L.: {The Disk Substructures at
  High Angular Resolution Project (DSHARP). I. Motivation, Sample, Calibration,
  and Overview}.
\newblock \apjl \textbf{869}(2), L41 (2018).
\newblock \doi{10.3847/2041-8213/aaf741}

\bibitem{andrews05}
{Andrews}, S.M., {Williams}, J.P.: {Circumstellar Dust Disks in Taurus-Auriga:
  The Submillimeter Perspective}.
\newblock \apj \textbf{631}, 1134--1160 (2005).
\newblock \doi{10.1086/432712}

\bibitem{andrews07a}
{Andrews}, S.M., {Williams}, J.P.: {A Submillimeter View of Circumstellar Dust
  Disks in {$\rho$} Ophiuchi}.
\newblock \apj \textbf{671}, 1800--1812 (2007).
\newblock \doi{10.1086/522885}

\bibitem{andrews07b}
{Andrews}, S.M., {Williams}, J.P.: {High-Resolution Submillimeter Constraints
  on Circumstellar Disk Structure}.
\newblock \apj \textbf{659}, 705--728 (2007).
\newblock \doi{10.1086/511741}

\bibitem{andrews09}
{Andrews}, S.M., {Wilner}, D.J., {Hughes}, A.M., {Qi}, C., {Dullemond}, C.P.:
  {Protoplanetary Disk Structures in Ophiuchus}.
\newblock \apj \textbf{700}, 1502--1523 (2009).
\newblock \doi{10.1088/0004-637X/700/2/1502}

\bibitem{andrews10}
{Andrews}, S.M., {Wilner}, D.J., {Hughes}, A.M., {Qi}, C., {Dullemond}, C.P.:
  {Protoplanetary Disk Structures in Ophiuchus. II. Extension to Fainter
  Sources}.
\newblock \apj \textbf{723}, 1241--1254 (2010).
\newblock \doi{10.1088/0004-637X/723/2/1241}

\bibitem{andrews16}
{Andrews}, S.M., {Wilner}, D.J., {Zhu}, Z., {Birnstiel}, T., {Carpenter}, J.M.,
  {P{\'e}rez}, L.M., {Bai}, X.N., {{\"O}berg}, K.I., {Hughes}, A.M., {Isella},
  A., {Ricci}, L.: {Ringed Substructure and a Gap at 1 au in the Nearest
  Protoplanetary Disk}.
\newblock \apjl \textbf{820}, L40 (2016).
\newblock \doi{10.3847/2041-8205/820/2/L40}

\bibitem{anglada10}
{Anglada-Escud{\'e}}, G., {L{\'o}pez-Morales}, M., {Chambers}, J.E.: {How
  Eccentric Orbital Solutions Can Hide Planetary Systems in 2:1 Resonant
  Orbits}.
\newblock \apj \textbf{709}(1), 168--178 (2010).
\newblock \doi{10.1088/0004-637X/709/1/168}

\bibitem{anglada13}
{Anglada-Escud{\'e}}, G., {Tuomi}, M., {Gerlach}, E., {Barnes}, R., {Heller},
  R., {Jenkins}, J.S., {Wende}, S., {Vogt}, S.S., {Butler}, R.P., {Reiners},
  A., {Jones}, H.R.A.: {A dynamically-packed planetary system around GJ 667C
  with three super-Earths in its habitable zone}.
\newblock \aap \textbf{556}, A126 (2013).
\newblock \doi{10.1051/0004-6361/201321331}

\bibitem{armitage11}
{Armitage}, P.J.: {Dynamics of Protoplanetary Disks}.
\newblock \araa \textbf{49}, 195--236 (2011).
\newblock \doi{10.1146/annurev-astro-081710-102521}

\bibitem{armitage16}
{Armitage}, P.J., {Eisner}, J.A., {Simon}, J.B.: {Prompt Planetesimal Formation
  beyond the Snow Line}.
\newblock \apjl \textbf{828}, L2 (2016).
\newblock \doi{10.3847/2041-8205/828/1/L2}

\bibitem{asaduzzaman14}
{Asaduzzaman}, A.M., {Zega}, T.J., {Laref}, S., {Runge}, K., {Deymier}, P.A.,
  {Muralidharan}, K.: {A computational investigation of adsorption of organics
  on mineral surfaces: Implications for organics delivery in the early solar
  system}.
\newblock Earth and Planetary Science Letters \textbf{408}, 355--361 (2014).
\newblock \doi{10.1016/j.epsl.2014.10.029}

\bibitem{badro14}
{Badro}, J., {Cote}, A., {Brodholt}, J.: {A seismologically consistent
  compositional model of Earth's core}.
\newblock PNAS \textbf{132}, 94 (2014)

\bibitem{bae19}
{Bae}, J., {Zhu}, Z., {Baruteau}, C., {Benisty}, M., {Dullemond}, C.P.,
  {Facchini}, S., {Isella}, A., {Keppler}, M., {P{\'e}rez}, L.M., {Teague}, R.:
  {An Ideal Testbed for Planet-Disk Interaction: Two Giant Protoplanets in
  Resonance Shaping the PDS 70 Protoplanetary Disk}.
\newblock \apjl \textbf{884}(2), L41 (2019).
\newblock \doi{10.3847/2041-8213/ab46b0}

\bibitem{Bai16}
{Bai}, X.N.: {Towards a Global Evolutionary Model of Protoplanetary Disks}.
\newblock \apj \textbf{821}, 80 (2016).
\newblock \doi{10.3847/0004-637X/821/2/80}

\bibitem{bai17}
{Bai}, X.N.: {Global Simulations of the Inner Regions of Protoplanetary Disks
  with Comprehensive Disk Microphysics}.
\newblock \apj \textbf{845}(1), 75 (2017).
\newblock \doi{10.3847/1538-4357/aa7dda}

\bibitem{bai13}
{Bai}, X.N., {Stone}, J.M.: {Wind-driven Accretion in Protoplanetary Disks. I.
  Suppression of the Magnetorotational Instability and Launching of the
  Magnetocentrifugal Wind}.
\newblock \apj \textbf{769}(1), 76 (2013).
\newblock \doi{10.1088/0004-637X/769/1/76}

\bibitem{baillie15}
{Bailli{\'e}}, K., {Charnoz}, S., {Pantin}, E.: {Time evolution of snow regions
  and planet traps in an evolving protoplanetary disk}.
\newblock \aap \textbf{577}, A65 (2015).
\newblock \doi{10.1051/0004-6361/201424987}

\bibitem{balbus98}
{Balbus}, S.A., {Hawley}, J.F.: {Instability, turbulence, and enhanced
  transport in accretion disks}.
\newblock Reviews of Modern Physics \textbf{70}, 1--53 (1998).
\newblock \doi{10.1103/RevModPhys.70.1}

\bibitem{barbato18}
{Barbato}, D., {Sozzetti}, A., {Desidera}, S., {Damasso}, M., {Bonomo}, A.S.,
  {Giacobbe}, P., {Colombo}, L.S., {Lazzoni}, C., {Claudi}, R., {Gratton}, R.,
  {LoCurto}, G., {Marzari}, F., {Mordasini}, C.: {Exploring the realm of scaled
  solar system analogues with HARPS}.
\newblock \aap \textbf{615}, A175 (2018).
\newblock \doi{10.1051/0004-6361/201832791}

\bibitem{barenfeld17}
{Barenfeld}, S.A., {Carpenter}, J.M., {Sargent}, A.I., {Isella}, A., {Ricci},
  L.: {Measurement of Circumstellar Disk Sizes in the Upper Scorpius OB
  Association with ALMA}.
\newblock \apj \textbf{851}(2), 85 (2017).
\newblock \doi{10.3847/1538-4357/aa989d}

\bibitem{baruteau14}
{Baruteau}, C., {Meru}, F., {Paardekooper}, S.J.: {Rapid inward migration of
  planets formed by gravitational instability}.
\newblock \mnras \textbf{416}(3), 1971--1982 (2011).
\newblock \doi{10.1111/j.1365-2966.2011.19172.x}

\bibitem{batalha13}
{Batalha}, N.M., {Rowe}, J.F., {Bryson}, S.T., {Barclay}, T., {Burke}, C.J.,
  {Caldwell}, D.A., {Christiansen}, J.L., {Mullally}, F., {Thompson}, S.E.,
  {Brown}, T.M., {Dupree}, A.K., {Fabrycky}, D.C., {Ford}, E.B., {Fortney},
  J.J., {Gilliland}, R.L., {Isaacson}, H., {Latham}, D.W., {Marcy}, G.W.,
  {Quinn}, S.N., {Ragozzine}, D., {Shporer}, A., {Borucki}, W.J., {Ciardi},
  D.R., {Gautier} III, T.N., {Haas}, M.R., {Jenkins}, J.M., {Koch}, D.G.,
  {Lissauer}, J.J., {Rapin}, W., {Basri}, G.S., {Boss}, A.P., {Buchhave}, L.A.,
  {Carter}, J.A., {Charbonneau}, D., {Christensen-Dalsgaard}, J., {Clarke},
  B.D., {Cochran}, W.D., {Demory}, B.O., {Desert}, J.M., {Devore}, E., {Doyle},
  L.R., {Esquerdo}, G.A., {Everett}, M., {Fressin}, F., {Geary}, J.C.,
  {Girouard}, F.R., {Gould}, A., {Hall}, J.R., {Holman}, M.J., {Howard}, A.W.,
  {Howell}, S.B., {Ibrahim}, K.A., {Kinemuchi}, K., {Kjeldsen}, H., {Klaus},
  T.C., {Li}, J., {Lucas}, P.W., {Meibom}, S., {Morris}, R.L., {Pr{\v s}a}, A.,
  {Quintana}, E., {Sanderfer}, D.T., {Sasselov}, D., {Seader}, S.E., {Smith},
  J.C., {Steffen}, J.H., {Still}, M., {Stumpe}, M.C., {Tarter}, J.C.,
  {Tenenbaum}, P., {Torres}, G., {Twicken}, J.D., {Uddin}, K., {Van Cleve}, J.,
  {Walkowicz}, L., {Welsh}, W.F.: {Planetary Candidates Observed by Kepler.
  III. Analysis of the First 16 Months of Data}.
\newblock \apjs \textbf{204}, 24 (2013).
\newblock \doi{10.1088/0067-0049/204/2/24}

\bibitem{bate18}
{Bate}, M.R.: {On the diversity and statistical properties of protostellar
  discs}.
\newblock \mnras \textbf{475}, 5618--5658 (2018).
\newblock \doi{10.1093/mnras/sty169}

\bibitem{batygin13b}
{Batygin}, K., {Morbidelli}, A.: {Analytical treatment of planetary
  resonances}.
\newblock \aap \textbf{556}, A28 (2013).
\newblock \doi{10.1051/0004-6361/201220907}

\bibitem{batygin15b}
{Batygin}, K., {Morbidelli}, A., {Holman}, M.J.: {Chaotic Disintegration of the
  Inner Solar System}.
\newblock \apj \textbf{799}, 120 (2015).
\newblock \doi{10.1088/0004-637X/799/2/120}

\bibitem{beauge12}
{Beaug{\'e}}, C., {Nesvorn{\'y}}, D.: {Multiple-planet Scattering and the
  Origin of Hot Jupiters}.
\newblock \apj \textbf{751}, 119 (2012).
\newblock \doi{10.1088/0004-637X/751/2/119}

\bibitem{bell94}
{Bell}, K.R., {Lin}, D.N.C.: {Using FU Orionis Outbursts to Constrain
  Self-regulated Protostellar Disk Models}.
\newblock \apj \textbf{427}, 987 (1994).
\newblock \doi{10.1086/174206}

\bibitem{benitez15}
{Ben{\'{\i}}tez-Llambay}, P., {Masset}, F., {Koenigsberger}, G.,
  {Szul{\'a}gyi}, J.: {Planet heating prevents inward migration of planetary
  cores}.
\newblock \nat \textbf{520}, 63--65 (2015).
\newblock \doi{10.1038/nature14277}

\bibitem{benitez18}
{Ben{\'\i}tez-Llambay}, P., {Pessah}, M.E.: {Torques Induced by Scattered
  Pebble-flow in Protoplanetary Disks}.
\newblock \apjl \textbf{855}(2), L28 (2018).
\newblock \doi{10.3847/2041-8213/aab2ae}

\bibitem{bethune17}
{B{\'e}thune}, W., {Lesur}, G., {Ferreira}, J.: {Global simulations of
  protoplanetary disks with net magnetic flux. I. Non-ideal MHD case}.
\newblock \aap \textbf{600}, A75 (2017).
\newblock \doi{10.1051/0004-6361/201630056}

\bibitem{birnstiel16}
{Birnstiel}, T., {Fang}, M., {Johansen}, A.: {Dust Evolution and the Formation
  of Planetesimals}.
\newblock \ssr \textbf{205}, 41--75 (2016).
\newblock \doi{10.1007/s11214-016-0256-1}

\bibitem{birnstiel12}
{Birnstiel}, T., {Klahr}, H., {Ercolano}, B.: {A simple model for the evolution
  of the dust population in protoplanetary disks}.
\newblock \aap \textbf{539}, A148 (2012).
\newblock \doi{10.1051/0004-6361/201118136}

\bibitem{bitsch13}
{Bitsch}, B., {Crida}, A., {Morbidelli}, A., {Kley}, W., {Dobbs-Dixon}, I.:
  {Stellar irradiated discs and implications on migration of embedded planets.
  I. Equilibrium discs}.
\newblock \aap \textbf{549}, A124 (2013).
\newblock \doi{10.1051/0004-6361/201220159}

\bibitem{bitsch19}
{Bitsch}, B., {Izidoro}, A., {Johansen}, A., {Raymond}, S.N., {Morbidelli}, A.,
  {Lambrechts}, M., {Jacobson}, S.A.: {Formation of planetary systems by pebble
  accretion and migration: growth of gas giants}.
\newblock \aap \textbf{623}, A88 (2019).
\newblock \doi{10.1051/0004-6361/201834489}

\bibitem{bitsch15}
{Bitsch}, B., {Johansen}, A., {Lambrechts}, M., {Morbidelli}, A.: {The
  structure of protoplanetary discs around evolving young stars}.
\newblock \aap \textbf{575}, A28 (2015).
\newblock \doi{10.1051/0004-6361/201424964}

\bibitem{bitsch15b}
{Bitsch}, B., {Lambrechts}, M., {Johansen}, A.: {The growth of planets by
  pebble accretion in evolving protoplanetary discs}.
\newblock \aap \textbf{582}, A112 (2015).
\newblock \doi{10.1051/0004-6361/201526463}

\bibitem{bitsch18}
{Bitsch}, B., {Morbidelli}, A., {Johansen}, A., {Lega}, E., {Lambrechts}, M.,
  {Crida}, A.: {Pebble-isolation mass: Scaling law and implications for the
  formation of super-Earths and gas giants}.
\newblock \aap \textbf{612}, A30 (2018).
\newblock \doi{10.1051/0004-6361/201731931}

\bibitem{bitsch14}
{Bitsch}, B., {Morbidelli}, A., {Lega}, E., {Crida}, A.: {Stellar irradiated
  discs and implications on migration of embedded planets. II.
  Accreting-discs}.
\newblock \aap \textbf{564}, A135 (2014).
\newblock \doi{10.1051/0004-6361/201323007}

\bibitem{bitsch19b}
{Bitsch}, B., {Raymond}, S.N., {Izidoro}, A.: {Rocky super-Earths or
  waterworlds: the interplay of planet migration, pebble accretion, and disc
  evolution}.
\newblock \aap \textbf{624}, A109 (2019).
\newblock \doi{10.1051/0004-6361/201935007}

\bibitem{biver16}
{Biver}, N., {Moreno}, R., {Bockel{\'e}e-Morvan}, D., {Sandqvist}, A., {Colom},
  P., {Crovisier}, J., {Lis}, D.C., {Boissier}, J., {Debout}, V., {Paubert},
  G., {Milam}, S., {Hjalmarson}, A., {Lundin}, S., {Karlsson}, T., {Battelino},
  M., {Frisk}, U., {Murtagh}, D., {Odin Team}: {Isotopic ratios of H, C, N, O,
  and S in comets C/2012 F6 (Lemmon) and C/2014 Q2 (Lovejoy)}.
\newblock \aap \textbf{589}, A78 (2016).
\newblock \doi{10.1051/0004-6361/201528041}

\bibitem{blum08}
{Blum}, J., {Wurm}, G.: {The Growth Mechanisms of Macroscopic Bodies in
  Protoplanetary Disks}.
\newblock \araa \textbf{46}, 21--56 (2008).
\newblock \doi{10.1146/annurev.astro.46.060407.145152}

\bibitem{boehnke16}
{Boehnke}, P., {Harrison}, T.M.: {Illusory Late Heavy Bombardments}.
\newblock Proceedings of the National Academy of Science \textbf{113},
  10802--10806 (2016).
\newblock \doi{10.1073/pnas.1611535113}

\bibitem{boisvert18}
{Boisvert}, J.H., {Nelson}, B.E., {Steffen}, J.H.: {Systematic
  mischaracterization of exoplanetary system dynamical histories from a model
  degeneracy near mean-motion resonance}.
\newblock \mnras \textbf{480}, 2846--2852 (2018).
\newblock \doi{10.1093/mnras/sty2023}

\bibitem{boley09}
{Boley}, A.C.: {The Two Modes of Gas Giant Planet Formation}.
\newblock \apjl \textbf{695}(1), L53--L57 (2009).
\newblock \doi{10.1088/0004-637X/695/1/L53}

\bibitem{boley13}
{Boley}, A.C., {Ford}, E.B.: {The Formation of Systems with Tightly-packed
  Inner Planets (STIPs) via Aerodynamic Drift}.
\newblock arXiv:1306.0566  (2013)

\bibitem{boley10}
{Boley}, A.C., {Hayfield}, T., {Mayer}, L., {Durisen}, R.H.: {Clumps in the
  outer disk by disk instability: Why they are initially gas giants and the
  legacy of disruption}.
\newblock \icarus \textbf{207}(2), 509--516 (2010).
\newblock \doi{10.1016/j.icarus.2010.01.015}

\bibitem{bonomo17}
{Bonomo}, A.S., {Desidera}, S., {Benatti}, S., {Borsa}, F., {Crespi}, S.,
  {Damasso}, M., {Lanza}, A.F., {Sozzetti}, A., {Lodato}, G., {Marzari}, F.,
  {Boccato}, C., {Claudi}, R.U., {Cosentino}, R., {Covino}, E., {Gratton}, R.,
  {Maggio}, A., {Micela}, G., {Molinari}, E., {Pagano}, I., {Piotto}, G.,
  {Poretti}, E., {Smareglia}, R., {Affer}, L., {Biazzo}, K., {Bignamini}, A.,
  {Esposito}, M., {Giacobbe}, P., {H{\'e}brard}, G., {Malavolta}, L.,
  {Maldonado}, J., {Mancini}, L., {Martinez Fiorenzano}, A., {Masiero}, S.,
  {Nascimbeni}, V., {Pedani}, M., {Rainer}, M., {Scand ariato}, G.: {The GAPS
  Programme with HARPS-N at TNG . XIV. Investigating giant planet migration
  history via improved eccentricity and mass determination for 231 transiting
  planets}.
\newblock \aap \textbf{602}, A107 (2017).
\newblock \doi{10.1051/0004-6361/201629882}

\bibitem{boss97}
{Boss}, A.P.: {Giant planet formation by gravitational instability.}
\newblock Science \textbf{276}, 1836--1839 (1997).
\newblock \doi{10.1126/science.276.5320.1836}

\bibitem{boss98}
{Boss}, A.P.: {Evolution of the Solar Nebula. IV. Giant Gaseous Protoplanet
  Formation}.
\newblock \apj \textbf{503}(2), 923--937 (1998).
\newblock \doi{10.1086/306036}

\bibitem{boss00}
{Boss}, A.P.: {Possible Rapid Gas Giant Planet Formation in the Solar Nebula
  and Other Protoplanetary Disks}.
\newblock \apjl \textbf{536}(2), L101--L104 (2000).
\newblock \doi{10.1086/312737}

\bibitem{bouvier10}
{Bouvier}, A., {Wadhwa}, M.: {The age of the Solar System redefined by the
  oldest Pb-Pb age of a meteoritic inclusion}.
\newblock Nature Geoscience \textbf{3}, 637--641 (2010).
\newblock \doi{10.1038/ngeo941}

\bibitem{bowler18}
{Bowler}, B.P., {Nielsen}, E.L.: {Occurrence Rates from Direct Imaging
  Surveys}.
\newblock ArXiv e-prints  (2018)

\bibitem{brasser16}
{Brasser}, R., {Matsumura}, S., {Ida}, S., {Mojzsis}, S.J., {Werner}, S.C.:
  {Analysis of Terrestrial Planet Formation by the Grand Tack Model: System
  Architecture and Tack Location}.
\newblock \apj \textbf{821}, 75 (2016).
\newblock \doi{10.3847/0004-637X/821/2/75}

\bibitem{briceno01}
{Brice{\~n}o}, C., {Vivas}, A.K., {Calvet}, N., {Hartmann}, L., {Pacheco}, R.,
  {Herrera}, D., {Romero}, L., {Berlind}, P., {S{\'a}nchez}, G., {Snyder},
  J.A., {Andrews}, P.: {The CIDA-QUEST Large-Scale Survey of Orion OB1:
  Evidence for Rapid Disk Dissipation in a Dispersed Stellar Population}.
\newblock Science \textbf{291}, 93--97 (2001).
\newblock \doi{10.1126/science.291.5501.93}

\bibitem{bromley17}
{Bromley}, B.C., {Kenyon}, S.J.: {Terrestrial Planet Formation: Dynamical
  Shake-up and the Low Mass of Mars}.
\newblock \aj \textbf{153}, 216 (2017).
\newblock \doi{10.3847/1538-3881/aa6aaa}

\bibitem{bryan19}
{Bryan}, M.L., {Knutson}, H.A., {Lee}, E.J., {Fulton}, B.J., {Batygin}, K.,
  {Ngo}, H., {Meshkat}, T.: {An Excess of Jupiter Analogs in Super-Earth
  Systems}.
\newblock \aj \textbf{157}(2), 52 (2019).
\newblock \doi{10.3847/1538-3881/aaf57f}

\bibitem{bryden09}
{Bryden}, G., {Beichman}, C.A., {Carpenter}, J.M., {Rieke}, G.H.,
  {Stapelfeldt}, K.R., {Werner}, M.W., {Tanner}, A.M., {Lawler}, S.M., {Wyatt},
  M.C., {Trilling}, D.E., {Su}, K.Y.L., {Blaylock}, M., {Stansberry}, J.A.:
  {Planets and Debris Disks: Results from a Spitzer/MIPS Search for Infrared
  Excess}.
\newblock \apj \textbf{705}(2), 1226--1236 (2009).
\newblock \doi{10.1088/0004-637X/705/2/1226}

\bibitem{bryden06}
{Bryden}, G., {Beichman}, C.A., {Trilling}, D.E., {Rieke}, G.H., {Holmes},
  E.K., {Lawler}, S.M., {Stapelfeldt}, K.R., {Werner}, M.W., {Gautier}, T.N.,
  {Blaylock}, M., {Gordon}, K.D., {Stansberry}, J.A., {Su}, K.Y.L.: {Frequency
  of Debris Disks around Solar-Type Stars: First Results from a Spitzer MIPS
  Survey}.
\newblock \apj \textbf{636}, 1098--1113 (2006).
\newblock \doi{10.1086/498093}

\bibitem{budde16}
{Budde}, G., {Burkhardt}, C., {Brennecka}, G.A., {Fischer-G{\"o}dde}, M.,
  {Kruijer}, T.S., {Kleine}, T.: {Molybdenum isotopic evidence for the origin
  of chondrules and a distinct genetic heritage of carbonaceous and
  non-carbonaceous meteorites}.
\newblock Earth and Planetary Science Letters \textbf{454}, 293--303 (2016).
\newblock \doi{10.1016/j.epsl.2016.09.020}

\bibitem{budde19}
{Budde}, G., {Burkhardt}, C., {Kleine}, T.: {Molybdenum isotopic evidence for
  the late accretion of outer Solar System material to Earth}.
\newblock Nature Astronomy \textbf{3}, 736--741 (2019).
\newblock \doi{10.1038/s41550-019-0779-y}

\bibitem{butler06}
{Butler}, R.P., {Wright}, J.T., {Marcy}, G.W., {Fischer}, D.A., {Vogt}, S.S.,
  {Tinney}, C.G., {Jones}, H.R.A., {Carter}, B.D., {Johnson}, J.A., {McCarthy},
  C., {Penny}, A.J.: {Catalog of Nearby Exoplanets}.
\newblock \apj \textbf{646}, 505--522 (2006).
\newblock \doi{10.1086/504701}

\bibitem{caracausi16}
{Caracausi}, A., {Avice}, G., {Burnard}, P.G., {F{\"u}ri}, E., {Marty}, B.:
  {Chondritic xenon in the Earth's mantle}.
\newblock \nat \textbf{533}, 82--85 (2016).
\newblock \doi{10.1038/nature17434}

\bibitem{carpenter09}
{Carpenter}, J.M., {Bouwman}, J., {Mamajek}, E.E., {Meyer}, M.R.,
  {Hillenbrand}, L.A., {Backman}, D.E., {Henning}, T., {Hines}, D.C.,
  {Hollenbach}, D., {Kim}, J.S., {Moro-Martin}, A., {Pascucci}, I.,
  {Silverstone}, M.D., {Stauffer}, J.R., {Wolf}, S.: {Formation and Evolution
  of Planetary Systems: Properties of Debris Dust Around Solar-Type Stars}.
\newblock \apjs \textbf{181}, 197--226 (2009).
\newblock \doi{10.1088/0067-0049/181/1/197}

\bibitem{carrera16}
{Carrera}, D., {Davies}, M.B., {Johansen}, A.: {Survival of habitable planets
  in unstable planetary systems}.
\newblock \mnras \textbf{463}, 3226--3238 (2016).
\newblock \doi{10.1093/mnras/stw2218}

\bibitem{carrera18}
{Carrera}, D., {Ford}, E.B., {Izidoro}, A., {Jontof-Hutter}, D., {Raymond},
  S.N., {Wolfgang}, A.: {Identifying Inflated Super-Earths and Photo-evaporated
  Cores}.
\newblock \apj \textbf{866}, 104 (2018).
\newblock \doi{10.3847/1538-4357/aadf8a}

\bibitem{Carrera17}
{Carrera}, D., {Gorti}, U., {Johansen}, A., {Davies}, M.B.: {Planetesimal
  Formation by the Streaming Instability in a Photoevaporating Disk}.
\newblock \apj \textbf{839}, 16 (2017).
\newblock \doi{10.3847/1538-4357/aa6932}

\bibitem{carrera15}
{Carrera}, D., {Johansen}, A., {Davies}, M.B.: {How to form planetesimals from
  mm-sized chondrules and chondrule aggregates}.
\newblock \aap \textbf{579}, A43 (2015).
\newblock \doi{10.1051/0004-6361/201425120}

\bibitem{carrera19}
{Carrera}, D., {Raymond}, S.N., {Davies}, M.B.: {Planet-planet scattering as
  the source of the highest eccentricity exoplanets}.
\newblock \aap \textbf{629}, L7 (2019).
\newblock \doi{10.1051/0004-6361/201935744}

\bibitem{cassan12}
{Cassan}, A., {Kubas}, D., {Beaulieu}, J.P., {Dominik}, M., {Horne}, K.,
  {Greenhill}, J., {Wambsganss}, J., {Menzies}, J., {Williams}, A.,
  {J{\o}rgensen}, U.G., {Udalski}, A., {Bennett}, D.P., {Albrow}, M.D.,
  {Batista}, V., {Brillant}, S., {Caldwell}, J.A.R., {Cole}, A., {Coutures},
  C., {Cook}, K.H., {Dieters}, S., {Dominis Prester}, D., {Donatowicz}, J.,
  {Fouqu{\'e}}, P., {Hill}, K., {Kains}, N., {Kane}, S., {Marquette}, J.B.,
  {Martin}, R., {Pollard}, K.R., {Sahu}, K.C., {Vinter}, C., {Warren}, D.,
  {Watson}, B., {Zub}, M., {Sumi}, T., {Szyma{\'n}ski}, M.K., {Kubiak}, M.,
  {Poleski}, R., {Soszynski}, I., {Ulaczyk}, K., {Pietrzy{\'n}ski}, G.,
  {Wyrzykowski}, {\L}.: {One or more bound planets per Milky Way star from
  microlensing observations}.
\newblock \nat \textbf{481}, 167--169 (2012).
\newblock \doi{10.1038/nature10684}

\bibitem{chambers06}
{Chambers}, J.: {A semi-analytic model for oligarchic growth}.
\newblock Icarus \textbf{180}, 496--513 (2006).
\newblock \doi{10.1016/j.icarus.2005.10.017}

\bibitem{chambers19}
{Chambers}, J.: {An Analytic Model for an Evolving Protoplanetary Disk with a
  Disk Wind}.
\newblock \apj \textbf{879}(2), 98 (2019).
\newblock \doi{10.3847/1538-4357/ab2537}

\bibitem{chambers01}
{Chambers}, J.E.: {Making More Terrestrial Planets}.
\newblock Icarus \textbf{152}, 205--224 (2001).
\newblock \doi{10.1006/icar.2001.6639}

\bibitem{chambers98}
{Chambers}, J.E., {Wetherill}, G.W.: {Making the Terrestrial Planets: N-Body
  Integrations of Planetary Embryos in Three Dimensions}.
\newblock Icarus \textbf{136}, 304--327 (1998).
\newblock \doi{10.1006/icar.1998.6007}

\bibitem{chambers16}
{Chambers}, K.C., {Magnier}, E.A., {Metcalfe}, N., {Flewelling}, H.A., {Huber},
  M.E., {Waters}, C.Z., {Denneau}, L., {Draper}, P.W., {Farrow}, D.,
  {Finkbeiner}, D.P., {Holmberg}, C., {Koppenhoefer}, J., {Price}, P.A.,
  {Saglia}, R.P., {Schlafly}, E.F., {Smartt}, S.J., {Sweeney}, W., {Wainscoat},
  R.J., {Burgett}, W.S., {Grav}, T., {Heasley}, J.N., {Hodapp}, K.W.,
  {Jedicke}, R., {Kaiser}, N., {Kudritzki}, R.P., {Luppino}, G.A., {Lupton},
  R.H., {Monet}, D.G., {Morgan}, J.S., {Onaka}, P.M., {Stubbs}, C.W., {Tonry},
  J.L., {Banados}, E., {Bell}, E.F., {Bender}, R., {Bernard}, E.J.,
  {Botticella}, M.T., {Casertano}, S., {Chastel}, S., {Chen}, W.P., {Chen}, X.,
  {Cole}, S., {Deacon}, N., {Frenk}, C., {Fitzsimmons}, A., {Gezari}, S.,
  {Goessl}, C., {Goggia}, T., {Goldman}, B., {Grebel}, E.K., {Hambly}, N.C.,
  {Hasinger}, G., {Heavens}, A.F., {Heckman}, T.M., {Henderson}, R., {Henning},
  T., {Holman}, M., {Hopp}, U., {Ip}, W.H., {Isani}, S., {Keyes}, C.D.,
  {Koekemoer}, A., {Kotak}, R., {Long}, K.S., {Lucey}, J.R., {Liu}, M.,
  {Martin}, N.F., {McLean}, B., {Morganson}, E., {Murphy}, D.N.A.,
  {Nieto-Santisteban}, M.A., {Norberg}, P., {Peacock}, J.A., {Pier}, E.A.,
  {Postman}, M., {Primak}, N., {Rae}, C., {Rest}, A., {Riess}, A., {Riffeser},
  A., {Rix}, H.W., {Roser}, S., {Schilbach}, E., {Schultz}, A.S.B., {Scolnic},
  D., {Szalay}, A., {Seitz}, S., {Shiao}, B., {Small}, E., {Smith}, K.W.,
  {Soderblom}, D., {Taylor}, A.N., {Thakar}, A.R., {Thiel}, J., {Thilker}, D.,
  {Urata}, Y., {Valenti}, J., {Walter}, F., {Watters}, S.P., {Werner}, S.,
  {White}, R., {Wood-Vasey}, W.M., {Wyse}, R.: {The Pan-STARRS1 Surveys}.
\newblock arxiv:1612.05560  (2016)

\bibitem{chandrasehkar43}
{Chandrasekhar}, S.: {Dynamical Friction. I. General Considerations: the
  Coefficient of Dynamical Friction.}
\newblock \apj \textbf{97}, 255 (1943).
\newblock \doi{10.1086/144517}

\bibitem{chang10}
{Chang}, S.H., {Gu}, P.G., {Bodenheimer}, P.H.: {Tidal and Magnetic
  Interactions Between a Hot Jupiter and its Host Star in the Magnetospheric
  Cavity of a Protoplanetary Disk}.
\newblock \apj \textbf{708}(2), 1692--1702 (2010).
\newblock \doi{10.1088/0004-637X/708/2/1692}

\bibitem{chapman07}
{Chapman}, C.R., {Cohen}, B.A., {Grinspoon}, D.H.: {What are the real
  constraints on the existence and magnitude of the late heavy bombardment?}
\newblock Icarus \textbf{189}, 233--245 (2007).
\newblock \doi{10.1016/j.icarus.2006.12.020}

\bibitem{chatterjee08}
{Chatterjee}, S., {Ford}, E.B., {Matsumura}, S., {Rasio}, F.A.: {Dynamical
  Outcomes of Planet-Planet Scattering}.
\newblock \apj \textbf{686}, 580--602 (2008).
\newblock \doi{10.1086/590227}

\bibitem{chatterjee14}
{Chatterjee}, S., {Tan}, J.C.: {Inside-out Planet Formation}.
\newblock \apj \textbf{780}, 53 (2014).
\newblock \doi{10.1088/0004-637X/780/1/53}

\bibitem{chatterjee15}
{Chatterjee}, S., {Tan}, J.C.: {Vulcan Planets: Inside-out Formation of the
  Innermost Super-Earths}.
\newblock \apjl \textbf{798}, L32 (2015).
\newblock \doi{10.1088/2041-8205/798/2/L32}

\bibitem{chen17}
{Chen}, J., {Kipping}, D.: {Probabilistic Forecasting of the Masses and Radii
  of Other Worlds}.
\newblock \apj \textbf{834}, 17 (2017).
\newblock \doi{10.3847/1538-4357/834/1/17}

\bibitem{chiang13}
{Chiang}, E., {Laughlin}, G.: {The minimum-mass extrasolar nebula: in situ
  formation of close-in super-Earths}.
\newblock \mnras \textbf{431}, 3444--3455 (2013).
\newblock \doi{10.1093/mnras/stt424}

\bibitem{chiang10}
{Chiang}, E., {Youdin}, A.N.: {Forming Planetesimals in Solar and Extrasolar
  Nebulae}.
\newblock Annual Review of Earth and Planetary Sciences \textbf{38}, 493--522
  (2010).
\newblock \doi{10.1146/annurev-earth-040809-152513}

\bibitem{chiang97}
{Chiang}, E.I., {Goldreich}, P.: {Spectral Energy Distributions of T Tauri
  Stars with Passive Circumstellar Disks}.
\newblock \apj \textbf{490}, 368 (1997).
\newblock \doi{10.1086/304869}

\bibitem{clanton14}
{Clanton}, C., {Gaudi}, B.S.: {Synthesizing Exoplanet Demographics from Radial
  Velocity and Microlensing Surveys. II. The Frequency of Planets Orbiting M
  Dwarfs}.
\newblock \apj \textbf{791}, 91 (2014).
\newblock \doi{10.1088/0004-637X/791/2/91}

\bibitem{clanton16}
{Clanton}, C., {Gaudi}, B.S.: {Synthesizing Exoplanet Demographics: A Single
  Population of Long-period Planetary Companions to M Dwarfs Consistent with
  Microlensing, Radial Velocity, and Direct Imaging Surveys}.
\newblock \apj \textbf{819}, 125 (2016).
\newblock \doi{10.3847/0004-637X/819/2/125}

\bibitem{clement19a}
{Clement}, M.S., {Kaib}, N.A., {Raymond}, S.N., {Chambers}, J.E., {Walsh},
  K.J.: {The early instability scenario: Terrestrial planet formation during
  the giant planet instability, and the effect of collisional fragmentation}.
\newblock \icarus \textbf{321}, 778--790 (2019).
\newblock \doi{10.1016/j.icarus.2018.12.033}

\bibitem{clement18}
{Clement}, M.S., {Kaib}, N.A., {Raymond}, S.N., {Walsh}, K.J.: {Mars' growth
  stunted by an early giant planet instability}.
\newblock \icarus \textbf{311}, 340--356 (2018).
\newblock \doi{10.1016/j.icarus.2018.04.008}

\bibitem{clement19b}
{Clement}, M.S., {Raymond}, S.N., {Kaib}, N.A.: {Excitation and Depletion of
  the Asteroid Belt in the Early Instability Scenario}.
\newblock \aj \textbf{157}(1), 38 (2019).
\newblock \doi{10.3847/1538-3881/aaf21e}

\bibitem{coleman17}
{Coleman}, G.A.L., {Papaloizou}, J.C.B., {Nelson}, R.P.: {In situ accretion of
  gaseous envelopes on to planetary cores embedded in evolving protoplanetary
  discs}.
\newblock \mnras \textbf{470}(3), 3206--3219 (2017).
\newblock \doi{10.1093/mnras/stx1297}

\bibitem{connelly08}
{Connelly}, J.N., {Amelin}, Y., {Krot}, A.N., {Bizzarro}, M.: {Chronology of
  the Solar System's Oldest Solids}.
\newblock \apjl \textbf{675}, L121 (2008).
\newblock \doi{10.1086/533586}

\bibitem{connelly12}
{Connelly}, J.N., {Bizzarro}, M., {Krot}, A.N., {Nordlund}, {\AA}., {Wielandt},
  D., {Ivanova}, M.A.: {The Absolute Chronology and Thermal Processing of
  Solids in the Solar Protoplanetary Disk}.
\newblock Science \textbf{338}, 651 (2012).
\newblock \doi{10.1126/science.1226919}

\bibitem{cossou14}
{Cossou}, C., {Raymond}, S.N., {Hersant}, F., {Pierens}, A.: {Hot super-Earths
  and giant planet cores from different migration histories}.
\newblock \aap \textbf{569}, A56 (2014).
\newblock \doi{10.1051/0004-6361/201424157}

\bibitem{cossou13}
{Cossou}, C., {Raymond}, S.N., {Pierens}, A.: {Convergence zones for Type I
  migration: an inward shift for multiple planet systems}.
\newblock \aap \textbf{553}, L2 (2013).
\newblock \doi{10.1051/0004-6361/201220853}

\bibitem{cresswell07}
{Cresswell}, P., {Dirksen}, G., {Kley}, W., {Nelson}, R.P.: {On the evolution
  of eccentric and inclined protoplanets embedded in protoplanetary disks}.
\newblock \aap \textbf{473}, 329--342 (2007).
\newblock \doi{10.1051/0004-6361:20077666}

\bibitem{crida06}
{Crida}, A., {Morbidelli}, A., {Masset}, F.: {On the width and shape of gaps in
  protoplanetary disks}.
\newblock Icarus \textbf{181}, 587--604 (2006).
\newblock \doi{10.1016/j.icarus.2005.10.007}

\bibitem{cumming08}
{Cumming}, A., {Butler}, R.P., {Marcy}, G.W., {Vogt}, S.S., {Wright}, J.T.,
  {Fischer}, D.A.: {The Keck Planet Search: Detectability and the Minimum Mass
  and Orbital Period Distribution of Extrasolar Planets}.
\newblock \pasp \textbf{120}, 531--554 (2008).
\newblock \doi{10.1086/588487}

\bibitem{dangelo03}
{D'Angelo}, G., {Kley}, W., {Henning}, T.: {Orbital Migration and Mass
  Accretion of Protoplanets in Three-dimensional Global Computations with
  Nested Grids}.
\newblock \apj \textbf{586}(1), 540--561 (2003).
\newblock \doi{10.1086/367555}

\bibitem{dangelo19}
{D'Angelo}, M., {Cazaux}, S., {Kamp}, I., {Thi}, W.F., {Woitke}, P.: {Water
  delivery in the inner solar nebula. Monte Carlo simulations of forsterite
  hydration}.
\newblock \aap \textbf{622}, A208 (2019).
\newblock \doi{10.1051/0004-6361/201833715}

\bibitem{dauphas17}
{Dauphas}, N.: {The isotopic nature of the Earth's accreting material through
  time}.
\newblock \nat \textbf{541}, 521--524 (2017).
\newblock \doi{10.1038/nature20830}

\bibitem{dauphas11}
{Dauphas}, N., {Pourmand}, A.: {Hf-W-Th evidence for rapid growth of Mars and
  its status as a planetary embryo}.
\newblock \nat \textbf{473}, 489--492 (2011).
\newblock \doi{10.1038/nature10077}

\bibitem{davis05}
{Davis}, S.S.: {The Surface Density Distribution in the Solar Nebula}.
\newblock \apjl \textbf{627}, L153--L155 (2005).
\newblock \doi{10.1086/432464}

\bibitem{dawson15}
{Dawson}, R.I., {Chiang}, E., {Lee}, E.J.: {A metallicity recipe for rocky
  planets}.
\newblock \mnras \textbf{453}, 1471--1483 (2015).
\newblock \doi{10.1093/mnras/stv1639}

\bibitem{dawson16}
{Dawson}, R.I., {Lee}, E.J., {Chiang}, E.: {Correlations between Compositions
  and Orbits Established by the Giant Impact Era of Planet Formation}.
\newblock \apj \textbf{822}, 54 (2016).
\newblock \doi{10.3847/0004-637X/822/1/54}

\bibitem{dawson13}
{Dawson}, R.I., {Murray-Clay}, R.A.: {Giant Planets Orbiting Metal-rich Stars
  Show Signatures of Planet-Planet Interactions}.
\newblock \apjl \textbf{767}, L24 (2013).
\newblock \doi{10.1088/2041-8205/767/2/L24}

\bibitem{deck15}
{Deck}, K.M., {Batygin}, K.: {Migration of Two Massive Planets into (and out
  of) First Order Mean Motion Resonances}.
\newblock \apj \textbf{810}(2), 119 (2015).
\newblock \doi{10.1088/0004-637X/810/2/119}

\bibitem{deienno16}
{Deienno}, R., {Gomes}, R.S., {Walsh}, K.J., {Morbidelli}, A., {Nesvorn{\'y}},
  D.: {Is the Grand Tack model compatible with the orbital distribution of main
  belt asteroids?}
\newblock \icarus \textbf{272}, 114--124 (2016).
\newblock \doi{10.1016/j.icarus.2016.02.043}

\bibitem{deienno18}
{Deienno}, R., {Izidoro}, A., {Morbidelli}, A., {Gomes}, R.S., {Nesvorn{\'y}},
  D., {Raymond}, S.N.: {Excitation of a Primordial Cold Asteroid Belt as an
  Outcome of Planetary Instability}.
\newblock \apj \textbf{864}, 50 (2018).
\newblock \doi{10.3847/1538-4357/aad55d}

\bibitem{demeo13}
{DeMeo}, F.E., {Carry}, B.: {The taxonomic distribution of asteroids from
  multi-filter all-sky photometric surveys}.
\newblock Icarus \textbf{226}, 723--741 (2013).
\newblock \doi{10.1016/j.icarus.2013.06.027}

\bibitem{demeo14}
{DeMeo}, F.E., {Carry}, B.: {Solar System evolution from compositional mapping
  of the asteroid belt}.
\newblock \nat \textbf{505}, 629--634 (2014).
\newblock \doi{10.1038/nature12908}

\bibitem{demory11}
{Demory}, B.O., {Gillon}, M., {Deming}, D., {Valencia}, D., {Seager}, S.,
  {Benneke}, B., {Lovis}, C., {Cubillos}, P., {Harrington}, J., {Stevenson},
  K.B., {Mayor}, M., {Pepe}, F., {Queloz}, D., {S{\'e}gransan}, D., {Udry}, S.:
  {Detection of a transit of the super-Earth 55 Cancri e with warm Spitzer}.
\newblock \aap \textbf{533}, A114 (2011).
\newblock \doi{10.1051/0004-6361/201117178}

\bibitem{desch15}
{Desch}, S.J., {Turner}, N.J.: {High-temperature Ionization in Protoplanetary
  Disks}.
\newblock \apj \textbf{811}(2), 156 (2015).
\newblock \doi{10.1088/0004-637X/811/2/156}

\bibitem{dodsonrobinson11}
{Dodson-Robinson}, S.E., {Salyk}, C.: {Transitional Disks as Signposts of
  Young, Multiplanet Systems}.
\newblock \apj \textbf{738}(2), 131 (2011).
\newblock \doi{10.1088/0004-637X/738/2/131}

\bibitem{dodsonrobinson09}
{Dodson-Robinson}, S.E., {Willacy}, K., {Bodenheimer}, P., {Turner}, N.J.,
  {Beichman}, C.A.: {Ice lines, planetesimal composition and solid surface
  density in the solar nebula}.
\newblock \icarus \textbf{200}(2), 672--693 (2009).
\newblock \doi{10.1016/j.icarus.2008.11.023}

\bibitem{dong13}
{Dong}, S., {Zhu}, Z.: {Fast Rise of ''Neptune-size'' Planets (4-8 R $_{⊕}$)
  from P \~{} 10 to \~{}250 Days -- Statistics of Kepler Planet Candidates up
  to \~{}0.75 AU}.
\newblock \apj \textbf{778}, 53 (2013).
\newblock \doi{10.1088/0004-637X/778/1/53}

\bibitem{dorn15}
{Dorn}, C., {Khan}, A., {Heng}, K., {Connolly}, J.A.D., {Alibert}, Y., {Benz},
  W., {Tackley}, P.: {Can we constrain the interior structure of rocky
  exoplanets from mass and radius measurements?}
\newblock \aap \textbf{577}, A83 (2015).
\newblock \doi{10.1051/0004-6361/201424915}

\bibitem{dorn18}
{Dorn}, C., {Mosegaard}, K., {Grimm}, S.L., {Alibert}, Y.: {Interior
  Characterization in Multiplanetary Systems: TRAPPIST-1}.
\newblock \apj \textbf{865}(1), 20 (2018).
\newblock \doi{10.3847/1538-4357/aad95d}

\bibitem{drazkowska17}
{Dr{\c a}{\.z}kowska}, J., {Alibert}, Y.: {Planetesimal formation starts at the
  snow line}.
\newblock \aap \textbf{608}, A92 (2017).
\newblock \doi{10.1051/0004-6361/201731491}

\bibitem{drazkowska16}
{Dr{\c a}{\.z}kowska}, J., {Alibert}, Y., {Moore}, B.: {Close-in planetesimal
  formation by pile-up of drifting pebbles}.
\newblock \aap \textbf{594}, A105 (2016).
\newblock \doi{10.1051/0004-6361/201628983}

\bibitem{drazkowska18}
{Dr{\k{a}}{\.z}kowska}, J., {Dullemond}, C.P.: {Planetesimal formation during
  protoplanetary disk buildup}.
\newblock \aap \textbf{614}, A62 (2018).
\newblock \doi{10.1051/0004-6361/201732221}

\bibitem{duffell14}
{Duffell}, P.C., {Haiman}, Z., {MacFadyen}, A.I., {D'Orazio}, D.J., {Farris},
  B.D.: {The Migration of Gap-opening Planets is Not Locked to Viscous Disk
  Evolution}.
\newblock \apjl \textbf{792}(1), L10 (2014).
\newblock \doi{10.1088/2041-8205/792/1/L10}

\bibitem{dullemond18}
{Dullemond}, C.P., {Birnstiel}, T., {Huang}, J., {Kurtovic}, N.T., {Andrews},
  S.M., {Guzm{\'a}n}, V.V., {P{\'e}rez}, L.M., {Isella}, A., {Zhu}, Z.,
  {Benisty}, M., {Wilner}, D.J., {Bai}, X.N., {Carpenter}, J.M., {Zhang}, S.,
  {Ricci}, L.: {The Disk Substructures at High Angular Resolution Project
  (DSHARP). VI. Dust Trapping in Thin-ringed Protoplanetary Disks}.
\newblock \apjl \textbf{869}(2), L46 (2018).
\newblock \doi{10.3847/2041-8213/aaf742}

\bibitem{durmann15}
{D{\"u}rmann}, C., {Kley}, W.: {Migration of massive planets in accreting
  disks}.
\newblock \aap \textbf{574}, A52 (2015).
\newblock \doi{10.1051/0004-6361/201424837}

\bibitem{eisner03}
{Eisner}, J.A., {Carpenter}, J.M.: {Distribution of Circumstellar Disk Masses
  in the Young Cluster NGC 2024}.
\newblock \apj \textbf{598}, 1341--1349 (2003).
\newblock \doi{10.1086/379102}

\bibitem{eklund17}
{Eklund}, H., {Masset}, F.S.: {Evolution of eccentricity and inclination of hot
  protoplanets embedded in radiative discs}.
\newblock \mnras \textbf{469}(1), 206--217 (2017).
\newblock \doi{10.1093/mnras/stx856}

\bibitem{ertel14}
{Ertel}, S., {Absil}, O., {Defr{\`e}re}, D., {Le Bouquin}, J.B., {Augereau},
  J.C., {Marion}, L., {Blind}, N., {Bonsor}, A., {Bryden}, G., {Lebreton}, J.,
  {Milli}, J.: {A near-infrared interferometric survey of debris-disk stars.
  IV. An unbiased sample of 92 southern stars observed in H band with
  VLTI/PIONIER}.
\newblock \aap \textbf{570}, A128 (2014).
\newblock \doi{10.1051/0004-6361/201424438}

\bibitem{fabrycky14}
{Fabrycky}, D.C., {Lissauer}, J.J., {Ragozzine}, D., {Rowe}, J.F., {Steffen},
  J.H., {Agol}, E., {Barclay}, T., {Batalha}, N., {Borucki}, W., {Ciardi},
  D.R., {Ford}, E.B., {Gautier}, T.N., {Geary}, J.C., {Holman}, M.J.,
  {Jenkins}, J.M., {Li}, J., {Morehead}, R.C., {Morris}, R.L., {Shporer}, A.,
  {Smith}, J.C., {Still}, M., {Van Cleve}, J.: {Architecture of Kepler's
  Multi-transiting Systems. II. New Investigations with Twice as Many
  Candidates}.
\newblock \apj \textbf{790}, 146 (2014).
\newblock \doi{10.1088/0004-637X/790/2/146}

\bibitem{fang12}
{Fang}, J., {Margot}, J.L.: {Architecture of Planetary Systems Based on Kepler
  Data: Number of Planets and Coplanarity}.
\newblock \apj \textbf{761}, 92 (2012).
\newblock \doi{10.1088/0004-637X/761/2/92}

\bibitem{fernandes19}
{Fernandes}, R.B., {Mulders}, G.D., {Pascucci}, I., {Mordasini}, C.,
  {Emsenhuber}, A.: {Hints for a Turnover at the Snow Line in the Giant Planet
  Occurrence Rate}.
\newblock \apj \textbf{874}(1), 81 (2019).
\newblock \doi{10.3847/1538-4357/ab0300}

\bibitem{fischer08}
{Fischer}, D.A., {Marcy}, G.W., {Butler}, R.P., {Vogt}, S.S., {Laughlin}, G.,
  {Henry}, G.W., {Abouav}, D., {Peek}, K.M.G., {Wright}, J.T., {Johnson}, J.A.,
  {McCarthy}, C., {Isaacson}, H.: {Five Planets Orbiting 55 Cancri}.
\newblock \apj \textbf{675}, 790--801 (2008).
\newblock \doi{10.1086/525512}

\bibitem{fischer05}
{Fischer}, D.A., {Valenti}, J.: {The Planet-Metallicity Correlation}.
\newblock \apj \textbf{622}, 1102--1117 (2005).
\newblock \doi{10.1086/428383}

\bibitem{fischer14b}
{Fischer}, R.A., {Ciesla}, F.J.: {Dynamics of the terrestrial planets from a
  large number of N-body simulations}.
\newblock Earth and Planetary Science Letters \textbf{392}, 28--38 (2014).
\newblock \doi{10.1016/j.epsl.2014.02.011}

\bibitem{fischer18}
{Fischer}, R.A., {Nimmo}, F.: {Effects of core formation on the Hf-W isotopic
  composition of the Earth and dating of the Moon-forming impact}.
\newblock Earth and Planetary Science Letters \textbf{499}, 257--265 (2018).
\newblock \doi{10.1016/j.epsl.2018.07.030}

\bibitem{flock17}
{Flock}, M., {Fromang}, S., {Turner}, N.J., {Benisty}, M.: {3D Radiation
  Nonideal Magnetohydrodynamical Simulations of the Inner Rim in Protoplanetary
  Disks}.
\newblock \apj \textbf{835}, 230 (2017).
\newblock \doi{10.3847/1538-4357/835/2/230}

\bibitem{flock19}
{Flock}, M., {Turner}, N.J., {Mulders}, G.D., {Hasegawa}, Y., {Nelson}, R.P.,
  {Bitsch}, B.: {Planet formation and migration near the silicate sublimation
  front in protoplanetary disks}.
\newblock \aap \textbf{630}, A147 (2019).
\newblock \doi{10.1051/0004-6361/201935806}

\bibitem{fogg05}
{Fogg}, M.J., {Nelson}, R.P.: {Oligarchic and giant impact growth of
  terrestrial planets in the presence of gas giant planet migration}.
\newblock \aap \textbf{441}, 791--806 (2005).
\newblock \doi{10.1051/0004-6361:20053453}

\bibitem{fogg07}
{Fogg}, M.J., {Nelson}, R.P.: {On the formation of terrestrial planets in
  hot-Jupiter systems}.
\newblock \aap \textbf{461}, 1195--1208 (2007).
\newblock \doi{10.1051/0004-6361:20066171}

\bibitem{ford08}
{Ford}, E.B., {Rasio}, F.A.: {Origins of Eccentric Extrasolar Planets: Testing
  the Planet-Planet Scattering Model}.
\newblock \apj \textbf{686}, 621--636 (2008).
\newblock \doi{10.1086/590926}

\bibitem{foremanmackey16}
{Foreman-Mackey}, D., {Morton}, T.D., {Hogg}, D.W., {Agol}, E.,
  {Sch{\"o}lkopf}, B.: {The Population of Long-period Transiting Exoplanets}.
\newblock \aj \textbf{152}, 206 (2016).
\newblock \doi{10.3847/0004-6256/152/6/206}

\bibitem{fortney07}
{Fortney}, J.J., {Marley}, M.S., {Barnes}, J.W.: {Planetary Radii across Five
  Orders of Magnitude in Mass and Stellar Insolation: Application to Transits}.
\newblock \apj \textbf{659}, 1661--1672 (2007).
\newblock \doi{10.1086/512120}

\bibitem{fressin13}
{Fressin}, F., {Torres}, G., {Charbonneau}, D., {Bryson}, S.T., {Christiansen},
  J., {Dressing}, C.D., {Jenkins}, J.M., {Walkowicz}, L.M., {Batalha}, N.M.:
  {The False Positive Rate of Kepler and the Occurrence of Planets}.
\newblock \apj \textbf{766}, 81 (2013).
\newblock \doi{10.1088/0004-637X/766/2/81}

\bibitem{fulton18}
{Fulton}, B.J., {Petigura}, E.A.: {The California Kepler Survey VII. Precise
  Planet Radii Leveraging Gaia DR2 Reveal the Stellar Mass Dependence of the
  Planet Radius Gap}.
\newblock ArXiv e-prints  (2018)

\bibitem{fulton17}
{Fulton}, B.J., {Petigura}, E.A., {Howard}, A.W., {Isaacson}, H., {Marcy},
  G.W., {Cargile}, P.A., {Hebb}, L., {Weiss}, L.M., {Johnson}, J.A., {Morton},
  T.D., {Sinukoff}, E., {Crossfield}, I.J.M., {Hirsch}, L.A.: {The
  California-Kepler Survey. III. A Gap in the Radius Distribution of Small
  Planets}.
\newblock \aj \textbf{154}, 109 (2017).
\newblock \doi{10.3847/1538-3881/aa80eb}

\bibitem{genda05}
{Genda}, H., {Abe}, Y.: {Enhanced atmospheric loss on protoplanets at the giant
  impact phase in the presence of oceans}.
\newblock \nat \textbf{433}, 842--844 (2005).
\newblock \doi{10.1038/nature03360}

\bibitem{genda08}
{Genda}, H., {Ikoma}, M.: {Origin of the ocean on the Earth: Early evolution of
  water D/H in a hydrogen-rich atmosphere}.
\newblock \icarus \textbf{194}(1), 42--52 (2008).
\newblock \doi{10.1016/j.icarus.2007.09.007}

\bibitem{gillon17}
{Gillon}, M., {Triaud}, A.H.M.J., {Demory}, B.O., {Jehin}, E., {Agol}, E.,
  {Deck}, K.M., {Lederer}, S.M., {de Wit}, J., {Burdanov}, A., {Ingalls}, J.G.,
  {Bolmont}, E., {Leconte}, J., {Raymond}, S.N., {Selsis}, F., {Turbet}, M.,
  {Barkaoui}, K., {Burgasser}, A., {Burleigh}, M.R., {Carey}, S.J., {Chaushev},
  A., {Copperwheat}, C.M., {Delrez}, L., {Fernandes}, C.S., {Holdsworth}, D.L.,
  {Kotze}, E.J., {Van Grootel}, V., {Almleaky}, Y., {Benkhaldoun}, Z.,
  {Magain}, P., {Queloz}, D.: {Seven temperate terrestrial planets around the
  nearby ultracool dwarf star TRAPPIST-1}.
\newblock \nat \textbf{542}, 456--460 (2017).
\newblock \doi{10.1038/nature21360}

\bibitem{ginzburg16}
{Ginzburg}, S., {Schlichting}, H.E., {Sari}, R.: {Super-Earth Atmospheres:
  Self-consistent Gas Accretion and Retention}.
\newblock \apj \textbf{825}, 29 (2016).
\newblock \doi{10.3847/0004-637X/825/1/29}

\bibitem{goldreich14}
{Goldreich}, P., {Schlichting}, H.E.: {Overstable Librations can Account for
  the Paucity of Mean Motion Resonances among Exoplanet Pairs}.
\newblock \aj \textbf{147}(2), 32 (2014).
\newblock \doi{10.1088/0004-6256/147/2/32}

\bibitem{goldreich79}
{Goldreich}, P., {Tremaine}, S.: {The excitation of density waves at the
  Lindblad and corotation resonances by an external potential.}
\newblock \apj \textbf{233}, 857--871 (1979).
\newblock \doi{10.1086/157448}

\bibitem{goldreich80}
{Goldreich}, P., {Tremaine}, S.: {Disk-satellite interactions}.
\newblock \apj \textbf{241}, 425--441 (1980).
\newblock \doi{10.1086/158356}

\bibitem{gomes05}
{Gomes}, R., {Levison}, H.F., {Tsiganis}, K., {Morbidelli}, A.: {Origin of the
  cataclysmic Late Heavy Bombardment period of the terrestrial planets}.
\newblock \nat \textbf{435}, 466--469 (2005).
\newblock \doi{10.1038/nature03676}

\bibitem{gomes04}
{Gomes}, R.S., {Morbidelli}, A., {Levison}, H.F.: {Planetary migration in a
  planetesimal disk: why did Neptune stop at 30 AU?}
\newblock Icarus \textbf{170}, 492--507 (2004).
\newblock \doi{10.1016/j.icarus.2004.03.011}

\bibitem{gonzalez97}
{Gonzalez}, G.: {The stellar metallicity-giant planet connection}.
\newblock \mnras \textbf{285}, 403--412 (1997)

\bibitem{gould10}
{Gould}, A., {Dong}, S., {Gaudi}, B.S., {Udalski}, A., {Bond}, I.A.,
  {Greenhill}, J., {Street}, R.A., {Dominik}, M., {Sumi}, T., {Szyma{\'n}ski},
  M.K., {Han}, C., {Allen}, W., {Bolt}, G., {Bos}, M., {Christie}, G.W.,
  {DePoy}, D.L., {Drummond}, J., {Eastman}, J.D., {Gal-Yam}, A., {Higgins}, D.,
  {Janczak}, J., {Kaspi}, S., {Koz{\l}owski}, S., {Lee}, C., {Mallia}, F.,
  {Maury}, A., {Maoz}, D., {McCormick}, J., {Monard}, L.A.G., {Moorhouse}, D.,
  {Morgan}, N., {Natusch}, T., {Ofek}, E.O., {Park}, B., {Pogge}, R.W.,
  {Polishook}, D., {Santallo}, R., {Shporer}, A., {Spector}, O., {Thornley},
  G., {Yee}, J.C., {{$\mu$}FUN Collaboration}, {Kubiak}, M., {Pietrzy{\'n}ski},
  G., {Soszy{\'n}ski}, I., {Szewczyk}, O., {Wyrzykowski}, {\L}., {Ulaczyk}, K.,
  {Poleski}, R., {OGLE Collaboration}, {Abe}, F., {Bennett}, D.P., {Botzler},
  C.S., {Douchin}, D., {Freeman}, M., {Fukui}, A., {Furusawa}, K., {Hearnshaw},
  J.B., {Hosaka}, S., {Itow}, Y., {Kamiya}, K., {Kilmartin}, P.M., {Korpela},
  A., {Lin}, W., {Ling}, C.H., {Makita}, S., {Masuda}, K., {Matsubara}, Y.,
  {Miyake}, N., {Muraki}, Y., {Nagaya}, M., {Nishimoto}, K., {Ohnishi}, K.,
  {Okumura}, T., {Perrott}, Y.C., {Philpott}, L., {Rattenbury}, N., {Saito},
  T., {Sako}, T., {Sullivan}, D.J., {Sweatman}, W.L., {Tristram}, P.J., {von
  Seggern}, E., {Yock}, P.C.M., {MOA Collaboration}, {Albrow}, M., {Batista},
  V., {Beaulieu}, J.P., {Brillant}, S., {Caldwell}, J., {Calitz}, J.J.,
  {Cassan}, A., {Cole}, A., {Cook}, K., {Coutures}, C., {Dieters}, S., {Dominis
  Prester}, D., {Donatowicz}, J., {Fouqu{\'e}}, P., {Hill}, K., {Hoffman}, M.,
  {Jablonski}, F., {Kane}, S.R., {Kains}, N., {Kubas}, D., {Marquette}, J.,
  {Martin}, R., {Martioli}, E., {Meintjes}, P., {Menzies}, J., {Pedretti}, E.,
  {Pollard}, K., {Sahu}, K.C., {Vinter}, C., {Wambsganss}, J., {Watson}, R.,
  {Williams}, A., {Zub}, M., {PLANET Collaboration}, {Allan}, A., {Bode}, M.F.,
  {Bramich}, D.M., {Burgdorf}, M.J., {Clay}, N., {Fraser}, S., {Hawkins}, E.,
  {Horne}, K., {Kerins}, E., {Lister}, T.A., {Mottram}, C., {Saunders}, E.S.,
  {Snodgrass}, C., {Steele}, I.A., {Tsapras}, Y., {RoboNet Collaboration},
  {J{\o}rgensen}, U.G., {Anguita}, T., {Bozza}, V., {Calchi Novati}, S.,
  {Harps{\o}e}, K., {Hinse}, T.C., {Hundertmark}, M., {Kj{\ae}rgaard}, P.,
  {Liebig}, C., {Mancini}, L., {Masi}, G., {Mathiasen}, M., {Rahvar}, S.,
  {Ricci}, D., {Scarpetta}, G., {Southworth}, J., {Surdej}, J., {Th{\"o}ne},
  C.C., {MiNDSTEp Consortium}: {Frequency of Solar-like Systems and of Ice and
  Gas Giants Beyond the Snow Line from High-magnification Microlensing Events
  in 2005-2008}.
\newblock \apj \textbf{720}, 1073--1089 (2010).
\newblock \doi{10.1088/0004-637X/720/2/1073}

\bibitem{gradie82}
{Gradie}, J., {Tedesco}, E.: {Compositional structure of the asteroid belt}.
\newblock Science \textbf{216}, 1405--1407 (1982).
\newblock \doi{10.1126/science.216.4553.1405}

\bibitem{greaves11}
{Greaves}, J.S., {Rice}, W.K.M.: {Do all Sun-like stars have planets?
  Inferences from the disc mass reservoirs of Class 0 protostars}.
\newblock \mnras \textbf{412}(1), L88--L92 (2011).
\newblock \doi{10.1111/j.1745-3933.2011.01011.x}

\bibitem{greenberg78}
{Greenberg}, R., {Hartmann}, W.K., {Chapman}, C.R., {Wacker}, J.F.:
  {Planetesimals to planets - Numerical simulation of collisional evolution}.
\newblock Icarus \textbf{35}, 1--26 (1978).
\newblock \doi{10.1016/0019-1035(78)90057-X}

\bibitem{gressel15}
{Gressel}, O., {Turner}, N.J., {Nelson}, R.P., {McNally}, C.P.: {Global
  Simulations of Protoplanetary Disks With Ohmic Resistivity and Ambipolar
  Diffusion}.
\newblock \apj \textbf{801}(2), 84 (2015).
\newblock \doi{10.1088/0004-637X/801/2/84}

\bibitem{grimm93}
{Grimm}, R.E., {McSween}, H.Y.: {Heliocentric zoning of the asteroid belt by
  aluminum-26 heating}.
\newblock Science \textbf{259}, 653--655 (1993)

\bibitem{grishin15}
{Grishin}, E., {Perets}, H.B.: {Application of Gas Dynamical Friction for
  Planetesimals. I. Evolution of Single Planetesimals}.
\newblock \apj \textbf{811}(1), 54 (2015).
\newblock \doi{10.1088/0004-637X/811/1/54}

\bibitem{gupta19}
{Gupta}, A., {Schlichting}, H.E.: {Sculpting the valley in the radius
  distribution of small exoplanets as a by-product of planet formation: the
  core-powered mass-loss mechanism}.
\newblock \mnras \textbf{487}(1), 24--33 (2019).
\newblock \doi{10.1093/mnras/stz1230}

\bibitem{hahn09}
Hahn, J.M.: The Dynamics of Planetary Systems and Astrophysical Disks.
\newblock WILEY-VCH (2009)

\bibitem{haisch01}
{Haisch} Jr., K.E., {Lada}, E.A., {Lada}, C.J.: {Disk Frequencies and Lifetimes
  in Young Clusters}.
\newblock \apjl \textbf{553}, L153--L156 (2001).
\newblock \doi{10.1086/320685}

\bibitem{halliday13}
{Halliday}, A.N.: {The origins of volatiles in the terrestrial planets}.
\newblock \gca \textbf{105}, 146--171 (2013).
\newblock \doi{10.1016/j.gca.2012.11.015}

\bibitem{halliday06}
{Halliday}, A.N., {Kleine}, T.: {Meteorites and the Timing, Mechanisms, and
  Conditions of Terrestrial Planet Accretion and Early Differentiation}, pp.
  775--801 (2006)

\bibitem{hansen09}
{Hansen}, B.M.S.: {Formation of the Terrestrial Planets from a Narrow Annulus}.
\newblock \apj \textbf{703}, 1131--1140 (2009).
\newblock \doi{10.1088/0004-637X/703/1/1131}

\bibitem{hansen12}
{Hansen}, B.M.S., {Murray}, N.: {Migration Then Assembly: Formation of
  Neptune-mass Planets inside 1 AU}.
\newblock \apj \textbf{751}, 158 (2012).
\newblock \doi{10.1088/0004-637X/751/2/158}

\bibitem{hansen13}
{Hansen}, B.M.S., {Murray}, N.: {Testing in Situ Assembly with the Kepler
  Planet Candidate Sample}.
\newblock \apj \textbf{775}, 53 (2013).
\newblock \doi{10.1088/0004-637X/775/1/53}

\bibitem{hartmann98}
{Hartmann}, L., {Calvet}, N., {Gullbring}, E., {D'Alessio}, P.: {Accretion and
  the Evolution of T Tauri Disks}.
\newblock \apj \textbf{495}, 385--400 (1998).
\newblock \doi{10.1086/305277}

\bibitem{hartmann19}
{Hartmann}, W.K.: {The Collapse of the Terminal Cataclysm Paradigm...and Where
  We Go from Here}.
\newblock In: Lunar and Planetary Science Conference, Lunar and Planetary
  Science Conference, p. 1064 (2019)

\bibitem{hartogh11}
{Hartogh}, P., {Lis}, D.C., {Bockel{\'e}e-Morvan}, D., {de Val-Borro}, M.,
  {Biver}, N., {K{\"u}ppers}, M., {Emprechtinger}, M., {Bergin}, E.A.,
  {Crovisier}, J., {Rengel}, M., {Moreno}, R., {Szutowicz}, S., {Blake}, G.A.:
  {Ocean-like water in the Jupiter-family comet 103P/Hartley 2}.
\newblock \nat \textbf{478}, 218--220 (2011).
\newblock \doi{10.1038/nature10519}

\bibitem{hasegawa12}
{Hasegawa}, Y., {Pudritz}, R.E.: {Evolutionary Tracks of Trapped, Accreting
  Protoplanets: The Origin of the Observed Mass-Period Relation}.
\newblock \apj \textbf{760}, 117 (2012).
\newblock \doi{10.1088/0004-637X/760/2/117}

\bibitem{hayashi81}
{Hayashi}, C.: {Structure of the Solar Nebula, Growth and Decay of Magnetic
  Fields and Effects of Magnetic and Turbulent Viscosities on the Nebula}.
\newblock Progress of Theoretical Physics Supplement \textbf{70}, 35--53
  (1981).
\newblock \doi{10.1143/PTPS.70.35}

\bibitem{helled14}
{Helled}, R., {Bodenheimer}, P., {Podolak}, M., {Boley}, A., {Meru}, F.,
  {Nayakshin}, S., {Fortney}, J.J., {Mayer}, L., {Alibert}, Y., {Boss}, A.P.:
  {Giant Planet Formation, Evolution, and Internal Structure}.
\newblock Protostars and Planets VI pp. 643--665 (2014)

\bibitem{henon64}
{Henon}, M., {Heiles}, C.: {The applicability of the third integral of motion:
  Some numerical experiments}.
\newblock \aj \textbf{69}, 73 (1964).
\newblock \doi{10.1086/109234}

\bibitem{hillenbrand08}
{Hillenbrand}, L.A., {Carpenter}, J.M., {Kim}, J.S., {Meyer}, M.R., {Backman},
  D.E., {Moro-Mart{\'{\i}}n}, A., {Hollenbach}, D.J., {Hines}, D.C.,
  {Pascucci}, I., {Bouwman}, J.: {The Complete Census of 70 {$\mu$}m-bright
  Debris Disks within ``the Formation and Evolution of Planetary Systems''
  Spitzer Legacy Survey of Sun-like Stars}.
\newblock \apj \textbf{677}, 630--656 (2008).
\newblock \doi{10.1086/529027}

\bibitem{hirschmann06}
{Hirschmann}, M.M.: {Water, Melting, and the Deep Earth H2O Cycle}.
\newblock Annual Review of Earth and Planetary Sciences \textbf{34}, 629--653
  (2006).
\newblock \doi{10.1146/annurev.earth.34.031405.125211}

\bibitem{hollenbach94}
{Hollenbach}, D., {Johnstone}, D., {Lizano}, S., {Shu}, F.: {Photoevaporation
  of disks around massive stars and application to ultracompact H II regions}.
\newblock \apj \textbf{428}, 654--669 (1994).
\newblock \doi{10.1086/174276}

\bibitem{howard12}
{Howard}, A.W., {Marcy}, G.W., {Bryson}, S.T., {Jenkins}, J.M., {Rowe}, J.F.,
  {Batalha}, N.M., {Borucki}, W.J., {Koch}, D.G., {Dunham}, E.W., {Gautier}
  III, T.N., {Van Cleve}, J., {Cochran}, W.D., {Latham}, D.W., {Lissauer},
  J.J., {Torres}, G., {Brown}, T.M., {Gilliland}, R.L., {Buchhave}, L.A.,
  {Caldwell}, D.A., {Christensen-Dalsgaard}, J., {Ciardi}, D., {Fressin}, F.,
  {Haas}, M.R., {Howell}, S.B., {Kjeldsen}, H., {Seager}, S., {Rogers}, L.,
  {Sasselov}, D.D., {Steffen}, J.H., {Basri}, G.S., {Charbonneau}, D.,
  {Christiansen}, J., {Clarke}, B., {Dupree}, A., {Fabrycky}, D.C., {Fischer},
  D.A., {Ford}, E.B., {Fortney}, J.J., {Tarter}, J., {Girouard}, F.R.,
  {Holman}, M.J., {Johnson}, J.A., {Klaus}, T.C., {Machalek}, P., {Moorhead},
  A.V., {Morehead}, R.C., {Ragozzine}, D., {Tenenbaum}, P., {Twicken}, J.D.,
  {Quinn}, S.N., {Isaacson}, H., {Shporer}, A., {Lucas}, P.W., {Walkowicz},
  L.M., {Welsh}, W.F., {Boss}, A., {Devore}, E., {Gould}, A., {Smith}, J.C.,
  {Morris}, R.L., {Prsa}, A., {Morton}, T.D., {Still}, M., {Thompson}, S.E.,
  {Mullally}, F., {Endl}, M., {MacQueen}, P.J.: {Planet Occurrence within 0.25
  AU of Solar-type Stars from Kepler}.
\newblock \apjs \textbf{201}, 15 (2012).
\newblock \doi{10.1088/0067-0049/201/2/15}

\bibitem{howard10}
{Howard}, A.W., {Marcy}, G.W., {Johnson}, J.A., {Fischer}, D.A., {Wright},
  J.T., {Isaacson}, H., {Valenti}, J.A., {Anderson}, J., {Lin}, D.N.C., {Ida},
  S.: {The Occurrence and Mass Distribution of Close-in Super-Earths, Neptunes,
  and Jupiters}.
\newblock Science \textbf{330}, 653-- (2010).
\newblock \doi{10.1126/science.1194854}

\bibitem{hu17}
{Hu}, X., {Tan}, J.C., {Zhu}, Z., {Chatterjee}, S., {Birnstiel}, T., {Youdin},
  A.N., {Mohanty}, S.: {Inside-Out Planet Formation. IV. Pebble Evolution and
  Planet Formation Timescales}.
\newblock ArXiv e-prints  (2017)

\bibitem{hu16}
{Hu}, X., {Zhu}, Z., {Tan}, J.C., {Chatterjee}, S.: {Inside-out Planet
  Formation. III. Planet-Disk Interaction at the Dead Zone Inner Boundary}.
\newblock \apj \textbf{816}, 19 (2016).
\newblock \doi{10.3847/0004-637X/816/1/19}

\bibitem{hubickyj05}
{Hubickyj}, O., {Bodenheimer}, P., {Lissauer}, J.J.: {Accretion of the gaseous
  envelope of Jupiter around a 5 10 Earth-mass core}.
\newblock Icarus \textbf{179}, 415--431 (2005).
\newblock \doi{10.1016/j.icarus.2005.06.021}

\bibitem{hughes18}
{Hughes}, A.M., {Duch{\^e}ne}, G., {Matthews}, B.C.: {Debris Disks: Structure,
  Composition, and Variability}.
\newblock \araa \textbf{56}, 541--591 (2018).
\newblock \doi{10.1146/annurev-astro-081817-052035}

\bibitem{ida16b}
{Ida}, S., {Guillot}, T.: {Formation of dust-rich planetesimals from sublimated
  pebbles inside of the snow line}.
\newblock \aap \textbf{596}, L3 (2016).
\newblock \doi{10.1051/0004-6361/201629680}

\bibitem{ida16}
{Ida}, S., {Guillot}, T., {Morbidelli}, A.: {The radial dependence of pebble
  accretion rates: A source of diversity in planetary systems. I. Analytical
  formulation}.
\newblock \aap \textbf{591}, A72 (2016).
\newblock \doi{10.1051/0004-6361/201628099}

\bibitem{ida04}
{Ida}, S., {Lin}, D.N.C.: {Toward a Deterministic Model of Planetary Formation.
  I. A Desert in the Mass and Semimajor Axis Distributions of Extrasolar
  Planets}.
\newblock \apj \textbf{604}, 388--413 (2004).
\newblock \doi{10.1086/381724}

\bibitem{ida08}
{Ida}, S., {Lin}, D.N.C.: {Toward a Deterministic Model of Planetary Formation.
  IV. Effects of Type I Migration}.
\newblock \apj \textbf{673}, 487--501 (2008).
\newblock \doi{10.1086/523754}

\bibitem{ida10}
{Ida}, S., {Lin}, D.N.C.: {Toward a Deterministic Model of Planetary Formation.
  VI. Dynamical Interaction and Coagulation of Multiple Rocky Embryos and
  Super-Earth Systems around Solar-type Stars}.
\newblock \apj \textbf{719}, 810--830 (2010).
\newblock \doi{10.1088/0004-637X/719/1/810}

\bibitem{ida13}
{Ida}, S., {Lin}, D.N.C., {Nagasawa}, M.: {Toward a Deterministic Model of
  Planetary Formation. VII. Eccentricity Distribution of Gas Giants}.
\newblock \apj \textbf{775}, 42 (2013).
\newblock \doi{10.1088/0004-637X/775/1/42}

\bibitem{ida19}
{Ida}, S., {Yamamura}, T., {Okuzumi}, S.: {Water delivery by pebble accretion
  to rocky planets in habitable zones in evolving disks}.
\newblock \aap \textbf{624}, A28 (2019).
\newblock \doi{10.1051/0004-6361/201834556}

\bibitem{ikoma06}
{Ikoma}, M., {Genda}, H.: {Constraints on the Mass of a Habitable Planet with
  Water of Nebular Origin}.
\newblock \apj \textbf{648}(1), 696--706 (2006).
\newblock \doi{10.1086/505780}

\bibitem{ikoma00}
{Ikoma}, M., {Nakazawa}, K., {Emori}, H.: {Formation of Giant Planets:
  Dependences on Core Accretion Rate and Grain Opacity}.
\newblock \apj \textbf{537}, 1013--1025 (2000).
\newblock \doi{10.1086/309050}

\bibitem{inamdar15}
{Inamdar}, N.K., {Schlichting}, H.E.: {The formation of super-Earths and
  mini-Neptunes with giant impacts}.
\newblock \mnras \textbf{448}, 1751--1760 (2015).
\newblock \doi{10.1093/mnras/stv030}

\bibitem{izidoro19}
{Izidoro}, A., {Bitsch}, B., {Raymond}, S.N., {Johansen}, A., {Morbidelli}, A.,
  {Lambrechts}, M., {Jacobson}, S.A.: {Formation of planetary systems by pebble
  accretion and migration: Hot super-Earth systems from breaking compact
  resonant chains}.
\newblock arXiv e-prints arXiv:1902.08772 (2019)

\bibitem{izidoro14}
{Izidoro}, A., {Morbidelli}, A., {Raymond}, S.N.: {Terrestrial Planet Formation
  in the Presence of Migrating Super-Earths}.
\newblock \apj \textbf{794}, 11 (2014).
\newblock \doi{10.1088/0004-637X/794/1/11}

\bibitem{izidoro15b}
{Izidoro}, A., {Morbidelli}, A., {Raymond}, S.N., {Hersant}, F., {Pierens}, A.:
  {Accretion of Uranus and Neptune from inward-migrating planetary embryos
  blocked by Jupiter and Saturn}.
\newblock \aap \textbf{582}, A99 (2015).
\newblock \doi{10.1051/0004-6361/201425525}

\bibitem{izidoro17}
{Izidoro}, A., {Ogihara}, M., {Raymond}, S.N., {Morbidelli}, A., {Pierens}, A.,
  {Bitsch}, B., {Cossou}, C., {Hersant}, F.: {Breaking the chains: hot
  super-Earth systems from migration and disruption of compact resonant
  chains}.
\newblock \mnras \textbf{470}, 1750--1770 (2017).
\newblock \doi{10.1093/mnras/stx1232}

\bibitem{izidoro15a}
{Izidoro}, A., {Raymond}, S.N., {Morbidelli}, A., {Hersant}, F., {Pierens}, A.:
  {Gas Giant Planets as Dynamical Barriers to Inward-Migrating Super-Earths}.
\newblock \apjl \textbf{800}, L22 (2015).
\newblock \doi{10.1088/2041-8205/800/2/L22}

\bibitem{izidoro15c}
{Izidoro}, A., {Raymond}, S.N., {Morbidelli}, A., {Winter}, O.C.: {Terrestrial
  planet formation constrained by Mars and the structure of the asteroid belt}.
\newblock \mnras \textbf{453}, 3619--3634 (2015).
\newblock \doi{10.1093/mnras/stv1835}

\bibitem{jacobson14b}
{Jacobson}, S.A., {Morbidelli}, A.: {Lunar and terrestrial planet formation in
  the Grand Tack scenario}.
\newblock Philosophical Transactions of the Royal Society of London Series A
  \textbf{372}, 0174 (2014).
\newblock \doi{10.1098/rsta.2013.0174}

\bibitem{jacobson14}
{Jacobson}, S.A., {Morbidelli}, A., {Raymond}, S.N., {O'Brien}, D.P., {Walsh},
  K.J., {Rubie}, D.C.: {Highly siderophile elements in Earth's mantle as a
  clock for the Moon-forming impact}.
\newblock \nat \textbf{508}, 84--87 (2014).
\newblock \doi{10.1038/nature13172}

\bibitem{jacquet11}
{Jacquet}, E., {Balbus}, S., {Latter}, H.: {On linear dust-gas streaming
  instabilities in protoplanetary discs}.
\newblock \mnras \textbf{415}(4), 3591--3598 (2011).
\newblock \doi{10.1111/j.1365-2966.2011.18971.x}

\bibitem{jin18}
{Jin}, S., {Mordasini}, C.: {Compositional Imprints in Density--Distance--Time:
  A Rocky Composition for Close-in Low-mass Exoplanets from the Location of the
  Valley of Evaporation}.
\newblock \apj \textbf{853}, 163 (2018).
\newblock \doi{10.3847/1538-4357/aa9f1e}

\bibitem{johansen14}
{Johansen}, A., {Blum}, J., {Tanaka}, H., {Ormel}, C., {Bizzarro}, M.,
  {Rickman}, H.: {The Multifaceted Planetesimal Formation Process}.
\newblock Protostars and Planets VI pp. 547--570 (2014)

\bibitem{johansen12}
{Johansen}, A., {Davies}, M.B., {Church}, R.P., {Holmelin}, V.: {Can Planetary
  Instability Explain the Kepler Dichotomy?}
\newblock \apj \textbf{758}, 39 (2012).
\newblock \doi{10.1088/0004-637X/758/1/39}

\bibitem{johansen17}
{Johansen}, A., {Lambrechts}, M.: {Forming Planets via Pebble Accretion}.
\newblock Annual Review of Earth and Planetary Sciences \textbf{45}, 359--387
  (2017).
\newblock \doi{10.1146/annurev-earth-063016-020226}

\bibitem{johansen15}
{Johansen}, A., {Mac Low}, M.M., {Lacerda}, P., {Bizzarro}, M.: {Growth of
  asteroids, planetary embryos, and Kuiper belt objects by chondrule
  accretion}.
\newblock Science Advances \textbf{1}, 1500109 (2015).
\newblock \doi{10.1126/sciadv.1500109}

\bibitem{johansen09}
{Johansen}, A., {Youdin}, A., {Klahr}, H.: {Zonal Flows and Long-lived
  Axisymmetric Pressure Bumps in Magnetorotational Turbulence}.
\newblock \apj \textbf{697}, 1269--1289 (2009).
\newblock \doi{10.1088/0004-637X/697/2/1269}

\bibitem{johnson16}
Johnson, B.C., Walsh, K.J., Minton, D.A., Krot, A.N., Levison, H.F.: Timing of
  the formation and migration of giant planets as constrained by cb chondrites.
\newblock Science Advances \textbf{2}(12) (2016).
\newblock \doi{10.1126/sciadv.1601658}.
\newblock \urlprefix\url{http://advances.sciencemag.org/content/2/12/e1601658}

\bibitem{johnson07}
{Johnson}, J.A., {Butler}, R.P., {Marcy}, G.W., {Fischer}, D.A., {Vogt}, S.S.,
  {Wright}, J.T., {Peek}, K.M.G.: {A New Planet around an M Dwarf: Revealing a
  Correlation between Exoplanets and Stellar Mass}.
\newblock \apj \textbf{670}, 833--840 (2007).
\newblock \doi{10.1086/521720}

\bibitem{jones06}
{Jones}, H.R.A., {Butler}, R.P., {Tinney}, C.G., {Marcy}, G.W., {Carter}, B.D.,
  {Penny}, A.J., {McCarthy}, C., {Bailey}, J.: {High-eccentricity planets from
  the Anglo-Australian Planet Search}.
\newblock \mnras \textbf{369}, 249--256 (2006).
\newblock \doi{10.1111/j.1365-2966.2006.10298.x}

\bibitem{juric08}
{Juri{\'c}}, M., {Tremaine}, S.: {Dynamical Origin of Extrasolar Planet
  Eccentricity Distribution}.
\newblock \apj \textbf{686}, 603--620 (2008).
\newblock \doi{10.1086/590047}

\bibitem{kaib16}
{Kaib}, N.A., {Chambers}, J.E.: {The fragility of the terrestrial planets
  during a giant-planet instability}.
\newblock \mnras \textbf{455}, 3561--3569 (2016).
\newblock \doi{10.1093/mnras/stv2554}

\bibitem{kaib15}
{Kaib}, N.A., {Cowan}, N.B.: {The feeding zones of terrestrial planets and
  insights into Moon formation}.
\newblock \icarus \textbf{252}, 161--174 (2015).
\newblock \doi{10.1016/j.icarus.2015.01.013}

\bibitem{kaib13}
{Kaib}, N.A., {Raymond}, S.N., {Duncan}, M.: {Planetary system disruption by
  Galactic perturbations to wide binary stars}.
\newblock \nat \textbf{493}, 381--384 (2013).
\newblock \doi{10.1038/nature11780}

\bibitem{kanagawa15}
{Kanagawa}, K.D., {Tanaka}, H., {Muto}, T., {Tanigawa}, T., {Takeuchi}, T.:
  {Formation of a disc gap induced by a planet: effect of the deviation from
  Keplerian disc rotation}.
\newblock \mnras \textbf{448}(1), 994--1006 (2015).
\newblock \doi{10.1093/mnras/stv025}

\bibitem{kanagawa18}
{Kanagawa}, K.D., {Tanaka}, H., {Szuszkiewicz}, E.: {Radial Migration of
  Gap-opening Planets in Protoplanetary Disks. I. The Case of a Single Planet}.
\newblock \apj \textbf{861}(2), 140 (2018).
\newblock \doi{10.3847/1538-4357/aac8d9}

\bibitem{kataoka13}
{Kataoka}, A., {Tanaka}, H., {Okuzumi}, S., {Wada}, K.: {Fluffy dust forms icy
  planetesimals by static compression}.
\newblock \aap \textbf{557}, L4 (2013).
\newblock \doi{10.1051/0004-6361/201322151}

\bibitem{kerridge85}
{Kerridge}, J.F.: {Carbon, hydrogen and nitrogen in carbonaceous chondrites
  Abundances and isotopic compositions in bulk samples}.
\newblock \gca \textbf{49}, 1707--1714 (1985).
\newblock \doi{10.1016/0016-7037(85)90141-3}

\bibitem{kimura74}
{Kimura}, K., {Lewis}, R.S., {Anders}, E.: {Distribution of gold and rhenium
  between nickel-iron and silicate melts: implications for the abundance of
  siderophile elements on the Earth and Moon}.
\newblock \gca \textbf{38}, 683--701 (1974).
\newblock \doi{10.1016/0016-7037(74)90144-6}

\bibitem{kimura12}
{Kimura}, S.S., {Tsuribe}, T.: {Conditions of Gravitational Instability in
  Protoplanetary Disks}.
\newblock \pasj \textbf{64}, 116 (2012).
\newblock \doi{10.1093/pasj/64.5.116}

\bibitem{kita05}
{Kita}, N.T., {Huss}, G.R., {Tachibana}, S., {Amelin}, Y., {Nyquist}, L.E.,
  {Hutcheon}, I.D.: {Constraints on the Origin of Chondrules and CAIs from
  Short-lived and Long-Lived Radionuclides}.
\newblock In: A.N. {Krot}, E.R.D. {Scott}, B.~{Reipurth} (eds.) Chondrites and
  the Protoplanetary Disk, \emph{Astronomical Society of the Pacific Conference
  Series}, vol. 341, p. 558 (2005)

\bibitem{kleine09}
{Kleine}, T., {Touboul}, M., {Bourdon}, B., {Nimmo}, F., {Mezger}, K., {Palme},
  H., {Jacobsen}, S.B., {Yin}, Q.Z., {Halliday}, A.N.: {Hf-W chronology of the
  accretion and early evolution of asteroids and terrestrial planets}.
\newblock \gca \textbf{73}, 5150--5188 (2009)

\bibitem{kokubo96}
{Kokubo}, E., {Ida}, S.: {On Runaway Growth of Planetesimals}.
\newblock Icarus \textbf{123}, 180--191 (1996).
\newblock \doi{10.1006/icar.1996.0148}

\bibitem{kokubo98}
{Kokubo}, E., {Ida}, S.: {Oligarchic Growth of Protoplanets}.
\newblock Icarus \textbf{131}, 171--178 (1998).
\newblock \doi{10.1006/icar.1997.5840}

\bibitem{kokubo00}
{Kokubo}, E., {Ida}, S.: {Formation of Protoplanets from Planetesimals in the
  Solar Nebula}.
\newblock Icarus \textbf{143}, 15--27 (2000).
\newblock \doi{10.1006/icar.1999.6237}

\bibitem{kokubo07}
{Kokubo}, E., {Ida}, S.: {Formation of Terrestrial Planets from Protoplanets.
  II. Statistics of Planetary Spin}.
\newblock \apj \textbf{671}, 2082--2090 (2007).
\newblock \doi{10.1086/522364}

\bibitem{kral17}
{Kral}, Q., {Krivov}, A.V., {Defr{\`e}re}, D., {van Lieshout}, R., {Bonsor},
  A., {Augereau}, J.C., {Th{\'e}bault}, P., {Ertel}, S., {Lebreton}, J.,
  {Absil}, O.: {Exozodiacal clouds: hot and warm dust around main sequence
  stars}.
\newblock The Astronomical Review \textbf{13}(2), 69--111 (2017).
\newblock \doi{10.1080/21672857.2017.1353202}

\bibitem{krasinsky02}
{Krasinsky}, G.A., {Pitjeva}, E.V., {Vasilyev}, M.V., {Yagudina}, E.I.: {Hidden
  Mass in the Asteroid Belt}.
\newblock \icarus \textbf{158}, 98--105 (2002).
\newblock \doi{10.1006/icar.2002.6837}

\bibitem{kretke12}
{Kretke}, K.A., {Lin}, D.N.C.: {The Importance of Disk Structure in Stalling
  Type I Migration}.
\newblock \apj \textbf{755}, 74 (2012).
\newblock \doi{10.1088/0004-637X/755/1/74}

\bibitem{krivov10}
{Krivov}, A.V.: {Debris disks: seeing dust, thinking of planetesimals and
  planets}.
\newblock Research in Astronomy and Astrophysics \textbf{10}, 383--414 (2010).
\newblock \doi{10.1088/1674-4527/10/5/001}

\bibitem{krot05}
{Krot}, A.N., {Amelin}, Y., {Cassen}, P., {Meibom}, A.: {Young chondrules in CB
  chondrites from a giant impact in the early Solar System}.
\newblock \nat \textbf{436}, 989--992 (2005).
\newblock \doi{10.1038/nature03830}

\bibitem{kruijer17}
{Kruijer}, T.S., {Burkhardt}, C., {Budde}, C., {Kleine}, T.: {Age of Jupiter
  inferred from the distinct genetics and formation times of meteorites}.
\newblock PNAS  (2017)

\bibitem{kruijer14}
{Kruijer}, T.S., {Touboul}, M., {Fischer-G{\"o}dde}, M., {Bermingham}, K.R.,
  {Walker}, R.J., {Kleine}, T.: {Protracted core formation and rapid accretion
  of protoplanets}.
\newblock Science \textbf{344}, 1150--1154 (2014).
\newblock \doi{10.1126/science.1251766}

\bibitem{kuchynka13}
{Kuchynka}, P., {Folkner}, W.M.: {A new approach to determining asteroid masses
  from planetary range measurements}.
\newblock \icarus \textbf{222}, 243--253 (2013).
\newblock \doi{10.1016/j.icarus.2012.11.003}

\bibitem{lambrechts12}
{Lambrechts}, M., {Johansen}, A.: {Rapid growth of gas-giant cores by pebble
  accretion}.
\newblock \aap \textbf{544}, A32 (2012).
\newblock \doi{10.1051/0004-6361/201219127}

\bibitem{lambrechts14}
{Lambrechts}, M., {Johansen}, A.: {Forming the cores of giant planets from the
  radial pebble flux in protoplanetary discs}.
\newblock \aap \textbf{572}, A107 (2014).
\newblock \doi{10.1051/0004-6361/201424343}

\bibitem{lambrechts14b}
{Lambrechts}, M., {Johansen}, A., {Morbidelli}, A.: {Separating gas-giant and
  ice-giant planets by halting pebble accretion}.
\newblock \aap \textbf{572}, A35 (2014).
\newblock \doi{10.1051/0004-6361/201423814}

\bibitem{lambrechts17}
{Lambrechts}, M., {Lega}, E.: {Reduced gas accretion on super-Earths and ice
  giants}.
\newblock \aap \textbf{606}, A146 (2017).
\newblock \doi{10.1051/0004-6361/201731014}

\bibitem{lambrechts19b}
{Lambrechts}, M., {Lega}, E., {Nelson}, R.P., {Crida}, A., {Morbidelli}, A.:
  {Quasi-static contraction during runaway gas accretion onto giant planets}.
\newblock \aap \textbf{630}, A82 (2019).
\newblock \doi{10.1051/0004-6361/201834413}

\bibitem{lambrechts19}
{Lambrechts}, M., {Morbidelli}, A., {Jacobson}, S.A., {Johansen}, A., {Bitsch},
  B., {Izidoro}, A., {Raymond}, S.N.: {Formation of planetary systems by pebble
  accretion and migration. How the radial pebble flux determines a
  terrestrial-planet or super-Earth growth mode}.
\newblock \aap \textbf{627}, A83 (2019).
\newblock \doi{10.1051/0004-6361/201834229}

\bibitem{Laplace}
{Laplace}, P.S., {Bowditch}, N., {Bowditch}, N.I.: {M{\'e}canique c{\'e}leste}
  (1829)

\bibitem{laskar97}
{Laskar}, J.: {Large scale chaos and the spacing of the inner planets.}
\newblock \aap \textbf{317}, L75--L78 (1997)

\bibitem{laws03}
{Laws}, C., {Gonzalez}, G., {Walker}, K.M., {Tyagi}, S., {Dodsworth}, J.,
  {Snider}, K., {Suntzeff}, N.B.: {Parent Stars of Extrasolar Planets. VII. New
  Abundance Analyses of 30 Systems}.
\newblock \aj \textbf{125}, 2664--2677 (2003).
\newblock \doi{10.1086/374626}

\bibitem{lecar06}
{Lecar}, M., {Podolak}, M., {Sasselov}, D., {Chiang}, E.: {On the Location of
  the Snow Line in a Protoplanetary Disk}.
\newblock \apj \textbf{640}, 1115--1118 (2006).
\newblock \doi{10.1086/500287}

\bibitem{lee16}
{Lee}, E.J., {Chiang}, E.: {Breeding Super-Earths and Birthing Super-puffs in
  Transitional Disks}.
\newblock \apj \textbf{817}, 90 (2016).
\newblock \doi{10.3847/0004-637X/817/2/90}

\bibitem{lee17}
{Lee}, E.J., {Chiang}, E.: {Magnetospheric Truncation, Tidal Inspiral, and the
  Creation of Short-period and Ultra-short-period Planets}.
\newblock \apj \textbf{842}, 40 (2017).
\newblock \doi{10.3847/1538-4357/aa6fb3}

\bibitem{lee14}
{Lee}, E.J., {Chiang}, E., {Ormel}, C.W.: {Make Super-Earths, Not Jupiters:
  Accreting Nebular Gas onto Solid Cores at 0.1 AU and Beyond}.
\newblock \apj \textbf{797}, 95 (2014).
\newblock \doi{10.1088/0004-637X/797/2/95}

\bibitem{lee02}
{Lee}, M.H., {Peale}, S.J.: {Dynamics and Origin of the 2:1 Orbital Resonances
  of the GJ 876 Planets}.
\newblock \apj \textbf{567}, 596--609 (2002).
\newblock \doi{10.1086/338504}

\bibitem{lega14}
{Lega}, E., {Crida}, A., {Bitsch}, B., {Morbidelli}, A.: {Migration of
  Earth-sized planets in 3D radiative discs}.
\newblock \mnras \textbf{440}, 683--695 (2014).
\newblock \doi{10.1093/mnras/stu304}

\bibitem{lestrade12}
{Lestrade}, J.F., {Matthews}, B.C., {Sibthorpe}, B., {Kennedy}, G.M., {Wyatt},
  M.C., {Bryden}, G., {Greaves}, J.S., {Thilliez}, E., {Moro-Mart{\'\i}n}, A.,
  {Booth}, M., {Dent}, W.R.F., {Duch{\^e}ne}, G., {Harvey}, P.M., {Horner}, J.,
  {Kalas}, P., {Kavelaars}, J.J., {Phillips}, N.M., {Rodriguez}, D.R., {Su},
  K.Y.L., {Wilner}, D.J.: {A DEBRIS disk around the planet hosting M-star GJ
  581 spatially resolved with Herschel}.
\newblock \aap \textbf{548}, A86 (2012).
\newblock \doi{10.1051/0004-6361/201220325}

\bibitem{levison15b}
{Levison}, H.F., {Kretke}, K.A., {Walsh}, K.J., {Bottke}, W.F.: {Growing the
  terrestrial planets from the gradual accumulation of sub-meter sized
  objects}.
\newblock Proceedings of the National Academy of Science \textbf{112},
  14180--14185 (2015).
\newblock \doi{10.1073/pnas.1513364112}

\bibitem{levison11}
{Levison}, H.F., {Morbidelli}, A., {Tsiganis}, K., {Nesvorn{\'y}}, D., {Gomes},
  R.: {Late Orbital Instabilities in the Outer Planets Induced by Interaction
  with a Self-gravitating Planetesimal Disk}.
\newblock \aj \textbf{142}, 152 (2011).
\newblock \doi{10.1088/0004-6256/142/5/152}

\bibitem{levison08}
{Levison}, H.F., {Morbidelli}, A., {Vanlaerhoven}, C., {Gomes}, R., {Tsiganis},
  K.: {Origin of the structure of the Kuiper belt during a dynamical
  instability in the orbits of Uranus and Neptune}.
\newblock Icarus \textbf{196}, 258--273 (2008).
\newblock \doi{10.1016/j.icarus.2007.11.035}

\bibitem{levison01}
{Levison}, H.F., {Stewart}, G.R.: {Remarks on Modeling the Formation of Uranus
  and Neptune}.
\newblock Icarus \textbf{153}, 224--228 (2001).
\newblock \doi{10.1006/icar.2001.6672}

\bibitem{levison10}
{Levison}, H.F., {Thommes}, E., {Duncan}, M.J.: {Modeling the Formation of
  Giant Planet Cores. I. Evaluating Key Processes}.
\newblock \aj \textbf{139}, 1297--1314 (2010).
\newblock \doi{10.1088/0004-6256/139/4/1297}

\bibitem{lichtenberg19}
{Lichtenberg}, T., {Golabek}, G.J., {Burn}, R., {Meyer}, M.R., {Alibert}, Y.,
  {Gerya}, T.V., {Mordasini}, C.: {A water budget dichotomy of rocky
  protoplanets from $^{26}$Al-heating}.
\newblock Nature Astronomy \textbf{3}, 307--313 (2019).
\newblock \doi{10.1038/s41550-018-0688-5}

\bibitem{lin96}
{Lin}, D.N.C., {Bodenheimer}, P., {Richardson}, D.C.: {Orbital migration of the
  planetary companion of 51 Pegasi to its present location}.
\newblock \nat \textbf{380}, 606--607 (1996).
\newblock \doi{10.1038/380606a0}

\bibitem{lin97}
{Lin}, D.N.C., {Ida}, S.: {On the Origin of Massive Eccentric Planets}.
\newblock \apj \textbf{477}, 781--+ (1997).
\newblock \doi{10.1086/303738}

\bibitem{lin79}
{Lin}, D.N.C., {Papaloizou}, J.: {Tidal torques on accretion discs in binary
  systems with extreme mass ratios.}
\newblock \mnras \textbf{186}, 799--812 (1979).
\newblock \doi{10.1093/mnras/186.4.799}

\bibitem{lin86}
{Lin}, D.N.C., {Papaloizou}, J.: {On the tidal interaction between protoplanets
  and the protoplanetary disk. III - Orbital migration of protoplanets}.
\newblock \apj \textbf{309}, 846--857 (1986).
\newblock \doi{10.1086/164653}

\bibitem{lis13}
{Lis}, D.C., {Biver}, N., {Bockel{\'e}e-Morvan}, D., {Hartogh}, P., {Bergin},
  E.A., {Blake}, G.A., {Crovisier}, J., {de Val-Borro}, M., {Jehin}, E.,
  {K{\"u}ppers}, M., {Manfroid}, J., {Moreno}, R., {Rengel}, M., {Szutowicz},
  S.: {A Herschel Study of D/H in Water in the Jupiter-family Comet
  45P/Honda-Mrkos-Pajdu{\v s}{\'a}kov{\'a} and Prospects for D/H Measurements
  with CCAT}.
\newblock \apjl \textbf{774}, L3 (2013).
\newblock \doi{10.1088/2041-8205/774/1/L3}

\bibitem{lis19}
{Lis}, D.C., {Bockel{\'e}e-Morvan}, D., {G{\"u}sten}, R., {Biver}, N.,
  {Stutzki}, J., {Delorme}, Y., {Dur{\'a}n}, C., {Wiesemeyer}, H., {Okada}, Y.:
  {Terrestrial deuterium-to-hydrogen ratio in water in hyperactive comets}.
\newblock \aap \textbf{625}, L5 (2019).
\newblock \doi{10.1051/0004-6361/201935554}

\bibitem{lissauer87}
{Lissauer}, J.J.: {Timescales for planetary accretion and the structure of the
  protoplanetary disk}.
\newblock Icarus \textbf{69}, 249--265 (1987).
\newblock \doi{10.1016/0019-1035(87)90104-7}

\bibitem{lissauer93}
{Lissauer}, J.J.: {Planet formation}.
\newblock \araa \textbf{31}, 129--174 (1993).
\newblock \doi{10.1146/annurev.aa.31.090193.001021}

\bibitem{lissauer09}
{Lissauer}, J.J., {Hubickyj}, O., {D'Angelo}, G., {Bodenheimer}, P.: {Models of
  Jupiter's growth incorporating thermal and hydrodynamic constraints}.
\newblock Icarus \textbf{199}, 338--350 (2009).
\newblock \doi{10.1016/j.icarus.2008.10.004}

\bibitem{lissauer11b}
{Lissauer}, J.J., {Ragozzine}, D., {Fabrycky}, D.C., {Steffen}, J.H., {Ford},
  E.B., {Jenkins}, J.M., {Shporer}, A., {Holman}, M.J., {Rowe}, J.F.,
  {Quintana}, E.V., {Batalha}, N.M., {Borucki}, W.J., {Bryson}, S.T.,
  {Caldwell}, D.A., {Carter}, J.A., {Ciardi}, D., {Dunham}, E.W., {Fortney},
  J.J., {Gautier} III, T.N., {Howell}, S.B., {Koch}, D.G., {Latham}, D.W.,
  {Marcy}, G.W., {Morehead}, R.C., {Sasselov}, D.: {Architecture and Dynamics
  of Kepler's Candidate Multiple Transiting Planet Systems}.
\newblock \apjs \textbf{197}, 8 (2011).
\newblock \doi{10.1088/0067-0049/197/1/8}

\bibitem{lissauer07}
{Lissauer}, J.J., {Stevenson}, D.J.: {Formation of Giant Planets}.
\newblock Protostars and Planets V pp. 591--606 (2007)

\bibitem{lodders03}
{Lodders}, K.: {Solar System Abundances and Condensation Temperatures of the
  Elements}.
\newblock \apj \textbf{591}, 1220--1247 (2003).
\newblock \doi{10.1086/375492}

\bibitem{looney03}
{Looney}, L.W., {Mundy}, L.G., {Welch}, W.J.: {Envelope Emission in Young
  Stellar Systems: A Subarcsecond Survey of Circumstellar Structure}.
\newblock \apj \textbf{592}, 255--265 (2003).
\newblock \doi{10.1086/375582}

\bibitem{lopez17}
{Lopez}, E.D.: {Born dry in the photoevaporation desert: Kepler's
  ultra-short-period planets formed water-poor}.
\newblock \mnras \textbf{472}, 245--253 (2017).
\newblock \doi{10.1093/mnras/stx1558}

\bibitem{lovis07}
{Lovis}, C., {Mayor}, M.: {Planets around evolved intermediate-mass stars. I.
  Two substellar companions in the open clusters NGC 2423 and NGC 4349}.
\newblock \aap \textbf{472}, 657--664 (2007).
\newblock \doi{10.1051/0004-6361:20077375}

\bibitem{luger17}
{Luger}, R., {Sestovic}, M., {Kruse}, E., {Grimm}, S.L., {Demory}, B.O.,
  {Agol}, E., {Bolmont}, E., {Fabrycky}, D., {Fernandes}, C.S., {Van Grootel},
  V., {Burgasser}, A., {Gillon}, M., {Ingalls}, J.G., {Jehin}, E., {Raymond},
  S.N., {Selsis}, F., {Triaud}, A.H.M.J., {Barclay}, T., {Barentsen}, G.,
  {Howell}, S.B., {Delrez}, L., {de Wit}, J., {Foreman-Mackey}, D.,
  {Holdsworth}, D.L., {Leconte}, J., {Lederer}, S., {Turbet}, M., {Almleaky},
  Y., {Benkhaldoun}, Z., {Magain}, P., {Morris}, B.M., {Heng}, K., {Queloz},
  D.: {A seven-planet resonant chain in TRAPPIST-1}.
\newblock Nature Astronomy \textbf{1}, 0129 (2017).
\newblock \doi{10.1038/s41550-017-0129}

\bibitem{lykawka19}
{Lykawka}, P.S., {Ito}, T.: {Constraining the Formation of the Four Terrestrial
  Planets in the Solar System}.
\newblock arXiv e-prints arXiv:1908.04934 (2019)

\bibitem{lyndenbell74}
{Lynden-Bell}, D., {Pringle}, J.E.: {The evolution of viscous discs and the
  origin of the nebular variables.}
\newblock \mnras \textbf{168}, 603--637 (1974)

\bibitem{lyra10}
{Lyra}, W., {Paardekooper}, S.J., {Mac Low}, M.M.: {Orbital Migration of
  Low-mass Planets in Evolutionary Radiative Models: Avoiding Catastrophic
  Infall}.
\newblock \apjl \textbf{715}, L68--L73 (2010).
\newblock \doi{10.1088/2041-8205/715/2/L68}

\bibitem{mamajek09}
{Mamajek}, E.E.: {Initial Conditions of Planet Formation: Lifetimes of
  Primordial Disks}.
\newblock In: T.~{Usuda}, M.~{Tamura}, M.~{Ishii} (eds.) American Institute of
  Physics Conference Series, \emph{American Institute of Physics Conference
  Series}, vol. 1158, pp. 3--10 (2009).
\newblock \doi{10.1063/1.3215910}

\bibitem{manara18}
{Manara}, C.F., {Morbidelli}, A., {Guillot}, T.: {Why do protoplanetary disks
  appear not massive enough to form the known exoplanet population?}
\newblock \aap \textbf{618}, L3 (2018).
\newblock \doi{10.1051/0004-6361/201834076}

\bibitem{mandell07}
{Mandell}, A.M., {Raymond}, S.N., {Sigurdsson}, S.: {Formation of Earth-like
  Planets During and After Giant Planet Migration}.
\newblock \apj \textbf{660}, 823--844 (2007).
\newblock \doi{10.1086/512759}

\bibitem{marcy14}
{Marcy}, G.W., {Isaacson}, H., {Howard}, A.W., {Rowe}, J.F., {Jenkins}, J.M.,
  {Bryson}, S.T., {Latham}, D.W., {Howell}, S.B., {Gautier} III, T.N.,
  {Batalha}, N.M., {Rogers}, L., {Ciardi}, D., {Fischer}, D.A., {Gilliland},
  R.L., {Kjeldsen}, H., {Christensen-Dalsgaard}, J., {Huber}, D., {Chaplin},
  W.J., {Basu}, S., {Buchhave}, L.A., {Quinn}, S.N., {Borucki}, W.J., {Koch},
  D.G., {Hunter}, R., {Caldwell}, D.A., {Van Cleve}, J., {Kolbl}, R., {Weiss},
  L.M., {Petigura}, E., {Seager}, S., {Morton}, T., {Johnson}, J.A., {Ballard},
  S., {Burke}, C., {Cochran}, W.D., {Endl}, M., {MacQueen}, P., {Everett},
  M.E., {Lissauer}, J.J., {Ford}, E.B., {Torres}, G., {Fressin}, F., {Brown},
  T.M., {Steffen}, J.H., {Charbonneau}, D., {Basri}, G.S., {Sasselov}, D.D.,
  {Winn}, J., {Sanchis-Ojeda}, R., {Christiansen}, J., {Adams}, E., {Henze},
  C., {Dupree}, A., {Fabrycky}, D.C., {Fortney}, J.J., {Tarter}, J., {Holman},
  M.J., {Tenenbaum}, P., {Shporer}, A., {Lucas}, P.W., {Welsh}, W.F., {Orosz},
  J.A., {Bedding}, T.R., {Campante}, T.L., {Davies}, G.R., {Elsworth}, Y.,
  {Handberg}, R., {Hekker}, S., {Karoff}, C., {Kawaler}, S.D., {Lund}, M.N.,
  {Lundkvist}, M., {Metcalfe}, T.S., {Miglio}, A., {Silva Aguirre}, V.,
  {Stello}, D., {White}, T.R., {Boss}, A., {Devore}, E., {Gould}, A., {Prsa},
  A., {Agol}, E., {Barclay}, T., {Coughlin}, J., {Brugamyer}, E., {Mullally},
  F., {Quintana}, E.V., {Still}, M., {Thompson}, S.E., {Morrison}, D.,
  {Twicken}, J.D., {D{\'e}sert}, J.M., {Carter}, J., {Crepp}, J.R.,
  {H{\'e}brard}, G., {Santerne}, A., {Moutou}, C., {Sobeck}, C., {Hudgins}, D.,
  {Haas}, M.R., {Robertson}, P., {Lillo-Box}, J., {Barrado}, D.: {Masses,
  Radii, and Orbits of Small Kepler Planets: The Transition from Gaseous to
  Rocky Planets}.
\newblock \apjs \textbf{210}, 20 (2014).
\newblock \doi{10.1088/0067-0049/210/2/20}

\bibitem{marois08}
{Marois}, C., {Macintosh}, B., {Barman}, T., {Zuckerman}, B., {Song}, I.,
  {Patience}, J., {Lafreni{\`e}re}, D., {Doyon}, R.: {Direct Imaging of
  Multiple Planets Orbiting the Star HR 8799}.
\newblock Science \textbf{322}, 1348-- (2008).
\newblock \doi{10.1126/science.1166585}

\bibitem{marois10}
{Marois}, C., {Zuckerman}, B., {Konopacky}, Q.M., {Macintosh}, B., {Barman},
  T.: {Images of a fourth planet orbiting HR 8799}.
\newblock \nat \textbf{468}, 1080--1083 (2010).
\newblock \doi{10.1038/nature09684}

\bibitem{marshall14}
{Marshall}, J.P., {Moro-Mart{\'{\i}}n}, A., {Eiroa}, C., {Kennedy}, G., {Mora},
  A., {Sibthorpe}, B., {Lestrade}, J.F., {Maldonado}, J., {Sanz-Forcada}, J.,
  {Wyatt}, M.C., {Matthews}, B., {Horner}, J., {Montesinos}, B., {Bryden}, G.,
  {del Burgo}, C., {Greaves}, J.S., {Ivison}, R.J., {Meeus}, G., {Olofsson},
  G., {Pilbratt}, G.L., {White}, G.J.: {Correlations between the stellar,
  planetary, and debris components of exoplanet systems observed by Herschel}.
\newblock \aap \textbf{565}, A15 (2014).
\newblock \doi{10.1051/0004-6361/201323058}

\bibitem{martin12}
{Martin}, R.G., {Livio}, M.: {On the evolution of the snow line in
  protoplanetary discs}.
\newblock \mnras \textbf{425}, L6--L9 (2012).
\newblock \doi{10.1111/j.1745-3933.2012.01290.x}

\bibitem{martin15}
{Martin}, R.G., {Livio}, M.: {The Solar System as an Exoplanetary System}.
\newblock \apj \textbf{810}, 105 (2015).
\newblock \doi{10.1088/0004-637X/810/2/105}

\bibitem{marty12}
{Marty}, B.: {The origins and concentrations of water, carbon, nitrogen and
  noble gases on Earth}.
\newblock Earth and Planetary Science Letters \textbf{313}, 56--66 (2012).
\newblock \doi{10.1016/j.epsl.2011.10.040}

\bibitem{marty17}
{Marty}, B., {Altwegg}, K., {Balsiger}, H., {Bar-Nun}, A., {Bekaert}, D.V.,
  {Berthelier}, J.J., {Bieler}, A., {Briois}, C., {Calmonte}, U., {Combi}, M.,
  {De Keyser}, J., {Fiethe}, B., {Fuselier}, S.A., {Gasc}, S., {Gombosi}, T.I.,
  {Hansen}, K.C., {H{\"a}ssig}, M., {J{\"a}ckel}, A., {Kopp}, E., {Korth}, A.,
  {Le Roy}, L., {Mall}, U., {Mousis}, O., {Owen}, T., {R{\`e}me}, H., {Rubin},
  M., {S{\'e}mon}, T., {Tzou}, C.Y., {Waite}, J.H., {Wurz}, P.: {Xenon isotopes
  in 67P/Churyumov-Gerasimenko show that comets contributed to Earth's
  atmosphere}.
\newblock Science \textbf{356}, 1069--1072 (2017).
\newblock \doi{10.1126/science.aal3496}

\bibitem{marty16}
{Marty}, B., {Avice}, G., {Sano}, Y., {Altwegg}, K., {Balsiger}, H.,
  {H{\"a}ssig}, M., {Morbidelli}, A., {Mousis}, O., {Rubin}, M.: {Origins of
  volatile elements (H, C, N, noble gases) on Earth and Mars in light of recent
  results from the ROSETTA cometary mission}.
\newblock Earth and Planetary Science Letters \textbf{441}, 91--102 (2016).
\newblock \doi{10.1016/j.epsl.2016.02.031}

\bibitem{marty06}
{Marty}, B., {Yokochi}, R.: {Water in the Early Earth}.
\newblock Rev. Mineral Geophys. \textbf{62}, 421--450 (2006)

\bibitem{marzari14}
{Marzari}, F.: {Impact of planet-planet scattering on the formation and
  survival of debris discs}.
\newblock \mnras \textbf{444}, 1419--1424 (2014).
\newblock \doi{10.1093/mnras/stu1544}

\bibitem{marzari02}
{Marzari}, F., {Weidenschilling}, S.J.: {Eccentric Extrasolar Planets: The
  Jumping Jupiter Model}.
\newblock Icarus \textbf{156}, 570--579 (2002).
\newblock \doi{10.1006/icar.2001.6786}

\bibitem{masset01}
{Masset}, F., {Snellgrove}, M.: {Reversing type II migration: resonance
  trapping of a lighter giant protoplanet}.
\newblock \mnras \textbf{320}, L55--L59 (2001).
\newblock \doi{10.1046/j.1365-8711.2001.04159.x}

\bibitem{masset17}
{Masset}, F.S.: {Coorbital thermal torques on low-mass protoplanets}.
\newblock \mnras \textbf{472}(4), 4204--4219 (2017).
\newblock \doi{10.1093/mnras/stx2271}

\bibitem{masset06}
{Masset}, F.S., {Morbidelli}, A., {Crida}, A., {Ferreira}, J.: {Disk Surface
  Density Transitions as Protoplanet Traps}.
\newblock \apj \textbf{642}, 478--487 (2006).
\newblock \doi{10.1086/500967}

\bibitem{matsumoto12}
{Matsumoto}, Y., {Nagasawa}, M., {Ida}, S.: {The orbital stability of planets
  trapped in the first-order mean-motion resonances}.
\newblock \icarus \textbf{221}(2), 624--631 (2012).
\newblock \doi{10.1016/j.icarus.2012.08.032}

\bibitem{matsumura13}
{Matsumura}, S., {Ida}, S., {Nagasawa}, M.: {Effects of Dynamical Evolution of
  Giant Planets on Survival of Terrestrial Planets}.
\newblock \apj \textbf{767}, 129 (2013).
\newblock \doi{10.1088/0004-637X/767/2/129}

\bibitem{matsumura10}
{Matsumura}, S., {Thommes}, E.W., {Chatterjee}, S., {Rasio}, F.A.: {Unstable
  Planetary Systems Emerging Out of Gas Disks}.
\newblock \apj \textbf{714}, 194--206 (2010).
\newblock \doi{10.1088/0004-637X/714/1/194}

\bibitem{matthews14}
{Matthews}, B.C., {Krivov}, A.V., {Wyatt}, M.C., {Bryden}, G., {Eiroa}, C.:
  {Observations, Modeling, and Theory of Debris Disks}.
\newblock In: H.~{Beuther}, R.S. {Klessen}, C.P. {Dullemond}, T.~{Henning}
  (eds.) Protostars and Planets VI, p. 521 (2014)

\bibitem{mayer07}
{Mayer}, L., {Lufkin}, G., {Quinn}, T., {Wadsley}, J.: {Fragmentation of
  Gravitationally Unstable Gaseous Protoplanetary Disks with Radiative
  Transfer}.
\newblock \apjl \textbf{661}(1), L77--L80 (2007).
\newblock \doi{10.1086/518433}

\bibitem{mayer02}
{Mayer}, L., {Quinn}, T., {Wadsley}, J., {Stadel}, J.: {Formation of Giant
  Planets by Fragmentation of Protoplanetary Disks}.
\newblock Science \textbf{298}(5599), 1756--1759 (2002).
\newblock \doi{10.1126/science.1077635}

\bibitem{mayor11}
{Mayor}, M., {Marmier}, M., {Lovis}, C., {Udry}, S., {S{\'e}gransan}, D.,
  {Pepe}, F., {Benz}, W., {Bertaux}, J.., {Bouchy}, F., {Dumusque}, X., {Lo
  Curto}, G., {Mordasini}, C., {Queloz}, D., {Santos}, N.C.: {The HARPS search
  for southern extra-solar planets XXXIV. Occurrence, mass distribution and
  orbital properties of super-Earths and Neptune-mass planets}.
\newblock arXiv:1109.2497  (2011)

\bibitem{mccubbin19}
{McCubbin}, F.M., {Barnes}, J.J.: {Origin and abundances of H$_{2}$O in the
  terrestrial planets, Moon, and asteroids}.
\newblock Earth and Planetary Science Letters \textbf{526}, 115771 (2019).
\newblock \doi{10.1016/j.epsl.2019.115771}

\bibitem{mcnally19}
{McNally}, C.P., {Nelson}, R.P., {Paardekooper}, S.J., {Ben{\'\i}tez-Llambay},
  P.: {Migrating super-Earths in low-viscosity discs: unveiling the roles of
  feedback, vortices, and laminar accretion flows}.
\newblock \mnras \textbf{484}(1), 728--748 (2019).
\newblock \doi{10.1093/mnras/stz023}

\bibitem{mcneil10}
{McNeil}, D.S., {Nelson}, R.P.: {On the formation of hot Neptunes and
  super-Earths}.
\newblock \mnras \textbf{401}, 1691--1708 (2010).
\newblock \doi{10.1111/j.1365-2966.2009.15805.x}

\bibitem{meech19}
{Meech}, K., {Raymond}, S.N.: {Origin of Earth's water: sources and
  constraints}.
\newblock arXiv e-prints arXiv:1912.04361 (2019)

\bibitem{meru11}
{Meru}, F., {Bate}, M.R.: {On the fragmentation criteria of self-gravitating
  protoplanetary discs}.
\newblock \mnras \textbf{410}(1), 559--572 (2011).
\newblock \doi{10.1111/j.1365-2966.2010.17465.x}

\bibitem{meyer08}
{Meyer}, M.R., {Carpenter}, J.M., {Mamajek}, E.E., {Hillenbrand}, L.A.,
  {Hollenbach}, D., {Moro-Martin}, A., {Kim}, J.S., {Silverstone}, M.D.,
  {Najita}, J., {Hines}, D.C., {Pascucci}, I., {Stauffer}, J.R., {Bouwman}, J.,
  {Backman}, D.E.: {Evolution of Mid-Infrared Excess around Sun-like Stars:
  Constraints on Models of Terrestrial Planet Formation}.
\newblock \apjl \textbf{673}, L181--L184 (2008).
\newblock \doi{10.1086/527470}

\bibitem{millholland17}
{Millholland}, S., {Wang}, S., {Laughlin}, G.: {Kepler Multi-planet Systems
  Exhibit Unexpected Intra-system Uniformity in Mass and Radius}.
\newblock \apjl \textbf{849}(2), L33 (2017).
\newblock \doi{10.3847/2041-8213/aa9714}

\bibitem{mills16}
{Mills}, S.M., {Fabrycky}, D.C., {Migaszewski}, C., {Ford}, E.B., {Petigura},
  E., {Isaacson}, H.: {A resonant chain of four transiting, sub-Neptune
  planets}.
\newblock \nat \textbf{533}, 509--512 (2016).
\newblock \doi{10.1038/nature17445}

\bibitem{moeckel09}
{Moeckel}, N., {Throop}, H.B.: {Bondi-Hoyle-Lyttleton Accretion Onto a
  Protoplanetary Disk}.
\newblock \apj \textbf{707}(1), 268--277 (2009).
\newblock \doi{10.1088/0004-637X/707/1/268}

\bibitem{mojzsis19}
{Mojzsis}, S.J., {Brasser}, R., {Kelly}, N.M., {Abramov}, O., {Werner}, S.C.:
  {Onset of Giant Planet Migration before 4480 Million Years Ago}.
\newblock \apj \textbf{881}(1), 44 (2019).
\newblock \doi{10.3847/1538-4357/ab2c03}

\bibitem{montesinos16}
{Montesinos}, B., {Eiroa}, C., {Krivov}, A.V., {Marshall}, J.P., {Pilbratt},
  G.L., {Liseau}, R., {Mora}, A., {Maldonado}, J., {Wolf}, S., {Ertel}, S.,
  {Bayo}, A., {Augereau}, J.C., {Heras}, A.M., {Fridlund}, M., {Danchi}, W.C.,
  {Solano}, E., {Kirchschlager}, F., {del Burgo}, C., {Montes}, D.: {Incidence
  of debris discs around FGK stars in the solar neighbourhood}.
\newblock \aap \textbf{593}, A51 (2016).
\newblock \doi{10.1051/0004-6361/201628329}

\bibitem{monteux18}
{Monteux}, J., {Golabek}, G.J., {Rubie}, D.C., {Tobie}, G., {Young}, E.D.:
  {Water and the Interior Structure of Terrestrial Planets and Icy Bodies}.
\newblock \ssr \textbf{214}(1), 39 (2018).
\newblock \doi{10.1007/s11214-018-0473-x}

\bibitem{moorhead05}
{Moorhead}, A.V., {Adams}, F.C.: {Giant planet migration through the action of
  disk torques and planet planet scattering}.
\newblock Icarus \textbf{178}, 517--539 (2005).
\newblock \doi{10.1016/j.icarus.2005.05.005}

\bibitem{morales19}
{Morales}, J.C., {Mustill}, A.J., {Ribas}, I., {Davies}, M.B., {Reiners}, A.,
  {Bauer}, F.F., {Kossakowski}, D., {Herrero}, E., {Rodr{\'\i}guez}, E.,
  {L{\'o}pez-Gonz{\'a}lez}, M.J., {Rodr{\'\i}guez-L{\'o}pez}, C., {B{\'e}jar},
  V.J.S., {Gonz{\'a}lez-Cuesta}, L., {Luque}, R., {Pall{\'e}}, E., {Perger},
  M., {Baroch}, D., {Johansen}, A., {Klahr}, H., {Mordasini}, C.,
  {Anglada-Escud{\'e}}, G., {Caballero}, J.A., {Cort{\'e}s-Contreras}, M.,
  {Dreizler}, S., {Lafarga}, M., {Nagel}, E., {Passegger}, V.M., {Reffert}, S.,
  {Rosich}, A., {Schweitzer}, A., {Tal-Or}, L., {Trifonov}, T., {Zechmeister},
  M., {Quirrenbach}, A., {Amado}, P.J., {Guenther}, E.W., {Hagen}, H.J.,
  {Henning}, T., {Jeffers}, S.V., {Kaminski}, A., {K{\"u}rster}, M., {Montes},
  D., {Seifert}, W., {Abell{\'a}n}, F.J., {Abril}, M., {Aceituno}, J.,
  {Aceituno}, F.J., {Alonso-Floriano}, F.J., {Ammler-von Eiff}, M., {Antona},
  R., {Arroyo-Torres}, B., {Azzaro}, M., {Barrado}, D., {Becerril-Jarque}, S.,
  {Ben{\'\i}tez}, D., {Berdi{\~n}as}, Z.M., {Bergond}, G., {Brinkm{\"o}ller},
  M., {del Burgo}, C., {Burn}, R., {Calvo-Ortega}, R., {Cano}, J.,
  {C{\'a}rdenas}, M.C., {Guill{\'e}n}, C.C., {Carro}, J., {Casal}, E.,
  {Casanova}, V., {Casasayas-Barris}, N., {Chaturvedi}, P., {Cifuentes}, C.,
  {Claret}, A., {Colom{\'e}}, J., {Czesla}, S., {D{\'\i}ez-Alonso}, E.,
  {Dorda}, R., {Emsenhuber}, A., {Fern{\'a}ndez}, M.,
  {Fern{\'a}ndez-Mart{\'\i}n}, A., {Ferro}, I.M., {Fuhrmeister}, B.,
  {Galad{\'\i}-Enr{\'\i}quez}, D., {Cava}, I.G., {Vargas}, M.L.G.,
  {Garcia-Piquer}, A., {Gesa}, L., {Gonz{\'a}lez-{\'A}lvarez}, E.,
  {Hern{\'a}ndez}, J.I.G., {Gonz{\'a}lez-Peinado}, R., {Gu{\`a}rdia}, J.,
  {Guijarro}, A., {de Guindos}, E., {Hatzes}, A.P., {Hauschildt}, P.H.,
  {Hedrosa}, R.P., {Hermelo}, I., {Arabi}, R.H., {Otero}, F.H., {Hintz}, D.,
  {Holgado}, G., {Huber}, A., {Huke}, P., {Johnson}, E.N., {de Juan}, E.,
  {Kehr}, M., {Kemmer}, J., {Kim}, M., {Kl{\"u}ter}, J., {Klutsch}, A.,
  {Labarga}, F., {Labiche}, N., {Lalitha}, S., {Lamp{\'o}n}, M., {Lara}, L.M.,
  {Launhardt}, R., {L{\'a}zaro}, F.J., {Lizon}, J.L., {Llamas}, M., {Lodieu},
  N., {L{\'o}pez del Fresno}, M., {Salas}, J.F.L., {L{\'o}pez-Santiago}, J.,
  {Madinabeitia}, H.M., {Mall}, U., {Mancini}, L., {Mand el}, H., {Marfil}, E.,
  {Molina}, J.A.M., {Mart{\'\i}n}, E.L., {Mart{\'\i}n-Fern{\'a}ndez}, P.,
  {Mart{\'\i}n-Ruiz}, S., {Mart{\'\i}nez-Rodr{\'\i}guez}, H., {Marvin}, C.J.,
  {Mirabet}, E., {Moya}, A., {Naranjo}, V., {Nelson}, R.P., {Nortmann}, L.,
  {Nowak}, G., {Ofir}, A., {Pascual}, J., {Pavlov}, A., {Pedraz}, S.,
  {Medialdea}, D.P., {P{\'e}rez-Calpena}, A., {Perryman}, M.A.C., {Rabaza}, O.,
  {Ballesta}, A.R., {Rebolo}, R., {Redondo}, P., {Rix}, H.W., {Rodler}, F.,
  {Trinidad}, A.R., {Sabotta}, S., {Sadegi}, S., {Salz}, M.,
  {S{\'a}nchez-Blanco}, E., {Carrasco}, M.A.S., {S{\'a}nchez-L{\'o}pez}, A.,
  {Sanz-Forcada}, J., {Sarkis}, P., {Sarmiento}, L.F., {Sch{\"a}fer}, S.,
  {Schlecker}, M., {Schmitt}, J.H.M.M., {Sch{\"o}fer}, P., {Solano}, E.,
  {Sota}, A., {Stahl}, O., {Stock}, S., {Stuber}, T., {St{\"u}rmer}, J.,
  {Su{\'a}rez}, J.C., {Tabernero}, H.M., {Tulloch}, S.M., {Veredas}, G.,
  {Vico-Linares}, J.I., {Vilardell}, F., {Wagner}, K., {Winkler}, J.,
  {Wolthoff}, V., {Yan}, F., {Osorio}, M.R.Z.: {A giant exoplanet orbiting a
  very-low-mass star challenges planet formation models}.
\newblock Science \textbf{365}(6460), 1441--1445 (2019).
\newblock \doi{10.1126/science.aax3198}

\bibitem{morby16}
{Morbidelli}, A., {Bitsch}, B., {Crida}, A., {Gounelle}, M., {Guillot}, T.,
  {Jacobson}, S., {Johansen}, A., {Lambrechts}, M., {Lega}, E.: {Fossilized
  condensation lines in the Solar System protoplanetary disk}.
\newblock Icarus \textbf{267}, 368--376 (2016).
\newblock \doi{10.1016/j.icarus.2015.11.027}

\bibitem{morby00}
{Morbidelli}, A., {Chambers}, J., {Lunine}, J.I., {Petit}, J.M., {Robert}, F.,
  {Valsecchi}, G.B., {Cyr}, K.E.: {Source regions and time scales for the
  delivery of water to Earth}.
\newblock Meteoritics and Planetary Science \textbf{35}, 1309--1320 (2000).
\newblock \doi{10.1111/j.1945-5100.2000.tb01518.x}

\bibitem{morby15}
{Morbidelli}, A., {Lambrechts}, M., {Jacobson}, S., {Bitsch}, B.: {The great
  dichotomy of the Solar System: Small terrestrial embryos and massive giant
  planet cores}.
\newblock Icarus \textbf{258}, 418--429 (2015).
\newblock \doi{10.1016/j.icarus.2015.06.003}

\bibitem{morby05}
{Morbidelli}, A., {Levison}, H.F., {Tsiganis}, K., {Gomes}, R.: {Chaotic
  capture of Jupiter's Trojan asteroids in the early Solar System}.
\newblock \nat \textbf{435}, 462--465 (2005).
\newblock \doi{10.1038/nature03540}

\bibitem{morby12}
{Morbidelli}, A., {Nesvorny}, D.: {Dynamics of pebbles in the vicinity of a
  growing planetary embryo: hydro-dynamical simulations}.
\newblock \aap \textbf{546}, A18 (2012).
\newblock \doi{10.1051/0004-6361/201219824}

\bibitem{morby18}
{Morbidelli}, A., {Nesvorny}, D., {Laurenz}, V., {Marchi}, S., {Rubie}, D.C.,
  {Elkins-Tanton}, L., {Wieczorek}, M., {Jacobson}, S.: {The timeline of the
  lunar bombardment: Revisited}.
\newblock \icarus \textbf{305}, 262--276 (2018).
\newblock \doi{10.1016/j.icarus.2017.12.046}

\bibitem{morbyraymond16}
{Morbidelli}, A., {Raymond}, S.N.: {Challenges in planet formation}.
\newblock Journal of Geophysical Research (Planets) \textbf{121}, 1962--1980
  (2016).
\newblock \doi{10.1002/2016JE005088}

\bibitem{morby07}
{Morbidelli}, A., {Tsiganis}, K., {Crida}, A., {Levison}, H.F., {Gomes}, R.:
  {Dynamics of the Giant Planets of the Solar System in the Gaseous
  Protoplanetary Disk and Their Relationship to the Current Orbital
  Architecture}.
\newblock \aj \textbf{134}, 1790--1798 (2007).
\newblock \doi{10.1086/521705}

\bibitem{morbywood15}
{Morbidelli}, A., {Wood}, B.J.: {Late Accretion and the Late Veneer}.
\newblock Washington DC American Geophysical Union Geophysical Monograph Series
  \textbf{212}, 71--82 (2015).
\newblock \doi{10.1002/9781118860359.ch4}

\bibitem{mordasini09}
{Mordasini}, C., {Alibert}, Y., {Benz}, W.: {Extrasolar planet population
  synthesis. I. Method, formation tracks, and mass-distance distribution}.
\newblock \aap \textbf{501}, 1139--1160 (2009).
\newblock \doi{10.1051/0004-6361/200810301}

\bibitem{mori19}
{Mori}, S., {Bai}, X.N., {Okuzumi}, S.: {Temperature Structure in the Inner
  Regions of Protoplanetary Disks: Inefficient Accretion Heating Controlled by
  Nonideal Magnetohydrodynamics}.
\newblock \apj \textbf{872}(1), 98 (2019).
\newblock \doi{10.3847/1538-4357/ab0022}

\bibitem{moriarty16}
{Moriarty}, J., {Ballard}, S.: {The Kepler Dichotomy in Planetary Disks:
  Linking Kepler Observables to Simulations of Late-stage Planet Formation}.
\newblock \apj \textbf{832}, 34 (2016).
\newblock \doi{10.3847/0004-637X/832/1/34}

\bibitem{morishima08}
{Morishima}, R., {Schmidt}, M.W., {Stadel}, J., {Moore}, B.: {Formation and
  Accretion History of Terrestrial Planets from Runaway Growth through to Late
  Time: Implications for Orbital Eccentricity}.
\newblock \apj \textbf{685}, 1247--1261 (2008).
\newblock \doi{10.1086/590948}

\bibitem{morishima10}
{Morishima}, R., {Stadel}, J., {Moore}, B.: {From planetesimals to terrestrial
  planets: N-body simulations including the effects of nebular gas and giant
  planets}.
\newblock Icarus \textbf{207}, 517--535 (2010).
\newblock \doi{10.1016/j.icarus.2009.11.038}

\bibitem{moromartin07}
{Moro-Mart{\'{\i}}n}, A., {Carpenter}, J.M., {Meyer}, M.R., {Hillenbrand},
  L.A., {Malhotra}, R., {Hollenbach}, D., {Najita}, J., {Henning}, T., {Kim},
  J.S., {Bouwman}, J., {Silverstone}, M.D., {Hines}, D.C., {Wolf}, S.,
  {Pascucci}, I., {Mamajek}, E.E., {Lunine}, J.: {Are Debris Disks and Massive
  Planets Correlated?}
\newblock \apj \textbf{658}, 1312--1321 (2007).
\newblock \doi{10.1086/511746}

\bibitem{moromartin15}
{Moro-Mart{\'{\i}}n}, A., {Marshall}, J.P., {Kennedy}, G., {Sibthorpe}, B.,
  {Matthews}, B.C., {Eiroa}, C., {Wyatt}, M.C., {Lestrade}, J.F., {Maldonado},
  J., {Rodriguez}, D., {Greaves}, J.S., {Montesinos}, B., {Mora}, A., {Booth},
  M., {Duch{\^e}ne}, G., {Wilner}, D., {Horner}, J.: {Does the Presence of
  Planets Affect the Frequency and Properties of Extrasolar Kuiper Belts?
  Results from the Herschel Debris and Dunes Surveys}.
\newblock \apj \textbf{801}, 143 (2015).
\newblock \doi{10.1088/0004-637X/801/2/143}

\bibitem{mottl07}
{Mottl}, M., {Glazer}, B., {Kaiser}, R., {Meech}, K.: {Water and astrobiology}.
\newblock Chemie der Erde / Geochemistry \textbf{67}(4), 253--282 (2007).
\newblock \doi{10.1016/j.chemer.2007.09.002}

\bibitem{sujoy12}
{Mukhopadhyay}, S.: {Early differentiation and volatile accretion recorded in
  deep-mantle neon and xenon}.
\newblock \nat \textbf{486}, 101--104 (2012).
\newblock \doi{10.1038/nature11141}

\bibitem{mulders19}
{Mulders}, G.D., {Mordasini}, C., {Pascucci}, I., {Ciesla}, F.J., {Emsenhuber},
  A., {Apai}, D.: {The Exoplanet Population Observation Simulator. II --
  Population Synthesis in the Era of Kepler}.
\newblock arXiv e-prints arXiv:1905.08804 (2019)

\bibitem{mulders18}
{Mulders}, G.D., {Pascucci}, I., {Apai}, D., {Ciesla}, F.J.: {The Exoplanet
  Population Observation Simulator. I. The Inner Edges of Planetary Systems}.
\newblock \aj \textbf{156}, 24 (2018).
\newblock \doi{10.3847/1538-3881/aac5ea}

\bibitem{mundy00}
{Mundy}, L.G., {Looney}, L.W., {Welch}, W.J.: {The Structure and Evolution of
  Envelopes and Disks in Young Stellar Systems}.
\newblock Protostars and Planets IV pp. 355--+ (2000)

\bibitem{muralidharan08}
{Muralidharan}, K., {Deymier}, P., {Stimpfl}, M., {de Leeuw}, N.H., {Drake},
  M.J.: {Origin of water in the inner Solar System: A kinetic Monte Carlo study
  of water adsorption on forsterite}.
\newblock \icarus \textbf{198}(2), 400--407 (2008).
\newblock \doi{10.1016/j.icarus.2008.07.017}

\bibitem{nagasawa08}
{Nagasawa}, M., {Ida}, S., {Bessho}, T.: {Formation of Hot Planets by a
  Combination of Planet Scattering, Tidal Circularization, and the Kozai
  Mechanism}.
\newblock \apj \textbf{678}, 498--508 (2008).
\newblock \doi{10.1086/529369}

\bibitem{nagasawa05}
{Nagasawa}, M., {Lin}, D.N.C., {Thommes}, E.: {Dynamical Shake-up of Planetary
  Systems. I. Embryo Trapping and Induced Collisions by the Sweeping Secular
  Resonance and Embryo-Disk Tidal Interaction}.
\newblock \apj \textbf{635}, 578--598 (2005).
\newblock \doi{10.1086/497386}

\bibitem{nayakshin15}
{Nayakshin}, S.: {Tidal downsizing model - I. Numerical methods: saving giant
  planets from tidal disruptions}.
\newblock \mnras \textbf{454}(1), 64--82 (2015).
\newblock \doi{10.1093/mnras/stv1915}

\bibitem{ndugu18}
{Ndugu}, N., {Bitsch}, B., {Jurua}, E.: {Planet population synthesis driven by
  pebble accretion in cluster environments}.
\newblock \mnras \textbf{474}(1), 886--897 (2018).
\newblock \doi{10.1093/mnras/stx2815}

\bibitem{neishtadt84}
{Neishtadt}, A.: {The separation of motions in systems with rapidly rotating
  phase}.
\newblock Journal of Applied Mathematics and Mechanics \textbf{48}(2), 133--139
  (1984).
\newblock \doi{10.1016/0021-8928(84)90078-9}

\bibitem{nesvorny15}
{Nesvorn{\'y}}, D.: {Evidence for Slow Migration of Neptune from the
  Inclination Distribution of Kuiper Belt Objects}.
\newblock \aj \textbf{150}, 73 (2015).
\newblock \doi{10.1088/0004-6256/150/3/73}

\bibitem{nesvorny18b}
{Nesvorn{\'y}}, D.: {Dynamical Evolution of the Early Solar System}.
\newblock \araa \textbf{56}, 137--174 (2018).
\newblock \doi{10.1146/annurev-astro-081817-052028}

\bibitem{Nesvorny19}
{Nesvorn{\'y}}, D., {Li}, R., {Youdin}, A.N., {Simon}, J.B., {Grundy}, W.M.:
  {Trans-Neptunian binaries as evidence for planetesimal formation by the
  streaming instability}.
\newblock Nature Astronomy \textbf{3}, 808--812 (2019).
\newblock \doi{10.1038/s41550-019-0806-z}

\bibitem{nesvorny12}
{Nesvorn{\'y}}, D., {Morbidelli}, A.: {Statistical Study of the Early Solar
  System's Instability with Four, Five, and Six Giant Planets}.
\newblock \aj \textbf{144}, 117 (2012).
\newblock \doi{10.1088/0004-6256/144/4/117}

\bibitem{nesvorny18}
{Nesvorn{\'y}}, D., {Vokrouhlick{\'y}}, D., {Bottke}, W.F., {Levison}, H.F.:
  {Evidence for very early migration of the Solar System planets from the
  Patroclus-Menoetius binary Jupiter Trojan}.
\newblock Nature Astronomy \textbf{2}, 878--882 (2018).
\newblock \doi{10.1038/s41550-018-0564-3}

\bibitem{nesvorny14}
{Nesvorn{\'y}}, D., {Vokrouhlick{\'y}}, D., {Deienno}, R.: {Capture of
  Irregular Satellites at Jupiter}.
\newblock \apj \textbf{784}(1), 22 (2014).
\newblock \doi{10.1088/0004-637X/784/1/22}

\bibitem{nesvorny13}
{Nesvorn{\'y}}, D., {Vokrouhlick{\'y}}, D., {Morbidelli}, A.: {Capture of
  Trojans by Jumping Jupiter}.
\newblock \apj \textbf{768}, 45 (2013).
\newblock \doi{10.1088/0004-637X/768/1/45}

\bibitem{nesvorny10b}
{Nesvorn{\'y}}, D., {Youdin}, A.N., {Richardson}, D.C.: {Formation of Kuiper
  Belt Binaries by Gravitational Collapse}.
\newblock \aj \textbf{140}(3), 785--793 (2010).
\newblock \doi{10.1088/0004-6256/140/3/785}

\bibitem{nimmo07}
{Nimmo}, F., {Kleine}, T.: {How rapidly did Mars accrete? Uncertainties in the
  Hf W timing of core formation}.
\newblock Icarus \textbf{191}, 497--504 (2007).
\newblock \doi{10.1016/j.icarus.2007.05.002}

\bibitem{noll08}
{Noll}, K.S., {Grundy}, W.M., {Chiang}, E.I., {Margot}, J.L., {Kern}, S.D.:
  {Binaries in the Kuiper Belt}, p. 345 (2008)

\bibitem{nomura14}
{Nomura}, R., {Hirose}, K., {Uesegi}, K., {Ohishi}, Y., {Tsuchiyama}, A.,
  {Miyake}, A., {Ueno}, Y.: {Low Core-Mantle Boundary Temperature Inferred from
  the Solidus of Pyrolite}.
\newblock Science \textbf{343}, 522--525 (2014)

\bibitem{nyquist09}
{Nyquist}, L.E., {Kleine}, T., {Shih}, C.Y., {Reese}, Y.D.: {The distribution
  of short-lived radioisotopes in the early solar system and the chronology of
  asteroid accretion, differentiation, and secondary mineralization}.
\newblock \gca \textbf{73}, 5115--5136 (2009).
\newblock \doi{10.1016/j.gca.2008.12.031}

\bibitem{obrien18}
{O'Brien}, D.P., {Izidoro}, A., {Jacobson}, S.A., {Raymond}, S.N., {Rubie},
  D.C.: {The Delivery of Water During Terrestrial Planet Formation}.
\newblock \ssr \textbf{214}(1), 47 (2018).
\newblock \doi{10.1007/s11214-018-0475-8}

\bibitem{obrien06}
{O'Brien}, D.P., {Morbidelli}, A., {Levison}, H.F.: {Terrestrial planet
  formation with strong dynamical friction}.
\newblock Icarus \textbf{184}, 39--58 (2006).
\newblock \doi{10.1016/j.icarus.2006.04.005}

\bibitem{obrien14}
{O'Brien}, D.P., {Walsh}, K.J., {Morbidelli}, A., {Raymond}, S.N., {Mandell},
  A.M.: {Water delivery and giant impacts in the Grand Tack scenario}.
\newblock Icarus \textbf{239}, 74--84 (2014).
\newblock \doi{10.1016/j.icarus.2014.05.009}

\bibitem{ogihara09}
{Ogihara}, M., {Ida}, S.: {N-Body Simulations of Planetary Accretion Around M
  Dwarf Stars}.
\newblock \apj \textbf{699}, 824--838 (2009).
\newblock \doi{10.1088/0004-637X/699/1/824}

\bibitem{ogihara18}
{Ogihara}, M., {Kokubo}, E., {Suzuki}, T.K., {Morbidelli}, A.: {Formation of
  close-in super-Earths in evolving protoplanetary disks due to disk winds}.
\newblock \aap \textbf{615}, A63 (2018).
\newblock \doi{10.1051/0004-6361/201832720}

\bibitem{ogihara18b}
{Ogihara}, M., {Kokubo}, E., {Suzuki}, T.K., {Morbidelli}, A.: {Formation of
  the terrestrial planets in the solar system around 1 au via radial
  concentration of planetesimals}.
\newblock \aap \textbf{612}, L5 (2018).
\newblock \doi{10.1051/0004-6361/201832654}

\bibitem{ogihara15}
{Ogihara}, M., {Morbidelli}, A., {Guillot}, T.: {A reassessment of the in situ
  formation of close-in super-Earths}.
\newblock \aap \textbf{578}, A36 (2015).
\newblock \doi{10.1051/0004-6361/201525884}

\bibitem{oka11}
{Oka}, A., {Nakamoto}, T., {Ida}, S.: {Evolution of Snow Line in Optically
  Thick Protoplanetary Disks: Effects of Water Ice Opacity and Dust Grain
  Size}.
\newblock \apj \textbf{738}(2), 141 (2011).
\newblock \doi{10.1088/0004-637X/738/2/141}

\bibitem{okuzumi12}
{Okuzumi}, S., {Tanaka}, H., {Kobayashi}, H., {Wada}, K.: {Rapid Coagulation of
  Porous Dust Aggregates outside the Snow Line: A Pathway to Successful Icy
  Planetesimal Formation}.
\newblock \apj \textbf{752}(2), 106 (2012).
\newblock \doi{10.1088/0004-637X/752/2/106}

\bibitem{ormel10}
{Ormel}, C.W., {Klahr}, H.H.: {The effect of gas drag on the growth of
  protoplanets. Analytical expressions for the accretion of small bodies in
  laminar disks}.
\newblock \aap \textbf{520}, A43 (2010).
\newblock \doi{10.1051/0004-6361/201014903}

\bibitem{owen11}
{Owen}, J.E., {Ercolano}, B., {Clarke}, C.J.: {Protoplanetary disc evolution
  and dispersal: the implications of X-ray photoevaporation}.
\newblock \mnras \textbf{412}(1), 13--25 (2011).
\newblock \doi{10.1111/j.1365-2966.2010.17818.x}

\bibitem{owen13}
{Owen}, J.E., {Wu}, Y.: {Kepler Planets: A Tale of Evaporation}.
\newblock \apj \textbf{775}, 105 (2013).
\newblock \doi{10.1088/0004-637X/775/2/105}

\bibitem{owen17}
{Owen}, J.E., {Wu}, Y.: {The Evaporation Valley in the Kepler Planets}.
\newblock \apj \textbf{847}, 29 (2017).
\newblock \doi{10.3847/1538-4357/aa890a}

\bibitem{paardekooper14}
{Paardekooper}, S.J.: {Dynamical corotation torques on low-mass planets}.
\newblock \mnras \textbf{444}, 2031--2042 (2014).
\newblock \doi{10.1093/mnras/stu1542}

\bibitem{paardekooper10}
{Paardekooper}, S.J., {Baruteau}, C., {Crida}, A., {Kley}, W.: {A torque
  formula for non-isothermal type I planetary migration - I. Unsaturated
  horseshoe drag}.
\newblock \mnras \textbf{401}, 1950--1964 (2010).
\newblock \doi{10.1111/j.1365-2966.2009.15782.x}

\bibitem{paardekooper11}
{Paardekooper}, S.J., {Baruteau}, C., {Kley}, W.: {A torque formula for
  non-isothermal Type I planetary migration - II. Effects of diffusion}.
\newblock \mnras \textbf{410}, 293--303 (2011).
\newblock \doi{10.1111/j.1365-2966.2010.17442.x}

\bibitem{paardekooper06}
{Paardekooper}, S.J., {Mellema}, G.: {Halting type I planet migration in
  non-isothermal disks}.
\newblock \aap \textbf{459}, L17--L20 (2006).
\newblock \doi{10.1051/0004-6361:20066304}

\bibitem{paetzold19}
{P{\"a}tzold}, M., {Andert}, T.P., {Hahn}, M., {Barriot}, J.P., {Asmar}, S.W.,
  {H{\"a}usler}, B., {Bird}, M.K., {Tellmann}, S., {Oschlisniok}, J., {Peter},
  K.: {The Nucleus of comet 67P/Churyumov-Gerasimenko - Part I: The global view
  - nucleus mass, mass-loss, porosity, and implications}.
\newblock \mnras \textbf{483}(2), 2337--2346 (2019).
\newblock \doi{10.1093/mnras/sty3171}

\bibitem{pecaut16}
{Pecaut}, M.J., {Mamajek}, E.E.: {The star formation history and accretion-disc
  fraction among the K-type members of the Scorpius-Centaurus OB association}.
\newblock \mnras \textbf{461}(1), 794--815 (2016).
\newblock \doi{10.1093/mnras/stw1300}

\bibitem{petigura13}
{Petigura}, E.A., {Howard}, A.W., {Marcy}, G.W.: {Prevalence of Earth-size
  planets orbiting Sun-like stars}.
\newblock Proceedings of the National Academy of Science \textbf{110},
  19273--19278 (2013)

\bibitem{pfalzner14}
{Pfalzner}, S., {Steinhausen}, M., {Menten}, K.: {Short Dissipation Times of
  Proto-planetary Disks: An Artifact of Selection Effects?}
\newblock \apjl \textbf{793}, L34 (2014).
\newblock \doi{10.1088/2041-8205/793/2/L34}

\bibitem{pichierri18}
{Pichierri}, G., {Morbidelli}, A., {Crida}, A.: {Capture into first-order
  resonances and long-term stability of pairs of equal-mass planets}.
\newblock Celestial Mechanics and Dynamical Astronomy \textbf{130}(8), 54
  (2018).
\newblock \doi{10.1007/s10569-018-9848-2}

\bibitem{pierens15}
{Pierens}, A.: {Fast migration of low-mass planets in radiative discs}.
\newblock \mnras \textbf{454}, 2003--2014 (2015).
\newblock \doi{10.1093/mnras/stv2024}

\bibitem{pierens08}
{Pierens}, A., {Nelson}, R.P.: {Constraints on resonant-trapping for two
  planets embedded in a protoplanetary disc}.
\newblock \aap \textbf{482}, 333--340 (2008).
\newblock \doi{10.1051/0004-6361:20079062}

\bibitem{pierens11}
{Pierens}, A., {Raymond}, S.N.: {Two phase, inward-then-outward migration of
  Jupiter and Saturn in the gaseous solar nebula}.
\newblock \aap \textbf{533}, A131 (2011).
\newblock \doi{10.1051/0004-6361/201117451}

\bibitem{pierens16}
{Pierens}, A., {Raymond}, S.N.: {Migration of accreting planets in radiative
  discs from dynamical torques}.
\newblock \mnras \textbf{462}(4), 4130--4140 (2016).
\newblock \doi{10.1093/mnras/stw1904}

\bibitem{pierens14}
{Pierens}, A., {Raymond}, S.N., {Nesvorny}, D., {Morbidelli}, A.: {Outward
  Migration of Jupiter and Saturn in 3:2 or 2:1 Resonance in Radiative Disks:
  Implications for the Grand Tack and Nice models}.
\newblock \apjl \textbf{795}, L11 (2014).
\newblock \doi{10.1088/2041-8205/795/1/L11}

\bibitem{pinte16}
{Pinte}, C., {Dent}, W.R.F., {M{\'e}nard}, F., {Hales}, A., {Hill}, T.,
  {Cortes}, P., {de Gregorio-Monsalvo}, I.: {Dust and Gas in the Disk of HL
  Tauri: Surface Density, Dust Settling, and Dust-to-gas Ratio}.
\newblock \apj \textbf{816}(1), 25 (2016).
\newblock \doi{10.3847/0004-637X/816/1/25}

\bibitem{pirani19}
{Pirani}, S., {Johansen}, A., {Bitsch}, B., {Mustill}, A.J., {Turrini}, D.:
  {Consequences of planetary migration on the minor bodies of the early solar
  system}.
\newblock \aap \textbf{623}, A169 (2019).
\newblock \doi{10.1051/0004-6361/201833713}

\bibitem{piso14}
{Piso}, A.M.A., {Youdin}, A.N.: {On the Minimum Core Mass for Giant Planet
  Formation at Wide Separations}.
\newblock \apj \textbf{786}(1), 21 (2014).
\newblock \doi{10.1088/0004-637X/786/1/21}

\bibitem{poincare1892}
{Poincare}, H.: {Les methodes nouvelles de la mecanique celeste} (1892)

\bibitem{poincare1897}
{Poincare}, H.: {Sur une forme Nouvelle des Equations du Probleme des Trois
  Corps}.
\newblock Bulletin Astronomique, Serie I \textbf{14}, 53--67 (1897)

\bibitem{pollack96}
{Pollack}, J.B., {Hubickyj}, O., {Bodenheimer}, P., {Lissauer}, J.J.,
  {Podolak}, M., {Greenzweig}, Y.: {Formation of the Giant Planets by
  Concurrent Accretion of Solids and Gas}.
\newblock Icarus \textbf{124}, 62--85 (1996).
\newblock \doi{10.1006/icar.1996.0190}

\bibitem{quarles19}
{Quarles}, B., {Kaib}, N.: {Instabilities in the Early Solar System Due to a
  Self-gravitating Disk}.
\newblock \aj \textbf{157}(2), 67 (2019).
\newblock \doi{10.3847/1538-3881/aafa71}

\bibitem{quintana16}
{Quintana}, E.V., {Barclay}, T., {Borucki}, W.J., {Rowe}, J.F., {Chambers},
  J.E.: {The Frequency of Giant Impacts on Earth-like Worlds}.
\newblock \apj \textbf{821}, 126 (2016).
\newblock \doi{10.3847/0004-637X/821/2/126}

\bibitem{quintana14}
{Quintana}, E.V., {Barclay}, T., {Raymond}, S.N., {Rowe}, J.F., {Bolmont}, E.,
  {Caldwell}, D.A., {Howell}, S.B., {Kane}, S.R., {Huber}, D., {Crepp}, J.R.,
  {Lissauer}, J.J., {Ciardi}, D.R., {Coughlin}, J.L., {Everett}, M.E., {Henze},
  C.E., {Horch}, E., {Isaacson}, H., {Ford}, E.B., {Adams}, F.C., {Still}, M.,
  {Hunter}, R.C., {Quarles}, B., {Selsis}, F.: {An Earth-Sized Planet in the
  Habitable Zone of a Cool Star}.
\newblock Science \textbf{344}, 277--280 (2014).
\newblock \doi{10.1126/science.1249403}

\bibitem{rafikov04}
{Rafikov}, R.R.: {Fast Accretion of Small Planetesimals by Protoplanetary
  Cores}.
\newblock \aj \textbf{128}, 1348--1363 (2004).
\newblock \doi{10.1086/423216}

\bibitem{rasio96}
{Rasio}, F.A., {Ford}, E.B.: {Dynamical instabilities and the formation of
  extrasolar planetary systems}.
\newblock Science \textbf{274}, 954--956 (1996).
\newblock \doi{10.1126/science.274.5289.954}

\bibitem{raymond10}
{Raymond}, S.N., {Armitage}, P.J., {Gorelick}, N.: {Planet-Planet Scattering in
  Planetesimal Disks. II. Predictions for Outer Extrasolar Planetary Systems}.
\newblock \apj \textbf{711}, 772--795 (2010).
\newblock \doi{10.1088/0004-637X/711/2/772}

\bibitem{raymond11}
{Raymond}, S.N., {Armitage}, P.J., {Moro-Mart{\'{\i}}n}, A., {Booth}, M.,
  {Wyatt}, M.C., {Armstrong}, J.C., {Mandell}, A.M., {Selsis}, F., {West},
  A.A.: {Debris disks as signposts of terrestrial planet formation}.
\newblock \aap \textbf{530}, A62 (2011).
\newblock \doi{10.1051/0004-6361/201116456}

\bibitem{raymond12}
{Raymond}, S.N., {Armitage}, P.J., {Moro-Mart{\'{\i}}n}, A., {Booth}, M.,
  {Wyatt}, M.C., {Armstrong}, J.C., {Mandell}, A.M., {Selsis}, F., {West},
  A.A.: {Debris disks as signposts of terrestrial planet formation. II.
  Dependence of exoplanet architectures on giant planet and disk properties}.
\newblock \aap \textbf{541}, A11 (2012).
\newblock \doi{10.1051/0004-6361/201117049}

\bibitem{raymond18c}
{Raymond}, S.N., {Armitage}, P.J., {Veras}, D.: {Interstellar Object
  {\textquoteright}Oumuamua as an Extinct Fragment of an Ejected Cometary
  Planetesimal}.
\newblock \apjl \textbf{856}(1), L7 (2018).
\newblock \doi{10.3847/2041-8213/aab4f6}

\bibitem{raymond18}
{Raymond}, S.N., {Armitage}, P.J., {Veras}, D., {Quintana}, E.V., {Barclay},
  T.: {Implications of the interstellar object 1I/'Oumuamua for planetary
  dynamics and planetesimal formation}.
\newblock \mnras \textbf{476}, 3031--3038 (2018).
\newblock \doi{10.1093/mnras/sty468}

\bibitem{raymond08b}
{Raymond}, S.N., {Barnes}, R., {Armitage}, P.J., {Gorelick}, N.: {Mean Motion
  Resonances from Planet-Planet Scattering}.
\newblock \apjl \textbf{687}, L107--L110 (2008).
\newblock \doi{10.1086/593301}

\bibitem{raymond08a}
{Raymond}, S.N., {Barnes}, R., {Mandell}, A.M.: {Observable consequences of
  planet formation models in systems with close-in terrestrial planets}.
\newblock \mnras \textbf{384}, 663--674 (2008).
\newblock \doi{10.1111/j.1365-2966.2007.12712.x}

\bibitem{raymond09a}
{Raymond}, S.N., {Barnes}, R., {Veras}, D., {Armitage}, P.J., {Gorelick}, N.,
  {Greenberg}, R.: {Planet-Planet Scattering Leads to Tightly Packed Planetary
  Systems}.
\newblock \apjl \textbf{696}, L98--L101 (2009).
\newblock \doi{10.1088/0004-637X/696/1/L98}

\bibitem{raymond18b}
{Raymond}, S.N., {Boulet}, T., {Izidoro}, A., {Esteves}, L., {Bitsch}, B.:
  {Migration-driven diversity of super-Earth compositions}.
\newblock \mnras \textbf{479}, L81--L85 (2018).
\newblock \doi{10.1093/mnrasl/sly100}

\bibitem{raymond14b}
{Raymond}, S.N., {Cossou}, C.: {No universal minimum-mass extrasolar nebula:
  evidence against in situ accretion of systems of hot super-Earths}.
\newblock \mnras \textbf{440}, L11--L15 (2014).
\newblock \doi{10.1093/mnrasl/slu011}

\bibitem{raymond17}
{Raymond}, S.N., {Izidoro}, A.: {Origin of water in the inner Solar System:
  Planetesimals scattered inward during Jupiter and Saturn's rapid gas
  accretion}.
\newblock Icarus \textbf{297}, 134--148 (2017).
\newblock \doi{10.1016/j.icarus.2017.06.030}

\bibitem{raymond17b}
{Raymond}, S.N., {Izidoro}, A.: {The empty primordial asteroid belt}.
\newblock Science Advances \textbf{3}, e1701138 (2017).
\newblock \doi{10.1126/sciadv.1701138}

\bibitem{raymond18d}
{Raymond}, S.N., {Izidoro}, A., {Morbidelli}, A.: {Solar System Formation in
  the Context of Extra-Solar Planets}.
\newblock arXiv e-prints arXiv:1812.01033 (2018)

\bibitem{raymond14}
{Raymond}, S.N., {Kokubo}, E., {Morbidelli}, A., {Morishima}, R., {Walsh},
  K.J.: {Terrestrial Planet Formation at Home and Abroad}.
\newblock Protostars and Planets VI pp. 595--618 (2014)

\bibitem{raymond06c}
{Raymond}, S.N., {Mandell}, A.M., {Sigurdsson}, S.: {Exotic Earths: Forming
  Habitable Worlds with Giant Planet Migration}.
\newblock Science \textbf{313}, 1413--1416 (2006).
\newblock \doi{10.1126/science.1130461}

\bibitem{raymond14c}
{Raymond}, S.N., {Morbidelli}, A.: {The Grand Tack model: a critical review}.
\newblock In: Complex Planetary Systems, Proceedings of the International
  Astronomical Union, \emph{IAU Symposium}, vol. 310, pp. 194--203 (2014).
\newblock \doi{10.1017/S1743921314008254}

\bibitem{raymond09c}
{Raymond}, S.N., {O'Brien}, D.P., {Morbidelli}, A., {Kaib}, N.A.: {Building the
  terrestrial planets: Constrained accretion in the inner Solar System}.
\newblock Icarus \textbf{203}, 644--662 (2009).
\newblock \doi{10.1016/j.icarus.2009.05.016}

\bibitem{raymond04}
{Raymond}, S.N., {Quinn}, T., {Lunine}, J.I.: {Making other earths: dynamical
  simulations of terrestrial planet formation and water delivery}.
\newblock Icarus \textbf{168}, 1--17 (2004).
\newblock \doi{10.1016/j.icarus.2003.11.019}

\bibitem{raymond06b}
{Raymond}, S.N., {Quinn}, T., {Lunine}, J.I.: {High-resolution simulations of
  the final assembly of Earth-like planets I. Terrestrial accretion and
  dynamics}.
\newblock Icarus \textbf{183}, 265--282 (2006).
\newblock \doi{10.1016/j.icarus.2006.03.011}

\bibitem{raymond07a}
{Raymond}, S.N., {Quinn}, T., {Lunine}, J.I.: {High-Resolution Simulations of
  The Final Assembly of Earth-Like Planets. 2. Water Delivery And Planetary
  Habitability}.
\newblock Astrobiology \textbf{7}, 66--84 (2007).
\newblock \doi{10.1089/ast.2006.06-0126}

\bibitem{raymond07b}
{Raymond}, S.N., {Scalo}, J., {Meadows}, V.S.: {A Decreased Probability of
  Habitable Planet Formation around Low-Mass Stars}.
\newblock \apj \textbf{669}, 606--614 (2007).
\newblock \doi{10.1086/521587}

\bibitem{raymond13}
{Raymond}, S.N., {Schlichting}, H.E., {Hersant}, F., {Selsis}, F.: {Dynamical
  and collisional constraints on a stochastic late veneer on the terrestrial
  planets}.
\newblock \icarus \textbf{226}(1), 671--681 (2013).
\newblock \doi{10.1016/j.icarus.2013.06.019}

\bibitem{ribas07}
{Ribas}, I., {Miralda-Escud{\'e}}, J.: {The eccentricity-mass distribution of
  exoplanets: signatures of different formation mechanisms?}
\newblock \aap \textbf{464}, 779--785 (2007).
\newblock \doi{10.1051/0004-6361:20065726}

\bibitem{ribeiro20}
{Ribeiro}, R., {Morbidelli}, A., {Raymond}, S., {Izidoro}, A., {Gomes}, R.:
  {Dynamical evidence for an early giant planet instability}.
\newblock Submitted to Icarus  (2020)

\bibitem{rivera10}
{Rivera}, E.J., {Laughlin}, G., {Butler}, R.P., {Vogt}, S.S., {Haghighipour},
  N., {Meschiari}, S.: {The Lick-Carnegie Exoplanet Survey: a Uranus-Mass
  Fourth Planet for GJ 876 in an Extrasolar Laplace Configuration}.
\newblock \apj \textbf{719}, 890--899 (2010).
\newblock \doi{10.1088/0004-637X/719/1/890}

\bibitem{robert18}
{Robert}, C.M.T., {Crida}, A., {Lega}, E., {M{\'e}heut}, H., {Morbidelli}, A.:
  {Toward a new paradigm for Type II migration}.
\newblock \aap \textbf{617}, A98 (2018).
\newblock \doi{10.1051/0004-6361/201833539}

\bibitem{robert77}
{Robert}, F., {Merlivat}, L., {Javoy}, M.: {Water and Deuterium Content in
  Eight Condrites}.
\newblock Meteoritics \textbf{12}, 349 (1977)

\bibitem{rogers15}
{Rogers}, L.A.: {Most 1.6 Earth-radius Planets are Not Rocky}.
\newblock \apj \textbf{801}, 41 (2015).
\newblock \doi{10.1088/0004-637X/801/1/41}

\bibitem{ronnet18}
{Ronnet}, T., {Mousis}, O., {Vernazza}, P., {Lunine}, J.I., {Crida}, A.:
  {Saturn{\textquoteright}s Formation and Early Evolution at the Origin of
  Jupiter{\textquoteright}s Massive Moons}.
\newblock \aj \textbf{155}(5), 224 (2018).
\newblock \doi{10.3847/1538-3881/aabcc7}

\bibitem{rowan16}
{Rowan}, D., {Meschiari}, S., {Laughlin}, G., {Vogt}, S.S., {Butler}, R.P.,
  {Burt}, J., {Wang}, S., {Holden}, B., {Hanson}, R., {Arriagada}, P.,
  {Keiser}, S., {Teske}, J., {Diaz}, M.: {The Lick-Carnegie Exoplanet Survey:
  HD 32963 -- A New Jupiter Analog Orbiting a Sun-like Star}.
\newblock \apj \textbf{817}, 104 (2016).
\newblock \doi{10.3847/0004-637X/817/2/104}

\bibitem{rowe14}
{Rowe}, J.F., {Bryson}, S.T., {Marcy}, G.W., {Lissauer}, J.J., {Jontof-Hutter},
  D., {Mullally}, F., {Gilliland}, R.L., {Issacson}, H., {Ford}, E., {Howell},
  S.B., {Borucki}, W.J., {Haas}, M., {Huber}, D., {Steffen}, J.H., {Thompson},
  S.E., {Quintana}, E., {Barclay}, T., {Still}, M., {Fortney}, J., {Gautier}
  III, T.N., {Hunter}, R., {Caldwell}, D.A., {Ciardi}, D.R., {Devore}, E.,
  {Cochran}, W., {Jenkins}, J., {Agol}, E., {Carter}, J.A., {Geary}, J.:
  {Validation of Kepler's Multiple Planet Candidates. III. Light Curve Analysis
  and Announcement of Hundreds of New Multi-planet Systems}.
\newblock \apj \textbf{784}, 45 (2014).
\newblock \doi{10.1088/0004-637X/784/1/45}

\bibitem{rubie15}
{Rubie}, D.C., {Jacobson}, S.A., {Morbidelli}, A., {O'Brien}, D.P., {Young},
  E.D., {de Vries}, J., {Nimmo}, F., {Palme}, H., {Frost}, D.J.: {Accretion and
  differentiation of the terrestrial planets with implications for the
  compositions of early-formed Solar System bodies and accretion of water}.
\newblock \icarus \textbf{248}, 89--108 (2015).
\newblock \doi{10.1016/j.icarus.2014.10.015}

\bibitem{safronov72}
{Safronov}, V.S.: {Evolution of the protoplanetary cloud and formation of the
  earth and planets.} (1972)

\bibitem{santos01}
{Santos}, N.C., {Israelian}, G., {Mayor}, M.: {The metal-rich nature of stars
  with planets}.
\newblock \aap \textbf{373}, 1019--1031 (2001).
\newblock \doi{10.1051/0004-6361:20010648}

\bibitem{sasselov00}
{Sasselov}, D.D., {Lecar}, M.: {On the Snow Line in Dusty Protoplanetary
  Disks}.
\newblock \apj \textbf{528}, 995--998 (2000).
\newblock \doi{10.1086/308209}

\bibitem{sato16}
{Sato}, T., {Okuzumi}, S., {Ida}, S.: {On the water delivery to terrestrial
  embryos by ice pebble accretion}.
\newblock \aap \textbf{589}, A15 (2016).
\newblock \doi{10.1051/0004-6361/201527069}

\bibitem{schaefer17}
{Sch{\"a}fer}, U., {Yang}, C.C., {Johansen}, A.: {Initial mass function of
  planetesimals formed by the streaming instability}.
\newblock \aap \textbf{597}, A69 (2017).
\newblock \doi{10.1051/0004-6361/201629561}

\bibitem{schiller18}
{Schiller}, M., {Bizzarro}, M., {Fernandes}, V.A.: {Isotopic evolution of the
  protoplanetary disk and the building blocks of Earth and the Moon}.
\newblock \nat \textbf{555}(7697), 507--510 (2018).
\newblock \doi{10.1038/nature25990}

\bibitem{schiller15}
{Schiller}, M., {Connelly}, J.N., {Glad}, A.C., {Mikouchi}, T., {Bizzarro}, M.:
  {Early accretion of protoplanets inferred from a reduced inner solar system
  $^{26}$Al inventory}.
\newblock Earth and Planetary Science Letters \textbf{420}, 45--54 (2015).
\newblock \doi{10.1016/j.epsl.2015.03.028}

\bibitem{schlichting14}
{Schlichting}, H.E.: {Formation of Close in Super-Earths and Mini-Neptunes:
  Required Disk Masses and their Implications}.
\newblock \apjl \textbf{795}, L15 (2014).
\newblock \doi{10.1088/2041-8205/795/1/L15}

\bibitem{schoonenberg17}
{Schoonenberg}, D., {Ormel}, C.W.: {Planetesimal formation near the snowline:
  in or out?}
\newblock \aap \textbf{602}, A21 (2017).
\newblock \doi{10.1051/0004-6361/201630013}

\bibitem{seager07}
{Seager}, S., {Kuchner}, M., {Hier-Majumder}, C.A., {Militzer}, B.:
  {Mass-Radius Relationships for Solid Exoplanets}.
\newblock \apj \textbf{669}(2), 1279--1297 (2007).
\newblock \doi{10.1086/521346}

\bibitem{selsis07b}
{Selsis}, F., {Chazelas}, B., {Bord{\'e}}, P., {Ollivier}, M., {Brachet}, F.,
  {Decaudin}, M., {Bouchy}, F., {Ehrenreich}, D., {Grie{\ss}meier}, J.M.,
  {Lammer}, H., {Sotin}, C., {Grasset}, O., {Moutou}, C., {Barge}, P.,
  {Deleuil}, M., {Mawet}, D., {Despois}, D., {Kasting}, J.F., {L{\'e}ger}, A.:
  {Could we identify hot ocean-planets with CoRoT, Kepler and Doppler
  velocimetry?}
\newblock Icarus \textbf{191}, 453--468 (2007).
\newblock \doi{10.1016/j.icarus.2007.04.010}

\bibitem{sessin84}
{Sessin}, W., {Ferraz-Mello}, S.: {Motion of two planets with periods
  commensurable in the ratio 2{\ensuremath{:}}1 solutions of the hori auxiliary
  system}.
\newblock Celestial Mechanics \textbf{32}(4), 307--332 (1984).
\newblock \doi{10.1007/BF01229087}

\bibitem{shakura73}
{Shakura}, N.I., {Sunyaev}, R.A.: {Black holes in binary systems. Observational
  appearance.}
\newblock \aap \textbf{24}, 337--355 (1973)

\bibitem{sharp17}
{Sharp}, Z.D.: {Nebular ingassing as a source of volatiles to the Terrestrial
  planets}.
\newblock Chemical Geology \textbf{448}, 137--150 (2017).
\newblock \doi{10.1016/j.chemgeo.2016.11.018}

\bibitem{simon16}
{Simon}, J.B., {Armitage}, P.J., {Li}, R., {Youdin}, A.N.: {The Mass and Size
  Distribution of Planetesimals Formed by the Streaming Instability. I. The
  Role of Self-gravity}.
\newblock \apj \textbf{822}, 55 (2016).
\newblock \doi{10.3847/0004-637X/822/1/55}

\bibitem{simon17}
{Simon}, J.B., {Armitage}, P.J., {Youdin}, A.N., {Li}, R.: {Evidence for
  Universality in the Initial Planetesimal Mass Function}.
\newblock \apjl \textbf{847}, L12 (2017).
\newblock \doi{10.3847/2041-8213/aa8c79}

\bibitem{snellgrove01}
{Snellgrove}, M.D., {Papaloizou}, J.C.B., {Nelson}, R.P.: {On disc driven
  inward migration of resonantly coupled planets with application to the system
  around GJ876}.
\newblock \aap \textbf{374}, 1092--1099 (2001).
\newblock \doi{10.1051/0004-6361:20010779}

\bibitem{sosa11}
{Sosa}, A., {Fern{\'a}ndez}, J.A.: {Masses of long-period comets derived from
  non-gravitational effects - analysis of the computed results and the
  consistency and reliability of the non-gravitational parameters}.
\newblock \mnras \textbf{416}(1), 767--782 (2011).
\newblock \doi{10.1111/j.1365-2966.2011.19111.x}

\bibitem{sotin07}
{Sotin}, C., {Grasset}, O., {Mocquet}, A.: {Mass radius curve for extrasolar
  Earth-like planets and ocean planets}.
\newblock \icarus \textbf{191}(1), 337--351 (2007).
\newblock \doi{10.1016/j.icarus.2007.04.006}

\bibitem{stimpfl06}
{Stimpfl}, M., {Walker}, A.M., {Drake}, M.J., {de Leeuw}, N.H., {Deymier}, P.:
  {An {\r{a}}ngstr{\"o}m-sized window on the origin of water in the inner solar
  system: Atomistic simulation of adsorption of water on olivine}.
\newblock Journal of Crystal Growth \textbf{294}(1), 83--95 (2006).
\newblock \doi{10.1016/j.jcrysgro.2006.05.057}

\bibitem{stone98}
{Stone}, J.M., {Ostriker}, E.C., {Gammie}, C.F.: {Dissipation in Compressible
  Magnetohydrodynamic Turbulence}.
\newblock \apjl \textbf{508}(1), L99--L102 (1998).
\newblock \doi{10.1086/311718}

\bibitem{su06}
{Su}, K.Y.L., {Rieke}, G.H., {Stansberry}, J.A., {Bryden}, G., {Stapelfeldt},
  K.R., {Trilling}, D.E., {Muzerolle}, J., {Beichman}, C.A., {Moro-Martin}, A.,
  {Hines}, D.C., {Werner}, M.W.: {Debris Disk Evolution around A Stars}.
\newblock \apj \textbf{653}, 675--689 (2006).
\newblock \doi{10.1086/508649}

\bibitem{suzuki16b}
{Suzuki}, D., {Bennett}, D.P., {Sumi}, T., {Bond}, I.A., {Rogers}, L.A., {Abe},
  F., {Asakura}, Y., {Bhattacharya}, A., {Donachie}, M., {Freeman}, M.,
  {Fukui}, A., {Hirao}, Y., {Itow}, Y., {Koshimoto}, N., {Li}, M.C.A., {Ling},
  C.H., {Masuda}, K., {Matsubara}, Y., {Muraki}, Y., {Nagakane}, M., {Onishi},
  K., {Oyokawa}, H., {Rattenbury}, N., {Saito}, T., {Sharan}, A., {Shibai}, H.,
  {Sullivan}, D.J., {Tristram}, P.J., {Yonehara}, A., {MOA Collaboration}: {The
  Exoplanet Mass-ratio Function from the MOA-II Survey: Discovery of a Break
  and Likely Peak at a Neptune Mass}.
\newblock \apj \textbf{833}, 145 (2016).
\newblock \doi{10.3847/1538-4357/833/2/145}

\bibitem{suzuki16}
{Suzuki}, T.K., {Ogihara}, M., {Morbidelli}, A., {Crida}, A., {Guillot}, T.:
  {Evolution of protoplanetary discs with magnetically driven disc winds}.
\newblock \aap \textbf{596}, A74 (2016).
\newblock \doi{10.1051/0004-6361/201628955}

\bibitem{svetsov07}
{Svetsov}, V.V.: {Atmospheric erosion and replenishment induced by impacts of
  cosmic bodies upon the Earth and Mars}.
\newblock Solar System Research \textbf{41}(1), 28--41 (2007).
\newblock \doi{10.1134/S0038094607010030}

\bibitem{tanaka02}
{Tanaka}, H., {Takeuchi}, T., {Ward}, W.R.: {Three-Dimensional Interaction
  between a Planet and an Isothermal Gaseous Disk. I. Corotation and Lindblad
  Torques and Planet Migration}.
\newblock \apj \textbf{565}, 1257--1274 (2002).
\newblock \doi{10.1086/324713}

\bibitem{tanaka04}
{Tanaka}, H., {Ward}, W.R.: {Three-dimensional Interaction between a Planet and
  an Isothermal Gaseous Disk. II. Eccentricity Waves and Bending Waves}.
\newblock \apj \textbf{602}, 388--395 (2004).
\newblock \doi{10.1086/380992}

\bibitem{tera74}
{Tera}, F., {Papanastassiou}, D.A., {Wasserburg}, G.J.: {Isotopic evidence for
  a terminal lunar cataclysm}.
\newblock Earth and Planetary Science Letters \textbf{22}, 1 (1974).
\newblock \doi{10.1016/0012-821X(74)90059-4}

\bibitem{terquem07}
{Terquem}, C., {Papaloizou}, J.C.B.: {Migration and the Formation of Systems of
  Hot Super-Earths and Neptunes}.
\newblock \apj \textbf{654}, 1110--1120 (2007).
\newblock \doi{10.1086/509497}

\bibitem{thommes03}
{Thommes}, E.W., {Duncan}, M.J., {Levison}, H.F.: {Oligarchic growth of giant
  planets}.
\newblock Icarus \textbf{161}, 431--455 (2003).
\newblock \doi{10.1016/S0019-1035(02)00043-X}

\bibitem{thommes08}
{Thommes}, E.W., {Matsumura}, S., {Rasio}, F.A.: {Gas Disks to Gas Giants:
  Simulating the Birth of Planetary Systems}.
\newblock Science \textbf{321}, 814-- (2008).
\newblock \doi{10.1126/science.1159723}

\bibitem{throop08}
{Throop}, H.B., {Bally}, J.: {Tail-End Bondi-Hoyle Accretion in Young Star
  Clusters: Implications for Disks, Planets, and Stars}.
\newblock \aj \textbf{135}(6), 2380--2397 (2008).
\newblock \doi{10.1088/0004-6256/135/6/2380}

\bibitem{tominaga19}
{Tominaga}, R.T., {Takahashi}, S.Z., {Inutsuka}, S.i.: {Revised Description of
  Dust Diffusion and a New Instability Creating Multiple Rings in
  Protoplanetary Disks}.
\newblock \apj \textbf{881}(1), 53 (2019).
\newblock \doi{10.3847/1538-4357/ab25ea}

\bibitem{toomre64}
{Toomre}, A.: {On the gravitational stability of a disk of stars.}
\newblock \apj \textbf{139}, 1217--1238 (1964).
\newblock \doi{10.1086/147861}

\bibitem{touboul07}
{Touboul}, M., {Kleine}, T., {Bourdon}, B., {Palme}, H., {Wieler}, R.: {Late
  formation and prolonged differentiation of the Moon inferred from W isotopes
  in lunar metals}.
\newblock \nat \textbf{450}, 1206--1209 (2007).
\newblock \doi{10.1038/nature06428}

\bibitem{tremaine12}
{Tremaine}, S., {Dong}, S.: {The Statistics of Multi-planet Systems}.
\newblock \aj \textbf{143}, 94 (2012).
\newblock \doi{10.1088/0004-6256/143/4/94}

\bibitem{trilling08}
{Trilling}, D.E., {Bryden}, G., {Beichman}, C.A., {Rieke}, G.H., {Su}, K.Y.L.,
  {Stansberry}, J.A., {Blaylock}, M., {Stapelfeldt}, K.R., {Beeman}, J.W.,
  {Haller}, E.E.: {Debris Disks around Sun-like Stars}.
\newblock \apj \textbf{674}, 1086--1105 (2008).
\newblock \doi{10.1086/525514}

\bibitem{tsiganis05}
{Tsiganis}, K., {Gomes}, R., {Morbidelli}, A., {Levison}, H.F.: {Origin of the
  orbital architecture of the giant planets of the Solar System}.
\newblock \nat \textbf{435}, 459--461 (2005).
\newblock \doi{10.1038/nature03539}

\bibitem{turner14}
{Turner}, N.J., {Fromang}, S., {Gammie}, C., {Klahr}, H., {Lesur}, G.,
  {Wardle}, M., {Bai}, X.N.: {Transport and Accretion in Planet-Forming Disks}.
\newblock Protostars and Planets VI pp. 411--432 (2014)

\bibitem{udry07b}
{Udry}, S., {Santos}, N.C.: {Statistical Properties of Exoplanets}.
\newblock \araa \textbf{45}, 397--439 (2007).
\newblock \doi{10.1146/annurev.astro.45.051806.110529}

\bibitem{uribe13}
{Uribe}, A.L., {Klahr}, H., {Henning}, T.: {Accretion of Gas onto Gap-opening
  Planets and Circumplanetary Flow Structure in Magnetized Turbulent Disks}.
\newblock \apj \textbf{769}(2), 97 (2013).
\newblock \doi{10.1088/0004-637X/769/2/97}

\bibitem{valencia07}
{Valencia}, D., {Sasselov}, D.D., {O'Connell}, R.J.: {Detailed Models of
  Super-Earths: How Well Can We Infer Bulk Properties?}
\newblock \apj \textbf{665}, 1413--1420 (2007).
\newblock \doi{10.1086/519554}

\bibitem{varniere04}
{Varni{\`e}re}, P., {Quillen}, A.C., {Frank}, A.: {The Evolution of
  Protoplanetary Disk Edges}.
\newblock \apj \textbf{612}(2), 1152--1162 (2004).
\newblock \doi{10.1086/422542}

\bibitem{veras05}
{Veras}, D., {Armitage}, P.J.: {The Influence of Massive Planet Scattering on
  Nascent Terrestrial Planets}.
\newblock \apjl \textbf{620}, L111--L114 (2005).
\newblock \doi{10.1086/428831}

\bibitem{veras06}
{Veras}, D., {Armitage}, P.J.: {Predictions for the Correlation between Giant
  and Terrestrial Extrasolar Planets in Dynamically Evolved Systems}.
\newblock \apj \textbf{645}, 1509--1515 (2006).
\newblock \doi{10.1086/504582}

\bibitem{villeneuve09}
{Villeneuve}, J., {Chaussidon}, M., {Libourel}, G.: {Homogeneous Distribution
  of $^{26}$Al in the Solar System from the Mg Isotopic Composition of
  Chondrules}.
\newblock Science \textbf{325}(5943), 985 (2009).
\newblock \doi{10.1126/science.1173907}

\bibitem{walsh11}
{Walsh}, K.J., {Morbidelli}, A., {Raymond}, S.N., {O'Brien}, D.P., {Mandell},
  A.M.: {A low mass for Mars from Jupiter's early gas-driven migration}.
\newblock \nat \textbf{475}, 206--209 (2011).
\newblock \doi{10.1038/nature10201}

\bibitem{walsh12}
{Walsh}, K.J., {Morbidelli}, A., {Raymond}, S.N., {O'Brien}, D.P., {Mandell},
  A.M.: {Populating the asteroid belt from two parent source regions due to the
  migration of giant planets--``The Grand Tack''}.
\newblock Meteoritics and Planetary Science \textbf{47}, 1941--1947 (2012).
\newblock \doi{10.1111/j.1945-5100.2012.01418.x}

\bibitem{ward86}
{Ward}, W.R.: {Density waves in the solar nebula - Differential Lindblad
  torque}.
\newblock Icarus \textbf{67}, 164--180 (1986).
\newblock \doi{10.1016/0019-1035(86)90182-X}

\bibitem{ward97}
{Ward}, W.R.: {Protoplanet Migration by Nebula Tides}.
\newblock Icarus \textbf{126}, 261--281 (1997).
\newblock \doi{10.1006/icar.1996.5647}

\bibitem{warren11}
{Warren}, P.H.: {Stable-isotopic anomalies and the accretionary assemblage of
  the Earth and Mars: A subordinate role for carbonaceous chondrites}.
\newblock Earth and Planetary Science Letters \textbf{311}, 93--100 (2011).
\newblock \doi{10.1016/j.epsl.2011.08.047}

\bibitem{weber18}
{Weber}, P., {Ben{\'\i}tez-Llambay}, P., {Gressel}, O., {Krapp}, L., {Pessah},
  M.E.: {Characterizing the Variable Dust Permeability of Planet-induced Gaps}.
\newblock \apj \textbf{854}(2), 153 (2018).
\newblock \doi{10.3847/1538-4357/aaab63}

\bibitem{weidenschilling77b}
{Weidenschilling}, S.J.: {Aerodynamics of solid bodies in the solar nebula}.
\newblock \mnras \textbf{180}, 57--70 (1977)

\bibitem{weidenschilling77}
{Weidenschilling}, S.J.: {The distribution of mass in the planetary system and
  solar nebula}.
\newblock \apss \textbf{51}, 153--158 (1977).
\newblock \doi{10.1007/BF00642464}

\bibitem{weidenschilling96}
{Weidenschilling}, S.J., {Marzari}, F.: {Gravitational scattering as a possible
  origin for giant planets at small stellar distances}.
\newblock \nat \textbf{384}, 619--621 (1996).
\newblock \doi{10.1038/384619a0}

\bibitem{weiss14}
{Weiss}, L.M., {Marcy}, G.W.: {The Mass-Radius Relation for 65 Exoplanets
  Smaller than 4 Earth Radii}.
\newblock \apjl \textbf{783}, L6 (2014).
\newblock \doi{10.1088/2041-8205/783/1/L6}

\bibitem{weiss18}
{Weiss}, L.M., {Marcy}, G.W., {Petigura}, E.A., {Fulton}, B.J., {Howard}, A.W.,
  {Winn}, J.N., {Isaacson}, H.T., {Morton}, T.D., {Hirsch}, L.A., {Sinukoff},
  E.J., {Cumming}, A., {Hebb}, L., {Cargile}, P.A.: {The California-Kepler
  Survey. V. Peas in a Pod: Planets in a Kepler Multi-planet System Are Similar
  in Size and Regularly Spaced}.
\newblock \aj \textbf{155}, 48 (2018).
\newblock \doi{10.3847/1538-3881/aa9ff6}

\bibitem{weiss13}
{Weiss}, L.M., {Marcy}, G.W., {Rowe}, J.F., {Howard}, A.W., {Isaacson}, H.,
  {Fortney}, J.J., {Miller}, N., {Demory}, B.O., {Fischer}, D.A., {Adams},
  E.R., {Dupree}, A.K., {Howell}, S.B., {Kolbl}, R., {Johnson}, J.A., {Horch},
  E.P., {Everett}, M.E., {Fabrycky}, D.C., {Seager}, S.: {The Mass of KOI-94d
  and a Relation for Planet Radius, Mass, and Incident Flux}.
\newblock \apj \textbf{768}, 14 (2013).
\newblock \doi{10.1088/0004-637X/768/1/14}

\bibitem{wetherill78}
{Wetherill}, G.W.: {Accumulation of the terrestrial planets}.
\newblock In: T.~{Gehrels} (ed.) IAU Colloq. 52: Protostars and Planets, pp.
  565--598 (1978)

\bibitem{wetherill91}
{Wetherill}, G.W.: {Why Isn't Mars as Big as Earth?}
\newblock In: Lunar and Planetary Institute Science Conference Abstracts,
  \emph{Lunar and Planetary Inst. Technical Report}, vol.~22, p. 1495 (1991)

\bibitem{wetherill92}
{Wetherill}, G.W.: {An alternative model for the formation of the asteroids}.
\newblock \icarus \textbf{100}, 307--325 (1992).
\newblock \doi{10.1016/0019-1035(92)90103-E}

\bibitem{wetherill96}
{Wetherill}, G.W.: {The Formation and Habitability of Extra-Solar Planets}.
\newblock Icarus \textbf{119}, 219--238 (1996).
\newblock \doi{10.1006/icar.1996.0015}

\bibitem{wetherill89}
{Wetherill}, G.W., {Stewart}, G.R.: {Accumulation of a swarm of small
  planetesimals}.
\newblock Icarus \textbf{77}, 330--357 (1989).
\newblock \doi{10.1016/0019-1035(89)90093-6}

\bibitem{wetherill93}
{Wetherill}, G.W., {Stewart}, G.R.: {Formation of planetary embryos - Effects
  of fragmentation, low relative velocity, and independent variation of
  eccentricity and inclination}.
\newblock Icarus \textbf{106}, 190 (1993).
\newblock \doi{10.1006/icar.1993.1166}

\bibitem{williams11}
{Williams}, J.P., {Cieza}, L.A.: {Protoplanetary Disks and Their Evolution}.
\newblock \araa \textbf{49}, 67--117 (2011).
\newblock \doi{10.1146/annurev-astro-081710-102548}

\bibitem{windmark12}
{Windmark}, F., {Birnstiel}, T., {G{\"u}ttler}, C., {Blum}, J., {Dullemond},
  C.P., {Henning}, T.: {Planetesimal formation by sweep-up: how the bouncing
  barrier can be beneficial to growth}.
\newblock \aap \textbf{540}, A73 (2012).
\newblock \doi{10.1051/0004-6361/201118475}

\bibitem{winn15}
{Winn}, J.N., {Fabrycky}, D.C.: {The Occurrence and Architecture of
  Exoplanetary Systems}.
\newblock \araa \textbf{53}, 409--447 (2015).
\newblock \doi{10.1146/annurev-astro-082214-122246}

\bibitem{wittenmyer16}
{Wittenmyer}, R.A., {Butler}, R.P., {Tinney}, C.G., {Horner}, J., {Carter},
  B.D., {Wright}, D.J., {Jones}, H.R.A., {Bailey}, J., {O'Toole}, S.J.: {The
  Anglo-Australian Planet Search XXIV: The Frequency of Jupiter Analogs}.
\newblock \apj \textbf{819}, 28 (2016).
\newblock \doi{10.3847/0004-637X/819/1/28}

\bibitem{wittenmyer20}
{Wittenmyer}, R.A., {Wang}, S., {Horner}, J., {Butler}, R.P., {Tinney}, C.G.,
  {Carter}, B.D., {Wright}, D.J., {Jones}, H.R.A., {Bailey}, J., {O'Toole},
  S.J., {Johns}, D.: {Cool Jupiters greatly outnumber their toasty siblings:
  occurrence rates from the Anglo-Australian Planet Search}.
\newblock \mnras \textbf{492}(1), 377--383 (2020).
\newblock \doi{10.1093/mnras/stz3436}

\bibitem{wolfgang16}
{Wolfgang}, A., {Rogers}, L.A., {Ford}, E.B.: {Probabilistic Mass-Radius
  Relationship for Sub-Neptune-Sized Planets}.
\newblock \apj \textbf{825}, 19 (2016).
\newblock \doi{10.3847/0004-637X/825/1/19}

\bibitem{wright11}
{Wright}, J.T., {Fakhouri}, O., {Marcy}, G.W., {Han}, E., {Feng}, Y.,
  {Johnson}, J.A., {Howard}, A.W., {Fischer}, D.A., {Valenti}, J.A.,
  {Anderson}, J., {Piskunov}, N.: {The Exoplanet Orbit Database}.
\newblock ArXiv e-prints  (2010)

\bibitem{wright08}
{Wright}, J.T., {Marcy}, G.W., {Butler}, R.P., {Vogt}, S.S., {Henry}, G.W.,
  {Isaacson}, H., {Howard}, A.W.: {The Jupiter Twin HD 154345b}.
\newblock \apjl \textbf{683}, L63--L66 (2008).
\newblock \doi{10.1086/587461}

\bibitem{wright09}
{Wright}, J.T., {Upadhyay}, S., {Marcy}, G.W., {Fischer}, D.A., {Ford}, E.B.,
  {Johnson}, J.A.: {Ten New and Updated Multiplanet Systems and a Survey of
  Exoplanetary Systems}.
\newblock \apj \textbf{693}, 1084--1099 (2009).
\newblock \doi{10.1088/0004-637X/693/2/1084}

\bibitem{wyatt08}
{Wyatt}, M.C.: {Evolution of Debris Disks}.
\newblock \araa \textbf{46}, 339--383 (2008).
\newblock \doi{10.1146/annurev.astro.45.051806.110525}

\bibitem{wyatt12}
{Wyatt}, M.C., {Kennedy}, G., {Sibthorpe}, B., {Moro-Mart{\'\i}n}, A.,
  {Lestrade}, J.F., {Ivison}, R.J., {Matthews}, B., {Udry}, S., {Greaves},
  J.S., {Kalas}, P., {Lawler}, S., {Su}, K.Y.L., {Rieke}, G.H., {Booth}, M.,
  {Bryden}, G., {Horner}, J., {Kavelaars}, J.J., {Wilner}, D.: {Herschel
  imaging of 61 Vir: implications for the prevalence of debris in low-mass
  planetary systems}.
\newblock \mnras \textbf{424}(2), 1206--1223 (2012).
\newblock \doi{10.1111/j.1365-2966.2012.21298.x}

\bibitem{yang17}
{Yang}, C.C., {Johansen}, A., {Carrera}, D.: {Concentrating small particles in
  protoplanetary disks through the streaming instability}.
\newblock \aap \textbf{606}, A80 (2017).
\newblock \doi{10.1051/0004-6361/201630106}

\bibitem{youdin05}
{Youdin}, A.N., {Goodman}, J.: {Streaming Instabilities in Protoplanetary
  Disks}.
\newblock \apj \textbf{620}, 459--469 (2005).
\newblock \doi{10.1086/426895}

\bibitem{zellner17}
{Zellner}, N.E.B.: {Cataclysm No More: New Views on the Timing and Delivery of
  Lunar Impactors}.
\newblock Origins of Life and Evolution of the Biosphere \textbf{47}, 261--280
  (2017).
\newblock \doi{10.1007/s11084-017-9536-3}

\bibitem{zhang10}
{Zhang}, H., {Zhou}, J.L.: {On the Orbital Evolution of a Giant Planet Pair
  Embedded in a Gaseous Disk. I. Jupiter-Saturn Configuration}.
\newblock \apj \textbf{714}, 532--548 (2010).
\newblock \doi{10.1088/0004-637X/714/1/532}

\bibitem{Zhang18}
{Zhang}, Q.: {Prospects for Backtracing 1I/{\lsquo}Oumuamua and Future
  Interstellar Objects}.
\newblock \apjl \textbf{852}, L13 (2018).
\newblock \doi{10.3847/2041-8213/aaa2f7}

\bibitem{zhou05}
{Zhou}, J.L., {Aarseth}, S.J., {Lin}, D.N.C., {Nagasawa}, M.: {Origin and
  Ubiquity of Short-Period Earth-like Planets: Evidence for the Sequential
  Accretion Theory of Planet Formation}.
\newblock \apjl \textbf{631}, L85--L88 (2005).
\newblock \doi{10.1086/497094}

\bibitem{zhu18}
{Zhu}, W., {Wu}, Y.: {The Super Earth-Cold Jupiter Relations}.
\newblock \aj \textbf{156}(3), 92 (2018).
\newblock \doi{10.3847/1538-3881/aad22a}

\bibitem{zube19}
{Zube}, N.G., {Nimmo}, F., {Fischer}, R.A., {Jacobson}, S.A.: {Constraints on
  terrestrial planet formation timescales and equilibration processes in the
  Grand Tack scenario from Hf-W isotopic evolution}.
\newblock Earth and Planetary Science Letters \textbf{522}, 210--218 (2019).
\newblock \doi{10.1016/j.epsl.2019.07.001}

\end{thebibliography}

